Temporal graph patterns by timed automata

Temporal graphs represent graph evolution over time, and have been receiving considerable research attention. Work on expressing temporal graph patterns or discovering temporal motifs typically assumes relatively simple temporal constraints, such as journeys or, more generally, existential constraints, possibly with finite delays. In this paper we propose to use timed automata to express temporal constraints, leading to a general and powerful notion of temporal basic graph pattern (BGP). The new difficulty is the evaluation of the temporal constraint on a large set of matchings. An important benefit of timed automata is that they support an iterative state assignment, which can be useful for early detection of matches and pruning of non-matches. We introduce algorithms to retrieve all instances of a temporal BGP match in a graph, and present results of an extensive experimental evaluation, demonstrating interesting performance trade-offs. We show that an on-demand algorithm that processes total matchings incrementally over time is preferable when dealing with cyclic patterns on sparse graphs. On acyclic patterns or dense graphs, and when connectivity of partial matchings can be guaranteed, the best performance is achieved by maintaining partial matchings over time and allowing automaton evaluation to be fully incremental.

==> TAA_vs_SQL.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!t]
\small
\caption{Best-performing timed-automaton algorithm (TAA) compared to \duck and \hyper, for SQL queries in Figure~\ref{fig:query-ta}.}
\label{table:query-ta}
\begin{tabular}{lrrrrr}
\multicolumn{3}{l}{} & \multicolumn{3}{c}{\textbf{time(sec)}} \\
\multicolumn{1}{l|}{\textbf{BGP/ \#match}} & \textbf{TA} & \multicolumn{1}{r|}{\textbf{\#Acc.}} & \textbf{TAA} & \textbf{DuckDB} & \textbf{Hyper} \\ \hline
\multicolumn{1}{l|}{\multirow{9}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}EPL \\ Path2 \\ (47464)\end{tabular}}}} & $\ta_e$ & \multicolumn{1}{r|}{35866} & \textbf{1.09} & 1.11 & 1.44 \\
\multicolumn{1}{l|}{} & $\ta_1$ & \multicolumn{1}{r|}{1801} & \textbf{0.06} & 60.14 & 17.84 \\
\multicolumn{1}{l|}{} & $\ta_2$ & \multicolumn{1}{r|}{374} & \textbf{0.05} & 69.89 & 11.36 \\
\multicolumn{1}{l|}{} & $\ta_3$ & \multicolumn{1}{r|}{21035} & \textbf{0.04} & 0.07 & 0.13 \\
\multicolumn{1}{l|}{} & $\ta_4$ & \multicolumn{1}{r|}{29726} & \textbf{0.06} & 0.07 & 0.13 \\
\multicolumn{1}{l|}{} & $\ta_5$ & \multicolumn{1}{r|}{1714} & \textbf{0.07} & 18.57 & 0.39 \\
\multicolumn{1}{l|}{} & $\ta_6$ & \multicolumn{1}{r|}{19578} & 0.54 & 0.12 & \textbf{0.09} \\
\multicolumn{1}{l|}{} & $\ta_7$ & \multicolumn{1}{r|}{257} & \textbf{1.3} & 8.22 & 5.56 \\
\multicolumn{1}{l|}{} & $\ta_8$ & \multicolumn{1}{r|}{5377} & 0.23 & \textbf{0.17} & 0.21 \\ \hline
\multicolumn{1}{l|}{\multirow{9}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}EPL\\ Cycle2 \\ (1158)\\ \amir{this can go} \end{tabular}}}} & $\ta_e$ & \multicolumn{1}{r|}{933} & 0.04 & 0.597 & \textbf{0.01} \\
\multicolumn{1}{l|}{} & $\ta_1$ & \multicolumn{1}{r|}{35} & \textbf{0.01} & 2.67 & 0.41 \\
\multicolumn{1}{l|}{} & $\ta_2$ & \multicolumn{1}{r|}{22} & \textbf{0.01} & 3.33 & 0.26 \\
\multicolumn{1}{l|}{} & $\ta_3$ & \multicolumn{1}{r|}{418} & \textbf{0.01} & 0.1 & \textbf{0.01} \\
\multicolumn{1}{l|}{} & $\ta_4$ & \multicolumn{1}{r|}{740} & \textbf{0.01} & 0.1 & \textbf{0.01} \\
\multicolumn{1}{l|}{} & $\ta_5$ & \multicolumn{1}{r|}{90} & \textbf{0.02} & 0.53 & 1.19 \\
\multicolumn{1}{l|}{} & $\ta_6$ & \multicolumn{1}{r|}{312} & 0.07 & 0.07 & \textbf{0.01} \\
\multicolumn{1}{l|}{} & $\ta_7$ & \multicolumn{1}{r|}{0} & \textbf{0.05} & 1.18 & 5.15 \\
\multicolumn{1}{l|}{} & $\ta_8$ & \multicolumn{1}{r|}{188} & 0.02 & \textbf{0.01} & 0.09 \\ \hline
\multicolumn{1}{l|}{\multirow{9}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Contact\\ O-Star2 \\ (417029)\end{tabular}}}} & $\ta_e$ & \multicolumn{1}{r|}{169410} & \textbf{8.87} & 22.43 & 19.29 \\
\multicolumn{1}{l|}{} & $\ta_1$ & \multicolumn{1}{r|}{0} & \textbf{0.67} & \omem & 316.5 \\
\multicolumn{1}{l|}{} & $\ta_2$ & \multicolumn{1}{r|}{0} & \textbf{0.72} & \omem & 205.95 \\
\multicolumn{1}{l|}{} & $\ta_3$ & \multicolumn{1}{r|}{101268} & \textbf{0.58} & 0.95 & 0.69 \\
\multicolumn{1}{l|}{} & $\ta_4$ & \multicolumn{1}{r|}{107650} & \textbf{0.67} & 0.91 & 0.68 \\
\multicolumn{1}{l|}{} & $\ta_5$ & \multicolumn{1}{r|}{4154} & \textbf{0.72} & \omem & 2.035 \\
\multicolumn{1}{l|}{} & $\ta_6$ & \multicolumn{1}{r|}{10832} & 4.68 & 0.99 & \textbf{0.54} \\
\multicolumn{1}{l|}{} & $\ta_7$ & \multicolumn{1}{r|}{76} & \textbf{15.12} & \omem & 102.89 \\
\multicolumn{1}{l|}{} & $\ta_8$ & \multicolumn{1}{r|}{4646} & 1.3 & \textbf{1.1} & 1.16 \\ \hline
\multicolumn{1}{l|}{\multirow{9}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Email \\ Path2 \\ (862020)\end{tabular}}}} & $\ta_e$ & \multicolumn{1}{r|}{719609} & 501.07 & 649.69 & \textbf{239.82} \\
\multicolumn{1}{l|}{} & $\ta_1$ & \multicolumn{1}{r|}{35594} & \textbf{22.35} & \omem & \omem \\
\multicolumn{1}{l|}{} & $\ta_2$ & \multicolumn{1}{r|}{801} & \textbf{3.73} & \omem & 1748.85 \\
\multicolumn{1}{l|}{} & $\ta_3$ & \multicolumn{1}{r|}{443431} & \textbf{2.71} & 17.84 & 8.59 \\
\multicolumn{1}{l|}{} & $\ta_4$ & \multicolumn{1}{r|}{455977} & \textbf{3.05} & 17.78 & 8.26 \\
\multicolumn{1}{l|}{} & $\ta_5$ & \multicolumn{1}{r|}{2474} & \textbf{1.27} & \omem & 48.87 \\
\multicolumn{1}{l|}{} & $\ta_6$ & \multicolumn{1}{r|}{693956} & 320.04 & 8.98 & \textbf{5.61} \\
\multicolumn{1}{l|}{} & $\ta_7$ & \multicolumn{1}{r|}{390} & \textbf{327.33} & \omem & \omem \\
\multicolumn{1}{l|}{} & $\ta_8$ & \multicolumn{1}{r|}{12919} & 19.32 & \textbf{8.02} & 21.58 \\ \hline
\multicolumn{1}{l|}{\multirow{9}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Email \\ Cycle2 \\ (17730)\end{tabular}}}} & $\ta_e$ & \multicolumn{1}{r|}{14188} & \textbf{4.71} & 254.7 & 15.3 \\
\multicolumn{1}{l|}{} & $\ta_1$ & \multicolumn{1}{r|}{843} & \textbf{0.83} & \omem & 1788.87 \\
\multicolumn{1}{l|}{} & $\ta_2$ & \multicolumn{1}{r|}{240} & \textbf{0.64} & \omem & 1733.05 \\
\multicolumn{1}{l|}{} & $\ta_3$ & \multicolumn{1}{r|}{6333} & 0.44 & \textbf{0.38} & 0.68 \\
\multicolumn{1}{l|}{} & $\ta_4$ & \multicolumn{1}{r|}{11396} & 0.43 & \textbf{0.38} & 0.68 \\
\multicolumn{1}{l|}{} & $\ta_5$ & \multicolumn{1}{r|}{1800} & \textbf{0.97} & 206.26 & 1.19 \\
\multicolumn{1}{l|}{} & $\ta_6$ & \multicolumn{1}{r|}{4230} & 24.09 & 8.63 & \textbf{5.48} \\
\multicolumn{1}{l|}{} & $\ta_7$ & \multicolumn{1}{r|}{134} & \textbf{7.1} & \omem & \omem \\
\multicolumn{1}{l|}{} & $\ta_8$ & \multicolumn{1}{r|}{3441} & 1.79 & \textbf{0.219} & 49.79
\end{tabular}
\end{table}

==> exp_old.tex <==
\section{Experiments}
\label{sec:experiments}
%In this section, we show our experimental results over the methods we proposed to enforce the constraints expressed by the temporal automata. 

We conducted an extensive experimental evaluation with several real datasets and temporal graph patterns, and demonstrated that using timed automata to evaluate temporal BGPs is practical.  We observed that the \od and \pmatch algorithms are effective at reducing the running time.  Interestingly, while no single algorithm performs best in all cases, the trade-off in performance can be explained by the properties of the dataset, of the BGP, and of the temporal constraint.

%we can predict which algorithm should be selected based on the graph pattern, temporal constraints, dataset structural density, and size of the graph. 

{\bf In summary,} our results indicate that the \pmatch algorithm is most efficient for acylic BGPs such as paths of bounded length. The \od algorithm outperforms \pmatch for cyclic BGPs such as triangles, particularly when evaluated over sparse temporal graphs.  Interestingly, the performance gap between \od and \pmatch is reduced with increasing graph density or BGP size, and \pmatch outperforms \od in some cases.
%Further, while the total running time for \od and the \pmatch follow similar trends, \od can be a better option for returning results sooner, as they are computed.
We also show that algorithm performance is independent of timed automata size and of the number of clocks.

%as the structural denisity of the graph or the BGP size increase, the performance gap between the partial matching algorithm and the baseline and on-demand algorithms for cyclic patterns becomes smaller and in some cases the partial matching algorithm can run faster than the other two. 

%Total running time for the on-demand algorithm and baseline algorithm follow the same trend, but the on-demand algorithm can be a better option for cases where we want to view the intermediate results. 


%for the cases where the temporal constraints can not guarantee the partial matching connectivity, we can not use the partial matching algorithm as this algorithm would not produce the correct result for all matching. 

Note that the baseline algorithm can only be used when a graph's evolution history is fully available, rather than when the graph is arriving as a stream.  Moreover, as discussed in Section~\ref{sec:par-good}, the \pmatch algorithm is only used when the matching is guaranteed to be connected.

%\subsection{Experimental setup}
%\label{sec:experiments:data}

%\begin{table}[t!]
%\caption{Temporal graph datasets used for evaluation.}  
%\label{tab:datasets}
%\centering
%\small 
%\begin{tabular}{lcccccc}
% & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{2}{c}{\textbf{density}} \\ \hline
%\multicolumn{1}{|l|}{} & \multicolumn{1}{c|}{\textbf{\# nodes}} & \multicolumn{1}{c|}{\textbf{\# edges}} & \multicolumn{1}{c|}{\textbf{\# active}} & \multicolumn{1}{c|}{\textbf{\# snaps}} & %\multicolumn{1}{c|}{\textbf{struct}} & \multicolumn{1}{c|}{\textbf{temp}} \\ \hline
%\multicolumn{1}{|l|}{\textbf{EPL}} & \multicolumn{1}{c|}{50} & \multicolumn{1}{c|}{1500} & %\multicolumn{1}{c|}{35K} & \multicolumn{1}{c|}{25} & \multicolumn{1}{c|}{0.6} & \multicolumn{1}{c|}{0.93} \\ %\hline
%\multicolumn{1}{|l|}{\textbf{EU-Email}} & \multicolumn{1}{c|}{776} & \multicolumn{1}{c|}{65K} & \multicolumn{1}{c|}{1.9M} & \multicolumn{1}{c|}{800} & \multicolumn{1}{c|}{0.1} & \multicolumn{1}{c|}{0.03} \\ \hline
%\multicolumn{1}{|l|}{\textbf{FB-Wall}} & \multicolumn{1}{c|}{46K} & \multicolumn{1}{c|}{264K} & \multicolumn{1}{c|}{856K} & \multicolumn{1}{c|}{1500} & \multicolumn{1}{c|}{0.0001} & \multicolumn{1}{c|}{0.002} %\\ \hline
%\end{tabular}
%\end{table}

\paragraph{Experimental setup} All experiments were executed over as a single-thread Rust program, running on a single cluster node with 32 GB of RAM, an Intel Xeon Platinum 8268 CPU, with the Slurm scheduler~\cite{yoo2003slurm}. %Experiments were run on a single node of NYU Greene which utilizes SLURM\cite{yoo2003slurm}. 
All reported execution times are averages of three runs, and include loading the data from the disk, loading the timed automata, and the execution of temporal BGP matching algorithms. The coefficient of variation of the running times was under 10\% in most cases (max 12\%). 

\paragraph{Datasets.} Experiments in this section were conducted over three real datasets and on several synthetic datasets that we derive from them to explore the impact of dataset characteristics on performance. In the table below, we list properties of the real datasets: the number of distinct nodes and edges, the size of the temporal domain (``snaps''), the number of active edges across snapshots (``active''), the structural density (``struct'', the number of edges in the graph, divided by the number of edges that would be present in a clique over the same number of nodes), and the temporal density (``temp'', the number of time points during which an edge is active, divided by the size of the temporal domain, on average).
\begin{center}
\small 
\begin{tabular}{lcccccc}
 & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{2}{c}{\textbf{density}} \\ \hline
\multicolumn{1}{|l|}{} & \multicolumn{1}{c|}{\textbf{nodes}} & \multicolumn{1}{c|}{\textbf{edges}} & \multicolumn{1}{c|}{\textbf{active}} & \multicolumn{1}{c|}{\textbf{snaps}} & \multicolumn{1}{c|}{\textbf{struct}} & \multicolumn{1}{c|}{\textbf{temp}} \\ \hline
\multicolumn{1}{|l|}{\textbf{EPL}} & \multicolumn{1}{c|}{50} & \multicolumn{1}{c|}{1500} & \multicolumn{1}{c|}{35K} & \multicolumn{1}{c|}{25} & \multicolumn{1}{c|}{0.6} & \multicolumn{1}{c|}{0.93} \\ \hline
\multicolumn{1}{|l|}{\textbf{EU-Email}} & \multicolumn{1}{c|}{776} & \multicolumn{1}{c|}{65K} & \multicolumn{1}{c|}{1.9M} & \multicolumn{1}{c|}{800} & \multicolumn{1}{c|}{0.1} & \multicolumn{1}{c|}{0.03} \\ \hline
\multicolumn{1}{|l|}{\textbf{FB-Wall}} & \multicolumn{1}{c|}{46K} & \multicolumn{1}{c|}{264K} & \multicolumn{1}{c|}{856K} & \multicolumn{1}{c|}{1500} & \multicolumn{1}{c|}{0.0001} & \multicolumn{1}{c|}{0.002} \\ \hline
\end{tabular}
\end{center}

{\bf EPL}, derived from the English soccer dataset~\cite{curley2016engsoccerdata}, represents 34,800 matches between 50 teams over a 25-year period. We represent this data as a temporal graph with 1-year temporal resolution, where each node corresponds to a team and a directed edge connects a pair of teams that played at least one match during that year.  The direction of the edge is from a team with the higher number of goals to the team with the lower number of goals in the matches they played against each other that year; edges are added in both directions in the case of a tied result.   This is the smallest dataset in our evaluation, but it is very dense both structurally and temporally.

{\bf EU-Email}, derived from a dataset of email communications within a large European research institution~\cite{DBLP:journals/tkdd/LeskovecKF07}, represents about 1.9M email messages exchanged by 776 users over an 800-day period, with about 65K distinct pairs of users exchanging messages.  This dataset has the largest number of active edges in our experiments, it has high structural density (10\% of all possible pairs of users are connected at some point during the graph's history), and intermediate temporal density (3\%).

{\bf FB-Wall}, derived from the Facebook New Orleans user network dataset~\cite{viswanath-2009-activity}, represents wall posts of about 46K users over a 1,500-day period, with 264K unique pairs of users (author / recipient of post).  This graph has the largest temporal domain in our experiments, and it is sparse, both structurally and temporally. 

%\jan{is it EFL or EPL? both are used in the text.}
%(1) Soccer, comprising 25 years of EPL data with 50 unique nodes, 1500 unique edges, and a temporal domain of 25 timepoints (years)~\cite{curley2016engsoccerdata}. In EPL the direction of each edge is from the winner team to the loser team and in cases of a tie one edge in each direction would exist. For cases where we have multiple games between the same pair of teams in one year, we select the winner based on the score total in the matches of that year. 
%(2) Eu-Email, email communications within a large European research institution over 800 days with 776 unique nodes, 65000 unique edges, and a temporal domain of 800 timepoints \cite{DBLP:journals/tkdd/LeskovecKF07}. 
%(3) FB-Wall, wall posts over a period of 1500 days within the Facebook New Orleans network~\cite{viswanath-2009-activity} with 46000 unique nodes and 264000 unique edges.

%Node ids and edge ids in all datasets have been randomly assigned to remove any possible correlation between ids and time.\jan{is this important?} \julia{no}

%The selected datasets differ not only in size, but also in structural density (number of existing edges divided by number of theoretically possible edges), and temporal density (average percentage of number of timepoints that an edge is active). Table~\ref{tab:datasets} shows a summary of the dataset characteristics.  The EPL dataset has a large temporal and structural density, meaning that most of the edges exist in all snapshots. Eu-Email has smaller densities, and even more so for FB-Wall which is quite sparse.

%\julia{what are these time points for each of these, do they correspond to years?  need citations to where you got the data also}


% \julia{temporal density: active/ (edges * snaps)}

\subsection{Relative performance of the algorithms}
\label{sec:experiments:constr}

\begin{figure}
\centering
\subfloat[EPL, 47K BGP matches ]{%
\label{fig:nfa-type:epl}%
\includegraphics[width=0.5\columnwidth]{figs/nfa-type/chart-37.pdf}}
\subfloat[EU-Email, 862K BGP matches]{%
\label{fig:nfa-type:euemail}%
\includegraphics[width=0.5\columnwidth]{figs/nfa-type/chart-38.pdf}}%%
\caption{Execution time of timed automata $\ta_1, \ta_2, and \ta_3$ for path of length 2 for the EPL and EU-Email datasets.}
\label{fig:nfa-type-time}
\end{figure}

In our first set of experiments, we evaluate the performance of the baseline, \od, and \pmatch algorithms for three temporal BGPs that look for a paths of length 2 under the temporal constraints expressed by timed automata $\ta_1$  (temporal alternation, Figure~\ref{fig:bgp-cycle2:ta1}), $\ta_2$ (temporal alternation with a clock, Figure~\ref{fig:bgp-cycle2:ta2}), and $\ta_3$ (edges appear in temporal order, Figure~\ref{fig:nfa-type-ta3}).  We discussed  $\ta_1$  and  $\ta_2$ in the introduction, and used  $\ta_2$ to illustrate our algorithms in Section~\ref{sec:algorithms}.  automata  $\ta_3$ expresses another simple and practically useful constraint, and it is interesting because it will allow us to show the impact of early acceptance and rejection on performance.   

%As our first experiment, we will look at the performance of various types of automata discussed in the body of this paper. To study this, we fixed our BGP structure to a simple ``path2'' query and  measured the execution time for different automata in Figure~\ref{fig:nfa-type} over different datasets.  We consider the timed automata $\ta_1$ and $\ta_2$ from the Introduction. We also consider automton $\ta_3$ shown in Figure~\ref{fig:nfa-type-ta3}, specifying the order constraint that the first time $y_1$ existed was before $y_2$. %\jan{do you mean $y_1 \land \neg y_2$? could be abbreviated by $\{y_1\}$ in the figure.}
%\jan{Also, TA3 is also given as an example in Section 3.} This automata is a good example to show the effects of early acceptance or early rejection.




Figure ~\ref{fig:nfa-type-time} show the execution time of the baseline, \od and \pmatch  algorithms for EPL and EU-Email, also noting the number of temporal matches.  The BGP, which is in common for all executions in this experiment, returns 47K matches on EPL and 862K matches on EU-Email.  When the temporal constraint is applied, the number of matches is reduced, and is presented on the $x$-axis.  For example, $\ta_1$ returns 319 temporal matches on EPL and 36K temporal matches on EU-Email.

We observe that \pmatch is the most efficient algorithm for all queries and for both datasets in this experiment, returning in under 0.06 sec for EPL, and in under 18 sec for EU-Email in all cases.  The \od algorithm outperforms the baseline in most cases, but is slower than \pmatch.  

We also observe that the relative performance of the algorithms is different depending on the number of matches.  We explore this relationship further in the next experiment, where we vary the BGP, fix the kind of a timed automata that is executed, and look at the relative performance of the algorithms.

%Next, we will further explore the relative performance of \od and \pmatch by relating it to properties of the temporal graph over which the temporal BGP is executed.

%and number of accepted matches for each of these timed automatas. In this figure x-axis shows the name of the automata and y-axis shows the execution time in seconds. As it can be seen, for both datasets and all timed automatas, the partial matching algorithm is significantly faster than the baseline and on-demand. Baseline algorithm and on-demand algorithm show similar trends. 
 
%Another  observation here is the number of accepted matchings. The total number of ``path2'' BGPs for  the EPL dataset is around 47K and for Eu-Email is 862K. For EPL, as we can see in Figure~\ref{fig:nfa-type:epl} $\ta_1$  accepted around 319, $\ta_2$ acceded 92 and $\ta_3$ accepted around 1.8k.   For Eu-Email, as we can see in Figure~\ref{fig:nfa-type:euemail} $\ta_1$  accepted around 36K, $\ta_2$ acceded 0 and $\ta_3$ accepted around 138k.  The difference between the number of accepted matchings in $\ta_1$ and $\ta_2$ is interesting because they are both enforcing the same constraint but in $\ta_2$ we have a clock. This means while many matchings satisfy the alternation constrain, the majority of those those(none for Eu-Email) do not satisfy it in a window smaller than 3. In Section~\ref{sec:ex:select} we will look at the effect of query selectivity on the performance of each of the algorithms.

\subsection{Properties of the temporal graph}
\label{sec:experiments:density}
In this set of experiments, we explore the effect of the structural density of the graph on algorithm performance.
%As we discussed in the previous section, the graph structural density can affect the total execution time. 
We synthetically generated a complete graph with 50 nodes and 2450 edges (the same size at the EPL dataset)  and temporal density of $0.5$. From this complete graph, then we sampled edges to create a graph with different structural densities. 

Using the timed automata in Figure~\ref{fig:all-nfa}, we measure our partial matching and baseline algorithm performance for different patterns. This automata passes the necessary conditions needed for the partial matching algorithm to work and does not drop any other matching.  Note that this figure is showing an automata for patterns of size 3, for the pattern of size 4 we used a similar automata with one extra state. 

Figure~\ref{fig:graph-dense-result} show the execution time of each algorithm for different densities from 0.1 to 1.0, where a graph with a density of 1.0 is a directed complete graph.  As it can be seen, for acyclic patterns as explained before, the partial algorithm shows a better performance, but for graphs with low structural density the performance of the two algorithms are similar. For the cyclic pattern of size 3, we can see that the baseline algorithm has a better performance, but as we increase the density, the partial algorithm makes the performance gap smaller. For the cycle of length 4 and sparse graphs, the baseline algorithm is faster, but we can see if we have a dense graph, the partial matching algorithm will become the best choice. Note that the performance of the on-demand algorithm follows the same trend as the baseline.  

In summary, the baseline algorithm and on-demand algorithm are faster when we have a sparse graph but lose its leverage when the graph becomes denser or when the patterns become larger. 


\begin{figure*}
\centering
\subfloat[Path 3  ]{%
%\label{fig:}%
\includegraphics[width=0.45\columnwidth]{figs/densitiy/chart-11.pdf}}
\subfloat[Cycle 3]{%

\includegraphics[width=0.45\columnwidth]{figs/densitiy/chart-12.pdf}}%%
\subfloat[Path 4]{%

\includegraphics[width=0.45\columnwidth]{figs/densitiy/chart-13.pdf}}%%
\subfloat[Cycle 4]{%

\includegraphics[width=0.45\columnwidth]{figs/densitiy/chart-14.pdf}}%%
\caption{Structural Density / Exec time for various BGPs using the automata $\ta_4$ , on-demand and partial algorithm. The on-demand algorithm followed the same trend as the baseline.  When graph density is low, the baseline and the partial matching algorithm perform comparably.  As density increases, the partial matching algorithm start having an advantage over the baseline.}
\label{fig:graph-dense-result}

\vspace{-0.5cm}
\end{figure*}

\subsection{Number of Clocks and automata Size}
\label{sec:experiments:automata}

In the previous section, we showed that different timed automatas result in different execution times. To study this further, here we are studying the affect of the  size of the automata and the number of clocks on the execution time. 

To study the effect of the timed automata size, we fixed our BGP to ``cycle4'', and our temporal constraint to a version of automata $\ta_0$ in Figure~\ref{fig:inc-nfa} with 4 states. The $\ta_0$ automata is generalized case of $\ta_1$ automata. This automata enforces an circular queue, meaning if $i<j$, we expect to see $y_i$ before $y_j$ once, and each edge would go to the end of the priority queue after their turn.  In addition, this automata is resilient to cases when none of the edges exist.  

Using $\ta_0$ automata, then we create equivalent automatas with different number of states. This is possible by copying the states in cycles. By doing this, we can guarantee that the output size will stay fixed.  Figure~\ref{fig:nfa-size} shows the execution time for a ``cycle4'' query over EPL dataset. In this figure axis-x shows the number of states and axis-y shows the execution times. As it can be seen, the total execution time is not a function of the number of states in the automata and even for an automata with 256 states the execution times remain fixed. The timed automata relation size compared to the matching relation is tiny and this result was expected. In practice, this means we can check many temporal constraints at once without seeing any significant impact on the performance. 

\begin{figure*}[t!]
    \centering
    \subfloat[$\ta_0$ generalizes $\ta_1$, specifying that edges should appear one at a time, in temporal order]{
    \label{fig:inc-nfa}%
    \resizebox{0.7\columnwidth}{!}{
 \begin{tikzpicture}[->, on grid, node distance=45pt]
    \node[state, initial] (s0) {$s_0$};
    \node[state, right of=s0,accepting] (s1) {$s_1$};
    \node[state, right of=s1,accepting] (s2) {$\dots$};
    \node[state, right of=s2,accepting] (s3) {$s_m$};
    \draw (s0)
     (s0) edge[loop above] node{$\emptyset   $} (s0)
      (s1) edge[loop above] node{$\emptyset $} (s1)
      (s2) edge[loop above] node{$\emptyset$} (s2)
      (s3) edge[loop above] node{$\emptyset$} (s3)
    
      (s0) edge[above] node{$\{y_1\}$} (s1)
      (s1) edge[above] node{$\dots$} (s2)
      (s2) edge[above] node{$\{y_{m-1}\}$} (s3)
      (s3) edge[below, bend left = 50] node{$\{y_m\} $} (s0);
    \end{tikzpicture}
}
     }
    \qquad
      \subfloat[$\ta_4$ accepts all temporal words of length 3]{
      \label{fig:all-nfa}
          \resizebox{0.7\columnwidth}{!}{
        \begin{tikzpicture}[->, on grid, node distance=50pt]
    \node[state, initial] (s0) {$s_0$};
    \node[state, right of=s0,accepting] (s1) {$s_1$};
    \node[state, right of=s1,accepting] (s2) {$s_2$};
    \node[state, right of=s2,accepting] (s3) {$s_3$};
    \draw (s0)
  (s0) edge[loop above] node{$\emptyset$} (s0)
  (s1) edge[loop above] node{$\emptyset$} (s1)
  (s2) edge[loop above] node{$\emptyset$} (s2)
  (s3) edge[loop above] node{$\mathit{true}$} (s3)

  (s0) edge[above] node{$\{y_1\}$} (s1)
  (s0) edge[below, bend right] node{$y_1 \land y_2  \land \neg y_3$} (s2)
  (s0) edge[below, bend right = 50] node{$y_1 \land y_2 \land y_3$} (s3)
  (s1) edge[below, bend right] node{$y_2 \land y_3$} (s3)
  (s1) edge[above] node{$\{y_2\}$} (s2)
  (s2) edge[above] node{$\{y_3\}$} (s3);
    \end{tikzpicture}
    }
        }
        \caption{$\ta_0$ and $\ta_4$}
\end{figure*}


% \begin{figure}
%  \resizebox{0.8\columnwidth}{!}{
%  \begin{tikzpicture}[->, on grid, node distance=50pt]
%     \node[state, initial] (s0) {$s_0$};
%     \node[state, right of=s0,accepting] (s1) {$s_1$};
%     \node[state, right of=s1,accepting] (s2) {$\dots$};
%     \node[state, right of=s2,accepting] (s3) {$s_m$};
%     \draw (s0)
% %   (s0) edge[loop above] node{$\bigwedge_{_{i=1,\dots,m}} ^{\neg y_i}   $} (s0)
% %   (s1) edge[loop above] node{$\bigwedge_{_{i=1,\dots,m}} ^{\neg y_i}   $} (s1)
% %   (s2) edge[loop above] node{$\bigwedge_{_{i=1,\dots,m}} ^{\neg y_i}   $} (s2)
% %   (s3) edge[loop above] node{$\bigwedge_{_{i=1,\dots,m}} ^{\neg y_i}   $} (s3)
%  (s0) edge[loop above] node{$\emptyset   $} (s0)
%   (s1) edge[loop above] node{$\emptyset $} (s1)
%   (s2) edge[loop above] node{$\emptyset$} (s2)
%   (s3) edge[loop above] node{$\emptyset$} (s3)

%   (s0) edge[above] node{$\{y_1\}$} (s1)
%   (s1) edge[above] node{$\dots$} (s2)
%   (s2) edge[above] node{$\{y_{m-1}\}$} (s3)
%   (s3) edge[below, bend left] node{$\{y_m\} $} (s0);
%     \end{tikzpicture}
%     }
%     \caption{$TA_0$ generalizes $TA_1$, specifying that edges should appear one at a time, in temporal order.}
%     \label{fig:inc-nfa}
% \end{figure}

To study effect of the number of clocks on performance, we added multiple clocks to the automata in Figure~\ref{fig:inc-nfa} and we reset  all clocks at every state of the automata. To ensure that any possible difference is not due to the change of the output size, the condition of each clock is set to $\mathit{true}$.  Figure~\ref{fig:clock} shows the result of this experiment. In this figure axis-x shows the number of clocks and axis-y shows the execution time in seconds. As it can be seen, the number of clocks affected on the performance is minor, which can be explained by the computation of the overhead of storing and updating clocks. 

\begin{figure}
\centering
\subfloat[\# states in automata ]{%
\label{fig:nfa-size}%
\includegraphics[width=0.5\columnwidth]{figs/nfa-size/chart-6.pdf}}
\subfloat[\# clock in  automata]{%
\label{fig:clock}%
\includegraphics[width=0.5\columnwidth]{figs/nfa-size/chart-7.pdf}}%%
\caption{Size of automata Effect on time for a ``cycle4''  and temporal constrain as described in the automata $\ta_0$ in Figure~\ref{fig:inc-nfa}. Results shows execution time for EPL dataset. }
\label{fig:nfa-size}
\vspace{-0.5cm}
\end{figure}

\subsection{Size of the temporal domain} Our algorithms run over all points in the time domain and hence for graphs with a larger time domain, we can expect to have a longer execution time. To measure this effect, without changing the structure or the size of the graph, we changed the temporal resolution of the Eu-Email dataset, creating graphs with 50 to 800 snapshots. In this way, the total number of matchings would remain unchanged, but the temporal domain would become smaller. Note that this process by nature would change the temporal density of the graph and affect the size of output. To reduce this effect, in this experiment we are using a timed automata described in Figure~\ref{fig:all-nfa}. 

Figure~\ref{fig:temp-size} shows the result of executing the cycle-3 query on Eu-Email dataset with varying temporal domain size. In this figure, the x-axis shows the size of the temporal domain and the y-axis shows the execution time in seconds. As it can be seen, the baseline and on-demand algorithm execution time increases linearly with the temporal domain size. For partial matching, the execution time increase seems to follow an exponential trend. 

\begin{figure}
	\centering
	\includegraphics[width=0.5\columnwidth]{figs/num-snaps.pdf}
    \caption{Num. of Snaps / Exec Time for Cycle3 pattern of Eu-Email with different temporal resolution using the automata $\ta_4$}
    \label{fig:temp-size}
\end{figure}


\subsection{Pattern Shape and Size}
In the previous sections, we studied the effect of automata shape and size on the performance. In this section, our focus is on pattern shape and size. Pattern shape and size will impact the number of total matchings and partial matching, hence impacting the execution time. In this section, we study this effect over the performance of our algorithm. For this experiment, we fixed the temporal constraint of the Temporal BGP to the automata in Figure~\ref{fig:inc-nfa}. Note that this automata has no clock, but as we showed before, the number of clocks would not have any effect on the overall performance.  Table~\ref{tab:diff-pattern} shows the total number of matchings, the number of accepted matchings at the end of temporal domain,  matching time, and the total execution time for different pattern shapes over our dataset. In this table, the matching time is measured by computing the matching using the most optimized join plan (join order) over each dataset using a non-incremental algorithm without running the timed automata. We tested our algorithms for paths and cycles with variant length 2 to 4. 

Table~\ref{tab:diff-pattern} shows, for  acylic patterns (e.g. paths), the partial matching  algorithm is significantly faster than on-demand and baseline algorithms. In acylic queries such as path, partial matchings are shared by many total matchings and larger size partial matchings, hence this algorithm reduces the computation time significantly. For cyclic patterns of size two and  three, the on-demand algorithm is the fastest option followed by baseline closely, but the partial matching shows a slower performance for this two patterns. For ``cycle4'' we can see that partial matching is the fastest algorithm.  In graphs there are much fewer closed cycles compared to possible open partial matchings and in smaller cycles this causes the partial matching algorithm to run slower. As the cycle sizes get larger, the performance of the partial matching algorithm will be comparable or faster than the other two algorithms. Another graph characteristic that can affect the partial match algorithm is the density of the graph, which we will discuss in the next section. Note that for EU-Email dataset the ``path4'' query and for FB-wall ``path4'' and ``cycle4'' query did not fit on our machine memory and we did not conducted experiments on those. 

The on-demand algorithm and the baseline algorithm in theory should have the same execution time. The time difference observed here can be caused by different join methods, different compiler optimization, or different memory allocation strategies. 




\begin{table}
\small 
\caption{Various Type of BGP / Exec Time using $\ta_0$ automatas over EPL, EU-email, Facebook-wall}
\label{tab:diff-pattern}
\begin{tabular}{lrrrrrr}

\textbf{EPL} & \multicolumn{2}{c|}{\# of matches} & \multicolumn{4}{c}{time (sec)} \\ \hline
\multicolumn{1}{l|}{pattern} & BGP & \multicolumn{1}{r|}{BGP + TA} & match & baseline & on-demand & partial \\ \hline
\multicolumn{1}{l|}{path2} & 47K & \multicolumn{1}{r|}{1.8K} & 0.01 & 0.22 & 0.19 & \textbf{0.06} \\
\multicolumn{1}{l|}{path3} & 1.5M & \multicolumn{1}{r|}{4.5K} & 0.21 & 5.23 & 5.15 & \textbf{0.20} \\
\multicolumn{1}{l|}{cycle2} & 1.1K & \multicolumn{1}{r|}{35} & 0.01 & \textbf{0.01} & \textbf{0.01} & 0.02 \\
\multicolumn{1}{l|}{cycle3} & 35K & \multicolumn{1}{r|}{56} & 0.02 & 0.12 & \textbf{0.09} & 0.36 \\
\multicolumn{1}{l|}{cycle4} & 1.1M & \multicolumn{1}{r|}{60} & 0.38 & 3.54 & 3.49 & \textbf{1.55} \\
 & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
\textbf{EU-email} & \multicolumn{2}{c|}{\# of matches} & \multicolumn{4}{c}{time (sec)} \\ \hline
\multicolumn{1}{l|}{pattern} & BGP & \multicolumn{1}{r|}{BGP + TA} & match & baseline & on-demand & partial \\ \hline
\multicolumn{1}{l|}{path2} & 862K & \multicolumn{1}{r|}{36K} & 0.25 & 59.76 & 63.14 & \textbf{17.54} \\
\multicolumn{1}{l|}{path3} & 42M & \multicolumn{1}{r|}{126K} & 41 & 2,126 & 1,732 & \textbf{224} \\
\multicolumn{1}{l|}{cycle2} & 18K & \multicolumn{1}{r|}{843} & 0.12 & \textbf{0.92} & 0.95 & 2.40 \\
\multicolumn{1}{l|}{cycle3} & 205K & \multicolumn{1}{r|}{309} & 0.19 & \textbf{16.85} & 17.28 & 17.65 \\
\multicolumn{1}{l|}{cycle4} & 8.4M & \multicolumn{1}{r|}{918} & 5 & 1,168 & 618 & \textbf{223} \\
 & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
\textbf{FB-wall} & \multicolumn{2}{c|}{\# of matches} & \multicolumn{4}{c}{time (sec)} \\ \hline
\multicolumn{1}{l|}{pattern} & BGP & \multicolumn{1}{r|}{BGP + TA} & match & baseline & on-demand & partial \\ \hline
\multicolumn{1}{l|}{path2} & 4.5M & \multicolumn{1}{r|}{618K} & 4 & 252 & 276 & \textbf{226} \\
\multicolumn{1}{l|}{path3} & 90M & \multicolumn{1}{r|}{235K} & 106 & 12,915 & 12,577 & \textbf{1,005} \\
\multicolumn{1}{l|}{cycle2} & 1.6M & \multicolumn{1}{r|}{16K} & 1 & 18 & \textbf{16} & 81 \\
\multicolumn{1}{l|}{cycle3} & 272K & \multicolumn{1}{r|}{4.7K} & 1 & \textbf{14} & 16 & 277
\end{tabular}
\end{table}






% \subsection{Throughput}
%\amir{I removed this section}
% \label{sec:throughput}
% One important aspect of on-line algorithm is throughput or turn around time, where we want to see how long users need to wait to see some results ready. This is important for temporal graphs that are small at the beginning of the graph history and exponentially grow over time.

% For this purpose, we selected a cycle of length 4 query over Eu-Email dataset and a path 4 query over EPL dataset. This two queries take significant time to finish and hence are good candidates for this experiment. The timed automata used in this experiment is the same as the one in Figure~\ref{fig:inc-nfa}


% Figure~\ref{fig:tput-snaps} shows the number of snapshots each algorithm processed in the first minute.  Accordingly  Figure~\ref{fig:tput-match} shows the number total matching passed through the timed-automata in the same first minute. As it can be seen, for the path-4 query, as expected, the partial matching algorithm has the highest throughput. One interesting observation here is that one-demand algorithm processed two times more snapshots than the baseline algorithm in the first two minutes, which translates to millions of more matchings. This happens because the baseline algorithm processes all existing matching each iteration, but the on-demand only processes the total matching that exists during the current time point. 

% Another interesting observation is that at which percentage of the total run-time which percent of matchings or snapshots have been processed by the timed automata. Figure~\ref{fig:tput-all-match} and Figure~\ref{fig:tput-all-snap} show this result. In this figures, the x-axis shows the total execution time of the longest running algorithm, which for cycle-4 on Eu-Email is the partial matching algorithm and for path-4 on EPL is on-demand algorithm. 
% The y-axis in Figure ~\ref{fig:tput-all-snap} shows which percentage of the graph snapshots have been processed and the y-axis in Figure ~\ref{fig:tput-all-matchi} shows which percentage of total matchings have been gone through the timed automata at least once.



% \begin{figure*}[!t]%
% \centering
% \subfloat[\# of Snapshots in a Minute ]{%
% \label{fig:tput-snaps}%
% \includegraphics[width=0.45\columnwidth]{figs/tput/chart-15.pdf}}
% \subfloat[\# of Matching in a Minute ]{%
% \label{fig:tput-match}%
% \includegraphics[width=0.45\columnwidth]{figs/tput/chart-16.pdf}}%%
% \subfloat[ \% of Snapshots]{%
% \label{fig:tput-all-snap}%
% \includegraphics[width=0.45\columnwidth]{figs/tput/chart-18.pdf}}
% \subfloat[ \% of Matching]{%
% \label{fig:tput-all-match}%
% \includegraphics[width=0.45\columnwidth]{figs/tput/chart-19.pdf}}

% \caption{System Throughput in One Minutes for rectangle over Eu-Email and path4 over EPL}
% \label{fig:tput}
% \vspace{-0.5cm}
% \end{figure*}



\subsection{Selectivity}
Trying different timed automatas in previous experiments showed us that there can be a relation between the number of accepted matchings and the execution time. To study this, we varied the clock condition in $\ta_2$ automata in Figure~\ref{fig:nfa-type-ta2} from $c < 2 $ to $c < 1024$. For a ``path2'' pattern in Eu-Email dataset, this clock range makes the automata accept zero matching for the smallest clock and 36K matching for the largest clock. 
Figure~\ref{fig:selectivity} shows the result of this experiment. Axis-x in this figure shows the number of matchings and axis-y shows the execution time in seconds. As it can be seen in this figure, increasing the number of accepted matchings increases the execution time, but the slope of this increase is small. 

\begin{figure}
	\centering
	\includegraphics[width=0.5\columnwidth]{figs/selectivity/chart-41.pdf}
    \caption{Output Size / Exec Time for Path2 pattern of Eu-Email for $\ta_2$ automata }
    \label{fig:selectivity}
\end{figure}



% \label{sec:ex:select}
% \begin{figure}[!t]%
% \centering
% \subfloat[Size of clock]{%
% %\label{fig:}%
% \includegraphics[width=0.5\columnwidth]{figs/selectivity/chart-41.pdf}}
% \subfloat[Number of Matching]{%
% \label{fig:clock}%
% \includegraphics[width=0.5\columnwidth]{figs/selectivity/chart-41.pdf}}%%
% \caption{Selectivity}
% \label{fig:selectivity}
% \vspace{-0.5cm}
% \end{figure}








==> fig5.tex <==
\begin{figure}[!h]
\centering
\small
% Please add the following Required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{tabular}{lllllll}
\multicolumn{4}{l}{\textbf{Node}} &  & \multicolumn{2}{l}{\textbf{Active}} \\ \cline{1-4} \cline{6-7} 
\multicolumn{2}{|l|}{\w{vid}} & \multicolumn{2}{l|}{\w{label}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{\w{eid}} & \multicolumn{1}{l|}{\w{time}} \\ \cline{1-4} \cline{6-7} 
\multicolumn{2}{|l|}{$v_1$}                                  & \multicolumn{2}{l|}{\emp}                                            & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{$e_1$}       & \multicolumn{1}{l|}{$1$}  \\ \cline{1-4} \cline{6-7} 
\multicolumn{2}{|l|}{$v_2$}                                  & \multicolumn{2}{l|}{\emp}                                            & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{$e_1$}       & \multicolumn{1}{l|}{3}    \\ \cline{1-4} \cline{6-7} 
\multicolumn{2}{|l|}{$v_3$}                                  & \multicolumn{2}{l|}{\emp}                                            & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{$e_2$}       & \multicolumn{1}{l|}{1.1}  \\ \cline{1-4} \cline{6-7} 
\multicolumn{2}{|l|}{$v_4$}                                  & \multicolumn{2}{l|}{\emp}                                            & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{$e_2$}       & \multicolumn{1}{l|}{1.9}  \\ \cline{1-4} \cline{6-7} 
\multicolumn{2}{|l|}{$v_5$}                                  & \multicolumn{2}{l|}{\cust}                                            & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{$e_3$}       & \multicolumn{1}{l|}{9}    \\ \cline{1-4} \cline{6-7} 
\multicolumn{2}{|l|}{$v_6$}                                  & \multicolumn{2}{l|}{\cust}                                            & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{$e_4$}       & \multicolumn{1}{l|}{1}    \\ \cline{1-4} \cline{6-7} 
\multicolumn{2}{|l|}{$v_7$}                                  & \multicolumn{2}{l|}{\cust}                                            & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{$e_5$}       & \multicolumn{1}{l|}{1}    \\ \cline{1-4} \cline{6-7} 
\multicolumn{2}{|l|}{$v_8$}                                  & \multicolumn{2}{l|}{\room}                                & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{$e_5$}       & \multicolumn{1}{l|}{3}    \\ \cline{1-4} \cline{6-7} 
                               &                             &                             &                                            & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{$e_5$}       & \multicolumn{1}{l|}{5}    \\ \cline{6-7} 
\multicolumn{4}{l}{\textbf{Edge}}                                                                                                       & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{$e_6$}       & \multicolumn{1}{l|}{2}    \\ \cline{1-4} \cline{6-7} 
\multicolumn{1}{|l|}{\w{eid}}      & \multicolumn{1}{l|}{\w{vid\_1}} & \multicolumn{1}{l|}{\w{vid\_2}} & \multicolumn{1}{l|}{\w{label}}                 & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{$e_6$}       & \multicolumn{1}{l|}{4}    \\ \cline{1-4} \cline{6-7} 
\multicolumn{1}{|l|}{$e_1$}    & \multicolumn{1}{l|}{$v_1$}  & \multicolumn{1}{l|}{$v_2$}  & \multicolumn{1}{l|}{\msg}               & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{$e_6$}       & \multicolumn{1}{l|}{6}    \\ \cline{1-4} \cline{6-7} 
\multicolumn{1}{|l|}{$e_2$}    & \multicolumn{1}{l|}{$v_1$}  & \multicolumn{1}{l|}{$v_3$}  & \multicolumn{1}{l|}{\msg}               & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{$e_7$}       & \multicolumn{1}{l|}{2}    \\ \cline{1-4} \cline{6-7} 
\multicolumn{1}{|l|}{$e_3$}    & \multicolumn{1}{l|}{$v_2$}  & \multicolumn{1}{l|}{$v_4$}  & \multicolumn{1}{l|}{\msg}               & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{$e_8$}       & \multicolumn{1}{l|}{2}    \\ \cline{1-4} \cline{6-7} 
\multicolumn{1}{|l|}{$e_4$}    & \multicolumn{1}{l|}{$v_3$}  & \multicolumn{1}{l|}{$v_4$}  & \multicolumn{1}{l|}{\msg}               & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{$e_8$}       & \multicolumn{1}{l|}{3}    \\ \cline{1-4} \cline{6-7} 
\dots &  &  &  &  & \dots &  \\ \cline{1-4} \cline{6-7} 
\multicolumn{1}{|l|}{$e_{11}$} & \multicolumn{1}{l|}{$v_2$}  & \multicolumn{1}{l|}{$v_8$}  & \multicolumn{1}{l|}{\visit} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{$e_{12}$} & \multicolumn{1}{l|}{2}    \\ \cline{1-4} \cline{6-7} 
\multicolumn{1}{|l|}{$e_{12}$} & \multicolumn{1}{l|}{$v_4$}  & \multicolumn{1}{l|}{$v_8$}  & \multicolumn{1}{l|}{\visit} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{$e_{12}$} & \multicolumn{1}{l|}{4}    \\ \cline{1-4} \cline{6-7} 
\end{tabular}
\caption{Representation of a temporal graph $H$ as relations $\it Node$, $\it Edge$ and $\it Active$ for the temporal graph in Figure~\ref{fig:def2}.}
\label{fig:h-rep}
\end{figure}

==> figs/automata_experiments_old.tex <==
\begin{figure*}%
\centering
\subfloat[TA1: Alternation]{
\label{fig:nfa-type-ta1}%
 \begin{tikzpicture}[->, on grid, node distance=42pt]
    \node[state, initial, accepting] (s0) {$s_0$};
    \node[state, right of=s0] (s1) {$s_1$};
    \draw (s0)
  (s1) edge[loop above] node{$\emptyset$} (s1)
  (s0) edge[loop above] node{$\emptyset$} (s0)
  (s0) edge[above, bend left] node{$y_1 \land \neg y_2$} (s1)
  (s0) edge[above, bend left] node{$y_1 \land \neg y_2$} (s1)
  (s1) edge[below, bend left] node{$y_2 \land \neg y_1$} (s0);
    \end{tikzpicture}
}\hspace{.01em}%
\subfloat[TA2: Alternation with Clock]{%
\label{fig:nfa-type-ta2}%
        \begin{tikzpicture}[->, on grid, node distance=72pt]
                \node[state, initial, accepting] (s0) {$s_0$};
                \node[state, accepting, right of=s0] (s1) {$s_1$};
                \draw
                (s0) edge[bend left] node[above]{$y_1 \land \neg y_2 \land \xx < 3$} node[below] {$\xx:=0$} (s1)
                     (s1) edge[loop above] node{$\emptyset$} (s1)
                      (s0) edge[loop above] node{$\emptyset$} (s0)
                (s1) edge[bend left] node[below]{$y_2 \land \neg y_1 \land \xx < 3$}
                node[above] {$\xx:=0$}(s0);
        \end{tikzpicture}}%
\subfloat[TA3: Ordered Constraint]{%
\label{fig:nfa-type-ta3}%
        \begin{tikzpicture}[->, on grid, node distance=40pt]
        \node[state, initial] (s0) {$s_0$};
        \node[state, right of=s0] (s1) {$s_1$};
        \node[state, accepting, right of=s1] (s2) {$s_2$};
        \draw (s0) edge[loop above] node{$\mathit{\emptyset}$} (s0)
      (s0) edge[above] node{$\{y_1\}$}  (s1)
      (s1) edge[loop above] node{$\mathit{\emptyset}$} (s1)
      (s1) edge[above] node{$\{y_2\}$} (s2);
        \end{tikzpicture}
}
\caption{Timed automata used in experimental evaluation}
\label{fig:nfa-type}
\vspace{-0.5cm}
\end{figure*}

\begin{figure}
 \resizebox{0.8\columnwidth}{!}{
 \begin{tikzpicture}[->, on grid, node distance=50pt]
    \node[state, initial] (s0) {$s_0$};
    \node[state, right of=s0,accepting] (s1) {$s_1$};
    \node[state, right of=s1,accepting] (s2) {$\dots$};
    \node[state, right of=s2,accepting] (s3) {$s_m$};
    \draw (s0)
%   (s0) edge[loop above] node{$\bigwedge_{_{i=1,\dots,m}} ^{\neg y_i}   $} (s0)
%   (s1) edge[loop above] node{$\bigwedge_{_{i=1,\dots,m}} ^{\neg y_i}   $} (s1)
%   (s2) edge[loop above] node{$\bigwedge_{_{i=1,\dots,m}} ^{\neg y_i}   $} (s2)
%   (s3) edge[loop above] node{$\bigwedge_{_{i=1,\dots,m}} ^{\neg y_i}   $} (s3)
 (s0) edge[loop above] node{$\emptyset   $} (s0)
  (s1) edge[loop above] node{$\emptyset $} (s1)
  (s2) edge[loop above] node{$\emptyset$} (s2)
  (s3) edge[loop above] node{$\emptyset$} (s3)

  (s0) edge[above] node{$\{y_1\}$} (s1)
  (s1) edge[above] node{$\dots$} (s2)
  (s2) edge[above] node{$\{y_{m-1}\}$} (s3)
  (s3) edge[below, bend left] node{$\{y_m\} $} (s0);
    \end{tikzpicture}
    }
    \caption{$TA_0$ generalizes $TA_1$: Incremental Order Constraint }
    \label{fig:inc-nfa}
\end{figure}

\begin{figure}
 \resizebox{0.8\columnwidth}{!}{
 \begin{tikzpicture}[->, on grid, node distance=50pt]
    \node[state, initial] (s0) {$s_0$};
    \node[state, right of=s0,accepting] (s1) {$s_1$};
    \node[state, right of=s1,accepting] (s2) {$s_2$};
    \node[state, right of=s2,accepting] (s3) {$s_3$};
    \draw (s0)
  (s0) edge[loop above] node{$\emptyset$} (s0)
  (s1) edge[loop above] node{$\emptyset$} (s1)
  (s2) edge[loop above] node{$\emptyset$} (s2)
  (s3) edge[loop above] node{$\mathit{true}$} (s3)

  (s0) edge[above] node{$\{y_1\}$} (s1)
  (s0) edge[below, bend right] node{$y_1 \land y_2  \land \neg y_3$} (s2)
  (s0) edge[below, bend right = 50] node{$y_1 \land y_2 \land y_3$} (s3)
  (s1) edge[below, bend right] node{$y_2 \land y_3$} (s3)
  (s1) edge[above] node{$\{y_2\}$} (s2)
  (s2) edge[above] node{$\{y_3\}$} (s3);
    \end{tikzpicture}
    }
    \caption{$TA_4$ All Accepting NFA of Size 3}
\label{fig:all-nfa}
\end{figure}

==> figs/data_pivot.tex <==
\begin{table}
\caption{Temporal graph datasets used for evaluation.}  
\label{tab:datasets}
\centering
\small 
\begin{tabular}{lcccccc}
 & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{2}{c}{\textbf{density}} \\ \hline
\multicolumn{1}{|l|}{} & \multicolumn{1}{c|}{\textbf{\# nodes}} & \multicolumn{1}{c|}{\textbf{\# edges}} & \multicolumn{1}{c|}{\textbf{\# active edges}} & \multicolumn{1}{c|}{\textbf{\# snaps}} & \multicolumn{1}{c|}{\textbf{structural}} & \multicolumn{1}{c|}{\textbf{temporal}} \\ \hline
\multicolumn{1}{|l|}{\textbf{EPL}} & \multicolumn{1}{c|}{50} & \multicolumn{1}{c|}{1500} & \multicolumn{1}{c|}{35K} & \multicolumn{1}{c|}{25} & \multicolumn{1}{c|}{0.6} & \multicolumn{1}{c|}{0.93} \\ \hline
\multicolumn{1}{|l|}{\textbf{Eu-Email}} & \multicolumn{1}{c|}{776} & \multicolumn{1}{c|}{65K} & \multicolumn{1}{c|}{1.9M} & \multicolumn{1}{c|}{800} & \multicolumn{1}{c|}{0.1} & \multicolumn{1}{c|}{0.03} \\ \hline
\multicolumn{1}{|l|}{\textbf{FB-Wall}} & \multicolumn{1}{c|}{46K} & \multicolumn{1}{c|}{264K} & \multicolumn{1}{c|}{856K} & \multicolumn{1}{c|}{1500} & \multicolumn{1}{c|}{0.0001} & \multicolumn{1}{c|}{0.002} \\ \hline
\end{tabular}
%\vspace{+0.2cm}
\end{table}

\begin{table}
\small 
\caption{Summary of experimental datasets.}
\label{tab:data}
\begin{tabular}{lrrrrrr}

\textbf{EPL} & \multicolumn{2}{c|}{\# of matches} & \multicolumn{4}{c}{time (sec)} \\ \hline
\multicolumn{1}{l|}{pattern} & BGP & \multicolumn{1}{r|}{BGP + TA} & match & baseline & on-demand & partial \\ \hline
\multicolumn{1}{l|}{path2} & 47K & \multicolumn{1}{r|}{1.8K} & 0.01 & 0.22 & 0.19 & \textbf{0.06} \\
\multicolumn{1}{l|}{path3} & 1.5M & \multicolumn{1}{r|}{4.5K} & 0.21 & 5.23 & 5.15 & \textbf{0.20} \\
\multicolumn{1}{l|}{cycle2} & 1.1K & \multicolumn{1}{r|}{35} & 0.01 & \textbf{0.01} & \textbf{0.01} & 0.02 \\
\multicolumn{1}{l|}{cycle3} & 35K & \multicolumn{1}{r|}{56} & 0.02 & 0.12 & \textbf{0.09} & 0.36 \\
\multicolumn{1}{l|}{cycle4} & 1.1M & \multicolumn{1}{r|}{60} & 0.38 & 3.54 & 3.49 & \textbf{1.55} \\
 & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
\textbf{EU-email} & \multicolumn{2}{c|}{\# of matches} & \multicolumn{4}{c}{time (sec)} \\ \hline
\multicolumn{1}{l|}{pattern} & BGP & \multicolumn{1}{r|}{BGP + TA} & match & baseline & on-demand & partial \\ \hline
\multicolumn{1}{l|}{path2} & 862K & \multicolumn{1}{r|}{36K} & 0.25 & 59.76 & 63.14 & \textbf{17.54} \\
\multicolumn{1}{l|}{path3} & 42M & \multicolumn{1}{r|}{126K} & 41 & 2,126 & 1,732 & \textbf{224} \\
\multicolumn{1}{l|}{cycle2} & 18K & \multicolumn{1}{r|}{843} & 0.12 & \textbf{0.92} & 0.95 & 2.40 \\
\multicolumn{1}{l|}{cycle3} & 205K & \multicolumn{1}{r|}{309} & 0.19 & \textbf{16.85} & 17.28 & 17.65 \\
\multicolumn{1}{l|}{cycle4} & 8.4M & \multicolumn{1}{r|}{918} & 5 & 1,168 & 618 & \textbf{223} \\
 & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
\textbf{FB-wall} & \multicolumn{2}{c|}{\# of matches} & \multicolumn{4}{c}{time (sec)} \\ \hline
\multicolumn{1}{l|}{pattern} & BGP & \multicolumn{1}{r|}{BGP + TA} & match & baseline & on-demand & partial \\ \hline
\multicolumn{1}{l|}{path2} & 4.5M & \multicolumn{1}{r|}{618K} & 4 & 252 & 276 & \textbf{226} \\
\multicolumn{1}{l|}{path3} & 90M & \multicolumn{1}{r|}{235K} & 106 & 12,915 & 12,577 & \textbf{1,005} \\
\multicolumn{1}{l|}{cycle2} & 1.6M & \multicolumn{1}{r|}{16K} & 1 & 18 & \textbf{16} & 81 \\
\multicolumn{1}{l|}{cycle3} & 272K & \multicolumn{1}{r|}{4.7K} & 1 & \textbf{14} & 16 & 277
\end{tabular}
\end{table}

==> intro.tex <==
\section{Introduction}
\label{sec:intro}

% We combine traditional BGP processing with event processing.
% This is why we use timed automata.
% Add lots of examples that are hard to represent in SQL.
% Add anecdotal experimental results comparing with SQL.

Graph pattern matching, the problem of finding instances of one
graph in a larger graph, has been extensively studied since the
1970s, and numerous algorithms have been
proposed~\cite{conte2004thirty, cheng2008fast,
ullmann1976algorithm, reza2020approximate, fan2010graph,
lai2019distributed}.  Initially, work in this area focused on
static graphs, in which information about changes in the graph is
not recorded.  Finding patterns in static graphs can be helpful
for many important tasks, such as finding mutual interests among
users in a social network.  However, understanding how interests
of social network users evolve over time, support for contact
tracing, and many other research questions and applications
require access to information about how a graph changes over
time.  Consequently, the focus of research has moved to
pattern matching in \emph{temporal graphs} for tasks
such as finding temporal motifs, temporal journeys, and temporal
shortest
paths~\cite{DBLP:journals/corr/abs-1107-5646,DBLP:conf/sigmod/GurukarRR15,DBLP:conf/wsdm/ParanjapeBL17,semertzidis2016durable,xu2017time,rost2021distributed,DBLP:conf/edbt/ZufleREF18}.   

%However, using static graphs for other tasks such as contact tracing will likely produce inaccurate results. Due to the shortcoming of static graphs during the past few years, researchers started focusing on graph matching in temporal graphs for tasks such as finding temporal motifs, temporal journeys, and temporal shortest paths .~\cite{DBLP:journals/corr/abs-1107-5646,DBLP:conf/sigmod/GurukarRR15,DBLP:conf/wsdm/ParanjapeBL17,semertzidis2016durable,xu2017time,rost2021distributed,DBLP:conf/edbt/ZufleREF18}. 

In this paper, we will elaborate on how temporal information can
add to the significance of graph patterns, and will describe
different types of \emph{temporal constraints} that can be stated
over such graphs.  Figure~\ref{fig:def2} gives our running
example, showing a interaction graph, where each node
represents a person, either an \emph{employee} (node label \emp)
or a \emph{customer} (node label \cust) or represent an \emph{office}(node label \room), and each edge represents either
email \emph{messages}  (edge label \msg) or a \emph{visit}(edge label \visit) from a source node to a target node. Each edge is associated with the set of timepoints when an interaction have occurred.  Graphs with static nodes but dynamic edges that are active at multiple timepoints are commonly used to represent interaction networks~\cite{zhao2010Comm, DBLP:conf/wsdm/ParanjapeBL17}. %We start with an example in which temporal information can be useful for analysis.

%\julia{Need to typeset labels differently here and in the text, hard to read.}




\begin{figure}
  \centering
   \resizebox{\columnwidth}{!}{
    \begin{tikzpicture}[on grid, node distance=80pt,auto]
      \node[state,minimum size= 10pt, node distance=80pt]   (v1)                     {$v_1$:\emp};
      \node[state,minimum size= 10pt, node distance=80pt]   (v2) [above right=of v1] {$v_2$:\emp};
      \node[state,minimum size= 10pt, node distance=80pt]   (v3) [below right=of v1] {$v_3$:\emp};
      \node[state,minimum size= 10pt, node distance=80pt]   (v5) [above left=of v1]   {$v_5$:\cust};
      \node[state,minimum size= 10pt, node distance=110pt]  (v6) [left=of v1]        {$v_6$:\cust};
      \node[state,minimum size= 10pt, node distance=90pt]   (v7) [below left=of v1]  {$v_7$:\cust};
      
      \node[state,minimum size= 10pt, node distance=70pt]   (v8) [right =of v2] {$v_8$:\room};
      \node[state,minimum size= 10pt, node distance=80pt]   (v4) [below =of v8] {$v_4$:\emp};


      
    \path[->] 
     (v1) edge  node [sloped,above] {$e_1$:\msg} node[sloped,below]{\small{$T=\{1,3\}$}} (v2)
     (v1) edge  node [sloped,above] {$e_2$:\msg} node[sloped,below]{\small{$T=\{1.1,1.9\}$}} (v3)
     (v2) edge  node [sloped,above] {$e_3$:\msg} node[sloped,below]{\small{$T=\{1,3\}$}} (v4)
     (v3) edge  node [sloped,above] {$e_4$:\msg} node[sloped,below]{\small{$T=\{1\}$}} (v4)
    
     (v5) edge [bend  left=25] node [sloped,above] {$e_5$:\msg} node[sloped,below]{\small{$T=\{1,3,5\}$}} (v1)
     (v1) edge [bend  left=25] node [sloped,above] {$e_6$:\msg} node[sloped,below]{\small{$T=\{2,4,6\}$}} (v5)
     
     (v2) edge node [sloped,above] {$e_{10}$:\msg} node[sloped,below]{\small{$T=\{2,4,6\}$}} (v3)
     
     (v6) edge  node [sloped,above] {$e_7$:\msg} node[sloped,below]{\small{$T=\{2\}$}} (v1)

     (v7) edge [bend  left=25] node [sloped,above] {$e_8$:\msg} node[sloped,below]{\small{$T=\{2,3,4\}$}} (v1)
     (v1) edge [bend  left=25] node [sloped,above] {$e_9$:\msg} node[sloped,below]{\small{$T=\{9\}$}} (v7)
     
     (v2) edge  node [sloped,above] {$e_{11}$:\visit} node[sloped,below]{\small{$T=\{1,3,6\}$}} (v8)
     (v4) edge  node [sloped,above] {$e_{12}$:\visit} node[sloped,below]{\small{$T=\{2,4\}$}} (v8)

    ;
    %             (v2) edge                node [above] {$e_3$:m} node[below]{\small{$T=\{1.7,2,3.5,6,8\}$}}(v3);
    \end{tikzpicture}
    }
  \caption{An example of a temporal graph: a labeled graph with
  nodes $v_1$--$v_4$ of type employee (\emp), nodes $v_5$--$v_7$
  of type customer (\cust), node $v_8$ type office(\room) ,edges $e_1$--$e_{10}$ of type
  message (\msg) and edges $e_{11} and e_{12}$ of type visit(\visit).  Each edge is associated with the set of timepoints during which that edge was active. \amir{I change the example by adding v8 and e11 and e12 as}}
  \label{fig:def2}
\end{figure}
 
 \begin{figure*}[t!]
    \centering
    \subfloat[BGP cycle of length 2]{
    \label{fig:bgp-cycle2:bgp}%
        \begin{tikzpicture}[->, on grid, node distance=50pt]
            \node[state ] (x) {$x_1:\cust$};
            \node[state, right of=x] (y) {$x_2:\emp$};
            \draw
            (x) edge[bend left] node[above]{$y_1$} (y)
            (y) edge[bend left] node[below]{$y_2$} (x);
         \end{tikzpicture}
     }
    \qquad
      \subfloat[timed automaton $\ta_1$]{
      \label{fig:bgp-cycle2:ta1}
        \begin{tikzpicture}[->, on grid, node distance=40pt]
                \node[state, initial, accepting] (s0) {$s_0$};
                \node[state, accepting, right of=s0] (s1) {$s_1$};
                \draw
                (s0) edge[bend left] node[above]{$\{y_1\} $} (s1)
                      (s1) edge[loop above] node{$\emptyset$} (s1)
                      (s0) edge[loop above] node{$\emptyset$} (s0)

                (s1) edge[bend left] node[below]{$\{y_2\} $}
                (s0);
        \end{tikzpicture}
        }
        \qquad
        \subfloat[timed automaton $\ta_2$]{
        \label{fig:bgp-cycle2:ta2}
        \begin{tikzpicture}[->, on grid, node distance=60pt]
                \node[state, initial, accepting] (s0) {$s_0$};
                \node[state, accepting, right of=s0] (s1) {$s_1$};
                \draw
                (s0) edge[bend left] node[above]{$\{y_1\} \land \xx < 3$} node[below] {$\xx:=0$} (s1)
                     (s1) edge[loop above] node{$\emptyset$} (s1)
                      (s0) edge[loop above] node{$\emptyset$} (s0)
                (s1) edge[bend left] node[below]{$\{y_2\} \land \xx < 3$}
                node[above] {$\xx:=0$}(s0);
        \end{tikzpicture}
        }
        \subfloat[timed automaton $\ta_3$]{%
            \label{fig:nfa-type-ta3}%
        \begin{tikzpicture}[->, on grid, node distance=40pt]
                \node[state, initial] (s0) {$s_0$};
                \node[state, right of=s0] (s1) {$s_1$};
                \node[state, accepting, right of=s1] (s2) {$s_2$};
                \draw (s0) edge[loop above] node{$\mathit{\emptyset}$} (s0)
              (s0) edge[above] node{$\{y_1\}$}  (s1)
              (s1) edge[loop above] node{$\mathit{\emptyset}$} (s1)
              (s1) edge[above] node{$\{y_2\}$} (s2)
              (s2) edge[loop above] node{$\mathit{true}$} (s2);
;
        \end{tikzpicture}
}


\caption{Temporal BGP that identifies (a) cycles of length two, with three alternative temporal constraints, specified by timed automata: (b) $\ta_1$: edges are observed in strict temporal alternation; (c) $\ta_2$: edges are observed in strict temporal alternation, with fewer than 3 time units passing between observations; (d)  $\ta_3$: edges are observed in strict temporal order. \julia{explain notation better}}
    \label{fig:bgp-cycle2}
\end{figure*}


 \begin{figure*}[t!]
    \centering
    % \subfloat[BGP Star of length 2 ]{
    % \label{fig:bgp-star2:bgp}%
    %     \begin{tikzpicture}[->, on grid, node distance=40pt]
    %     \node[state,minimum size= 10pt]   (v1) {$x_1$:\room};
    %   \node[state,minimum size= 10pt]   (v2) [right=of v1] {$x_2$:\emp};
    %   \node[state,minimum size= 10pt]   (v3) [left=of v1]  {$x_3$:\emp};
    %     \draw 
    %         (v2) edge[right] node[above]{$y_1$} (v1)
    %          (v3) edge[right] node[above]{$y_2$} (v1);
    %     \end{tikzpicture}
    %  }
    %      \qquad
    \subfloat[timed automaton $\ta_5$]{
    \label{fig:ta5}%
        \begin{tikzpicture}[->, on grid, node distance=40pt]
                \node[state, initial, accepting] (s0) {$s_0$};
                \draw
  (s0) edge[loop above] node{$\emptyset \lor (y_1 \land y_2) $} (s0);
        \end{tikzpicture}
     }
    \qquad
      \subfloat[timed automaton $\ta_6$]{
      \label{fig:ta6}
        \begin{tikzpicture}[->, on grid, node distance=40pt]
                \node[state, initial, accepting] (s0) {$s_0$};
                \draw
  (s0) edge[loop above] node{$\emptyset \lor ({y_1} \oplus {y_2} ) $} (s0);
        \end{tikzpicture}
        }
        \qquad
        \subfloat[timed automaton $\ta_7$]{
        \label{fig:ta7}
        \begin{tikzpicture}[->, on grid, node distance=50pt]
                \node[state, initial] (s0) {$s_0$};
                \node[state, right of=s0] (s1) {$s_1$};
                \node[node distance=65pt,state, accepting, right of=s1] (s2) {$s_2$};
                \draw
                (s0) edge[left] node[above]{${y_1} \land {y_2}$} node[below] {$\xx:=0$} (s1)
                (s0) edge[loop above] node{$\mathit{true}$} (s0)
                (s1) edge[loop above] node{${y_1} \land {y_2}$} (s1)
                % (s1) edge[left] node[above]{$(\emptyset \lor ({y_1} \oplus {y_2})) \land \xx > 3 $}  (s2)
                
                (s1) edge[left] node[above]{$\mathit{true} \land \xx > 3 $}  (s2)
                
                (s2) edge[loop above] node{$\mathit{true}$} (s2)
                ;
        \end{tikzpicture}
        }
                  \subfloat[TA8 .\amir{The subset query that we talked about in email, the s0->s1 edge can be removed }]{
    \label{fig:ta8}%
        \begin{tikzpicture}[->, on grid, node distance=60pt]
        \node[state,accepting]   (s0)                     {$s_0$};
      \node[state]   (s1) [right=of s0] {$s_1$};
        \draw 
            (s0) edge[loop above] node{$\neg y_1 \lor y_2$} (s0)
            (s0) edge[right] node[above]{$y_1 \land \neg y_2$} (s1);
        \end{tikzpicture}
     }
        
            \caption{Four alternative temporal constraints, specified by timed automata: (a) $\ta_5$: edges are observed always at the same time; (b) $\ta_6$: edges are observed never at the same time; (c)  $\ta_7$: edges are observed at the same time for at least 3 consecutive time points, (d)$\ta_8$: times  $y_1$ is observed is a subset of times $y_2$ is observed \julia{explain notation better} }
        \label{fig:bgp-star2}
        
        

\end{figure*}



%\amir{ added the labels : figure label~\ref{fig:bgp-cycle2:bgp} and label~\ref{fig:bgp-cycle2:ta1}}

\begin{example}
\label{ex:exist-const}
 Consider the temporal graph shown in Figure~\ref{fig:def2} that
 represents message exchanges between customers and employees of
 a publicly traded company. Suppose that employee $v_1$ shared
 confidential information with their colleagues $v_2$ and $v_3$, and that one of them subsequently shared this information with customer $v_4$, potentially constituting insider trading. Assuming that we have no access to the content of the messages, only to when they were sent, can we identify employees who may have leaked confidential information to $v_4$?
 
 Based on graph topology alone, both $v_2$ and $v_3$ could have been the source of the information leak to $v_4$.  However, by considering the timepoints on the edges, we  observe that there is no path from $v_1$ to $v_4$ that goes through $v_3$ and visits the nodes in temporal order.  We will represent this scenario with the following basic graph pattern (BGP), augmented with a temporal constraint:  $$\mathsf{v_1} \xrightarrow{y_1} x\xrightarrow{y_2} \mathsf{v_4}: \exists t_1 \in y_1.T, \exists t_2 \in y_2.T:  t_1 \leq t_2$$
 
Here, $\mathsf{v_1}$ and $\mathsf{v_4}$ are node constants, $x$
is a node variable, $y_1$ and $y_2$ are edge variables, and
$y_1.T$ and $y_2.T$ refer to the sets of timepoints associated
with edges $y_1$ and $y_2$.  The temporal
constraint states that there must exist a pair of timepoints
$t_1$, associated with edge $y_1$, and $t_2$, associated with
edge $y_2$, such that $t_1$ occurs before $t_2$.   We refer to
these types of patterns as \emph{temporal BGPs}. %, and to these types of temporal constraints as existential constraints.
\end{example}
 
In the remainder of this paper, we will formally present the semantics of temporal BGPs and  develop algorithms for evaluating them over large temporal graphs.  While particular kinds of temporal BGPs have been studied in the past~\cite{DBLP:conf/sigmod/GurukarRR15,DBLP:conf/wsdm/ParanjapeBL17,semertzidis2016durable,xu2017time,DBLP:conf/edbt/ZufleREF18}, as we will discuss in Section~\ref{sec:related}, a distinguishing feature of our approach is the use of \emph{timed automata}~\cite{timed-automata} to represent a rich class of temporal constraints, % study the complexity of their evaluation, 
and serve as basis for novel and practical algorithmic techniques. We now introduce timed automata as a means to express temporal constraints in graphs.
 
 %More formally, we can express a problem such as this, as a path pattern with a length equal to two, with a temporal order over edges. 
 
 %Example~\ref{ex:exist-const} shows a case where we are looking for a path of length two, where the first edge in the path exists before or at the same time as the second edge. 
%\begin{example}
%\label{ex:exist-const}
%Path of length two, where the first edge exists at time $t_1$ and second edge exists at time $t_2$, and $t_1 \leq t_2$. % and $t_2 - t_1 \leq 2$ 
%$$a \xrightarrow{e_i} b \xrightarrow{e_j}: e_i.t \leq e_j.t$$. 

%\begin{figure}[h!]
%    \centering
%    \begin{center}
%    \begin{tikzpicture}[->, on grid, node distance=60pt]
%    \node[state ] (a) {$x_1$};
%    \node[state, right of=a] (b) {$x_2$};
%     \node[state, right of=b] (c) {$x_3$};
%    \draw
%    (a) edge[left] node[above]{$y_1$} (b)
%    (b) edge[left] node[above]{$y_2$} (c);
%    \end{tikzpicture}
%    \end{center}    
%\caption{Path of Length 2}
%    \label{fig:bgp-path}
%\end{figure}


%$$x_1 \xrightarrow{y_1} x_2 \xrightarrow{y_2} x_3: \exists t_1 \in y_1.T \exists t_2 \in y_2.T:  t_1 \leq t_2$$
%\end{example}

% This type of temporal patterns, where we are assigning a temporal order to the edges, have been previously studied by researchers before\cite{DBLP:conf/sigmod/GurukarRR15,DBLP:conf/wsdm/ParanjapeBL17,semertzidis2016durable,xu2017time,DBLP:conf/edbt/ZufleREF18}. This kind of constraints can be expressed by comparison operators in SQL queries or Cypher queries~\cite{cypher}. For models where temporal information has been recorded as intervals, using Allen's interval algebra~\cite{allen1983maintaining} has also been utilized by researchers to specify a temporal constraint~\cite{xu2017time,rost2021distributed}. In this work, we call constraints such as the one above ``existential constraints''.  


%Not all temporal constraints can be described as a simple order over the edges of a pattern. As it can be seen in the graph in Figure~\ref{fig:def2} edge can reoccur many times, and this recurrence can be part of a temporal pattern.  Examples~\ref{ex:complex-const1} shows one case of such constraints in our toy graph in Figure~\ref{fig:def2}. 

\begin{example}
\label{ex:complex-const1}
Consider the temporal graph in Figure~\ref{fig:def2} and suppose that we are looking for customer-employee pairs who exchanged messages in strict alternation: the customer sent an email first, the employee replied, the customer replied again, and so on. We can express such patterns with the BGP in Figure~\ref{fig:bgp-cycle2:bgp}, with node variables $x_1$ of type customer and $x_2$ of type employee, and edge variables $y_1$ and $y_2$ that represent the email messages exchanged by $x_1$ and $x_2$. To concisely represent temporal alternation, we will use a two-state timed automaton $\ta_1$, shown in Figure~\ref{fig:bgp-cycle2:ta1}, with $s_0$ as the start state, and both $s_0$ and $s_1$ as accepting states.  State transitions are labeled with Boolean expressions over the existence of edge variables $y_1$ and $y_2$ at a particular timepoint.  For example, the edge transition from $s_0$ to $s_1$ is valid when only $y_1$ is observed (and $y_2$ is not), meaning that $x_1$ sent a message to $x_2$ but $x_2$ did not send a message to $x_1$ at that same timepoint.

The graph in Figure~\ref{fig:def2} contains two cycles of length two connecting a customer and an employee, and thus matching the structural portion of the temporal BGP in Figure~\ref{fig:bgp-cycle2:bgp}: the cycle containing $v_5$ and $v_1$, and that containing $v_7$ and $v_1$.  Of these, only the former meets the temporal constraint specified by $\ta_1$.

%matches for the structural portion of the BGP, $(e_5,e_6)$ and $(e_8,e_9)$, but only the latter also satisfies the temporal constraint. 

% \begin{figure}[h!]
%     \centering
%     \begin{center}
%     \begin{tikzpicture}[->, on grid, node distance=60pt]
%     \node[state ] (x) {$x_1:c$};
%     \node[state, right of=x] (y) {$x_2:e$};
%     \draw
%     (x) edge[bend left] node[above]{$y_1$} (y)
%     (y) edge[bend left] node[below]{$y_2$} (x);
%     \end{tikzpicture}

%     \end{center}    
% \caption{Cycle of length 2}
%     \label{fig:bgp-cycle2}
% \end{figure}

% \end{example}
\end{example}

Temporal re-occurrence of edges can be observed in numerous real graphs, and being able to identify this pattern is useful in real-life applications. For example, in fraud detection, a single transaction between suspicious clients may have no significance, but multiple transactions between two or more suspicious users during a short period of time can be a red flag. % In sports, teams compete with each other in fixed periods (\eg every season), using temporal constrains over re-occurrence of edges can be use in sport betting and sport analysis. In communication networks, users send multiple messages to each other; for instance, in social networks, users tend to send their friends messages every year during that friend's birthday week~\cite{DBLP:conf/sigmod/GurukarRR15}. Detecting re-occurring alternation such as the one in Example~\ref{ex:complex-const2} can be useful for quality assurance task for a customer support of a company.  In a collaboration graph such as DBLP, authors tend to collaborate with each other more than once~\cite{DBLP:conf/sigmod/AghasadeghiS18} which can be useful to . \todo{come up with better explanation for this example } %When we have recurrences of edges in temporal patterns, the constraints need to be expressed over multiple time points in the history of the edges.  Expressing such constraints as the one in Example~\ref{ex:complex-const1} will not be easy, if not impossible, in existing query languages such as SQL or Cypher~\cite{cypher}. To the best of our knowledge, this type of constraint has not previously been studied. 
%\amir{I added the timed automata to the Example~\ref{ex:complex-const1} and added another example with a clock in it ad Example~\ref{ex:complex-const2}. This two example can be merged but I left it as two example for now}
%
We will illustrate another feature of timed automata --- their use of clocks --- in our final motivating example.
\begin{example}
\label{ex:complex-const2}
Consider again the BGP in Figure~\ref{fig:bgp-cycle2:bgp}, discussed in Example~\ref{ex:complex-const1}, and suppose that we are looking for alternating messages that were sent in quick succession, with fewer than 3 time units passing between subsequent messages in an exchange.  We will express this additional requirement by augmenting the timed automaton $\ta_1$ with a \emph{clock} $\xx$ to specify that the \emph{temporal gap} between subsequent edges should  be less than 3 time units.  The resulting automaton is $\ta_2$, shown in Figure~\ref{fig:bgp-cycle2:ta2}.
\end{example}

\begin{example}
\label{ex:complex-contact}
\amir{I added this new example}
Suppose that we are looking for employees who share an office. The BGP $x_2:\emp \xrightarrow {y_1:\visit} x_1:\room \xleftarrow{y_2:\visit} x_3:\emp $ . In the graph represented in Figure~\ref{fig:def2}, nodes $v_2$ and $v_4$ share the office $v_8$. Due to pandemic restrictions or for resource management purposes, the company might want to find every two people who used the same office at the same time which can be represented by $\ta_5$ in Figure~\ref{fig:ta5}, or alternatively they can be interested in every office that have been used by not more than one employee at any instances which can be represented by the $\ta_6$ in Figure~\ref{fig:ta6}. Note that while $\ta_5$ and $\ta_6$ have similar structure, the difference between the condition on the timed-automaton edge created opposite constraints. Another possible use case can be when an employee tested positive for COVID and they want to find all the instances where another employee shared an office with the positive employee for more than 3 time points which can be represented by $\ta_7$ in Figure~\ref{fig:ta7}. Another possible constraints can be when we are interested in cases when $y_1$ is a subset of $y_2$ (e.g. $x_3$ is positive and we want to make sure $x_2$ never shared an office with them, or for a recomender system)
\end{example} 

We will formally present timed automata and will show that they
provide a general method for expressing a variety of useful
temporal constraints.  For example, as we will see in Section~\ref{sec:automata}, the existential constraint of Example~\ref{ex:exist-const} is also easily expressed by a timed automaton. 
Timed automata are a proven and expressive tool in the
verification of real-time systems \cite{timed-automata-survey}.
As we will discuss in Section~\ref{sec:related}, all types of temporal constraints considered in earlier work on
temporal graph patterns or temporal network motifs are readily
expressible by timed automata, as long as a point-based approach
to time is taken
\cite{DBLP:journals/corr/abs-1107-5646,DBLP:conf/sigmod/GurukarRR15,DBLP:conf/wsdm/ParanjapeBL17,DBLP:conf/wsdm/ParanjapeBL17,DBLP:conf/edbt/ZufleREF18}.

An important benefit of timed automata is that they support an iterative state assignment mechanism, which can be useful for early detection of matches and pruning of non-matches. Based on this observation, we will introduce three algorithms to retrieve all instances of a temporal BGP match in a graph.  The first is a baseline algorithm intended for offline processing when the complete history of graph evolution is available at the time of execution.  The second is an \od algorithm that supports online query processing when the temporal graph arrives as a stream.  The third is a \pmatch algorithm that speeds up processing by sharing computation between multiple matches. % and can be used in both offline and on-demand modes.  
We will present an implementation of these algorithms in a dataflow framework, and will analyze performance trade-offs induced by the properties of the temporal BGP and of the underlying temporal graph.  

%\julia{very brief but precise summary of related work part 2, with citations.}

%Our first algorithm is a baseline for offline processing of temporal graphs, where the complete history of the graph is available at the time of query execution. Building on top of the baseline algorithm, we will introduce our on-demand algorithm, which is an extension of our baseline to support online query processing for cases where the graph arrives as a stream over time. Our final algorithm leverages partial matchings to speed up the process by sharing the computation between multiple matches and can be used for both online and offline modes. We studied the performance of our algorithm over different datasets and queries, showing cases where each algorithm would be the best to use.     

\paragraph{Contributions and roadmap} 
% Our contributions are summarized as follows  
\begin{itemize}
    \item We formally introduce a temporal graph model, motivated by graph pattern matching with complex temporal constraints, in Section~\ref{sec:model}, and propose a novel method for expressing temporal constraints using timed automata in Section~\ref{sec:automata}. 
    
    \item We introduce algorithms to enforce temporal constraints expressed by timed automata in Section~\ref{sec:algorithms}, and describe an implementation of these algorithms in a state-of-the-art dataflow framework in Section~\ref{sec:impl}.
    
    \item We present results of a comprehensive experimental evaluation in Section~\ref{sec:experiments}, showing that timed automata are practical and demonstrating interesting performance trade-offs.
    
    %show the effectiveness of our method over two kinds of temporal graphs, those where the history of graph evolution is available and those when the graph arrives as a stream, in Section~\ref{sec:experiments}.  

%    \item We show that our method performance is independent of the size of temporal constraints and can be used to answer multiple constraints at once without change of performance. 
    
%    \item We study the performance of our algorithm over different datasets and queries, showing cases where each algorithm would be the best to use. 
\end{itemize}

We  discuss related work in Section~\ref{sec:related} and conclude in Section~\ref{sec:conclusion}.

%\paragraph{Roadmap}The rest of this paper is organized as follows. Section~\ref{?model} we will formally define a temporal graph model designed for graphs where nodes are static, but edges can exist over multiple time points. Over this model, we define temporal graph patterns and temporal constraints. Using these formal definitions, then we introduce a novel method of expressing temporal constraints over graph patterns based on timed automata~\cite{alur1994theory}. We will describe the timed automata in detail in Section~\ref{?timed-automata}. Section~\ref{dataflow?} is focus on describing our algorithms to enforce the temporal constraints described by timed-automata and how we can combine our algorithms with known matching algorithms that use incremental-joins over the stream of data. Using incremental algorithms would enable us to find temporal matching both when all information is available at once or when the graph is arriving over a period of time. In Section~\ref{?implementation} we will discuss our implementation details of these algorithms using Rust. Finally, we show our system performance for multiple real datasets, various patterns, and timed automata in Section~\ref{expr}. \amir{Need to be completed after the paper is ready} 






==> old-dataflow.tex <==
\section*{Old Section 5}
% \subsection{Temporal graph representation }
% \label{sec:graph-rep}

% Assume that, we are given a temporal graph $H=(G,\xi)$ where $G=(N,E,\rho_G,\lambda_G)$. We are also given a temporal BGP $Q=(P,\Gamma)$ where $P=(X,Y,\rho_P,\lambda_P)$ as defined in Section~\ref{sec:model}.

% Our goal is to compute all matchings $\mu$ of $Q$ in $H$; recall that this means that $\mu$ must be a matching of $P$ in $G$, and, moreover, the temporal assignment $\alpha_\mu$ must satisfy $\Gamma$ (Definition~\ref{defassign}). Here, we assume $\Gamma$ is specified as an NFA (nondeterministic finite automaton) over the alphabet $\Sigma=2^Y$.


% We represent a temporal graph $H$ by three relations $\Node(\vid,\lab)$, \\ $\Edge(\eid,\vid_1,\vid_2,\lab)$ and $\Xitab(\eid,\tim)$. An example of this representation can be viewed in Figure~\ref{fig:h-rep}. 

% \begin{figure}[!htb]
% \centering
% \small
% % Please add the following Required packages to your document preamble:
% % \usepackage[table,xcdraw]{xcolor}
% % If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \begin{tabular}{lllllll}
% \multicolumn{4}{l}{\textbf{Node}} &  & \multicolumn{2}{l}{\textbf{Active}} \\ \cline{1-4} \cline{6-7} 
% \multicolumn{2}{|l|}{\w{vid}} & \multicolumn{2}{l|}{\w{label}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{\w{eid}} & \multicolumn{1}{l|}{\w{time}} \\ \cline{1-4} \cline{6-7} 
% \multicolumn{2}{|l|}{$v_1$} & \multicolumn{2}{l|}{employee} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{$e_1$} & \multicolumn{1}{l|}{1} \\ \cline{1-4} \cline{6-7} 
% \multicolumn{2}{|l|}{$v_2$} & \multicolumn{2}{l|}{employee} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{$e_1$} & \multicolumn{1}{l|}{3} \\ \cline{1-4} \cline{6-7} 
% \multicolumn{2}{|l|}{$v_3$} & \multicolumn{2}{l|}{employee} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{$e_2$} & \multicolumn{1}{l|}{1.1} \\ \cline{1-4} \cline{6-7} 
% \multicolumn{2}{|l|}{$v_4$} & \multicolumn{2}{l|}{employee} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{$e_2$} & \multicolumn{1}{l|}{1.9} \\ \cline{1-4} \cline{6-7} 
% \multicolumn{2}{|l|}{$v_5$} & \multicolumn{2}{l|}{customer} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{$e_3$} & \multicolumn{1}{l|}{9} \\ \cline{1-4} \cline{6-7} 
% \multicolumn{2}{|l|}{$v_6$} & \multicolumn{2}{l|}{customer} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{$e_4$} & \multicolumn{1}{l|}{1} \\ \cline{1-4} \cline{6-7} 
% \multicolumn{2}{|l|}{$v_7$} & \multicolumn{2}{l|}{customer} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{$e_5$} & \multicolumn{1}{l|}{1} \\ \cline{1-4} \cline{6-7} 
%  &  &  &  & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{$e_5$} & \multicolumn{1}{l|}{3} \\ \cline{6-7} 
% \multicolumn{4}{l}{\textbf{Edge}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{$e_5$} & \multicolumn{1}{l|}{5} \\ \cline{1-4} \cline{6-7} 
% \multicolumn{1}{|l|}{\w{eid}} & \multicolumn{1}{l|}{\w{vid\textsubscript{1}}} & \multicolumn{1}{l|}{\w{vid\textsubscript{2}}} & \multicolumn{1}{l|}{\w{label}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{$e_6$} & \multicolumn{1}{l|}{2} \\ \cline{1-4} \cline{6-7} 
% \multicolumn{1}{|l|}{$e_1$} & \multicolumn{1}{l|}{$v_1$} & \multicolumn{1}{l|}{$v_2$} & \multicolumn{1}{l|}{message} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{$e_6$} & \multicolumn{1}{l|}{4} \\ \cline{1-4} \cline{6-7} 
% \multicolumn{1}{|l|}{$e_2$} & \multicolumn{1}{l|}{$v_1$} & \multicolumn{1}{l|}{$v_3$} & \multicolumn{1}{l|}{message} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{$e_6$} & \multicolumn{1}{l|}{6} \\ \cline{1-4} \cline{6-7} 
% \multicolumn{1}{|l|}{$e_3$} & \multicolumn{1}{l|}{$v_2$} & \multicolumn{1}{l|}{$v_4$} & \multicolumn{1}{l|}{message} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{$e_7$} & \multicolumn{1}{l|}{2} \\ \cline{1-4} \cline{6-7} 
% \multicolumn{1}{|l|}{$e_4$} & \multicolumn{1}{l|}{$v_3$} & \multicolumn{1}{l|}{$v_4$} & \multicolumn{1}{l|}{message} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{$e_8$} & \multicolumn{1}{l|}{2} \\ \cline{1-4} \cline{6-7} 
% \multicolumn{1}{|l|}{$e_5$} & \multicolumn{1}{l|}{$v_5$} & \multicolumn{1}{l|}{$v_1$} & \multicolumn{1}{l|}{message} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{$e_8$} & \multicolumn{1}{l|}{3} \\ \cline{1-4} \cline{6-7} 
% \multicolumn{1}{|l|}{$e_6$} & \multicolumn{1}{l|}{$v_1$} & \multicolumn{1}{l|}{$v_5$} & \multicolumn{1}{l|}{message} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{$e_8$} & \multicolumn{1}{l|}{4} \\ \cline{1-4} \cline{6-7} 
% \multicolumn{1}{|l|}{$e_7$} & \multicolumn{1}{l|}{$v_6$} & \multicolumn{1}{l|}{$v_1$} & \multicolumn{1}{l|}{message} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{$e_9$} & \multicolumn{1}{l|}{9} \\ \cline{1-4} \cline{6-7} 
% \multicolumn{1}{|l|}{$e_8$} & \multicolumn{1}{l|}{$v_7$} & \multicolumn{1}{l|}{$v_1$} & \multicolumn{1}{l|}{message} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{$e_{10}$} & \multicolumn{1}{l|}{2} \\ \cline{1-4} \cline{6-7} 
% \multicolumn{1}{|l|}{$e_9$} & \multicolumn{1}{l|}{$v_1$} & \multicolumn{1}{l|}{$v_7$} & \multicolumn{1}{l|}{message} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{$e_{10}$} & \multicolumn{1}{l|}{4} \\ \cline{1-4} \cline{6-7} 
% \multicolumn{1}{|l|}{$e_{10}$} & \multicolumn{1}{l|}{$v_2$} & \multicolumn{1}{l|}{$v_3$} & \multicolumn{1}{l|}{message} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{$e_{10}$} & \multicolumn{1}{l|}{6} \\ \cline{1-4} \cline{6-7} 
% \end{tabular}
% \caption{Representation of a temporal graph $H$ as relations $Node$, $Edge$ and $Active$ for the temporal graph in Figure~\ref{fig:def2}.}
% \label{fig:h-rep}
% \end{figure}



% % \begin{figure}[!htb]
% % \centering
% % \small
% % % Please add the following Required packages to your document preamble:
% % % \usepackage[table,xcdraw]{xcolor}
% % % If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% % \begin{tabular}{ccccclcclcc}
% % \multicolumn{3}{l}{\textbf{Node}} & \multicolumn{2}{p{3em}}{} & & \multicolumn{4}{l}{\textbf{Active}} \\ \cline{1-4} \cline{7-8} \cline{10-11} 
% % \multicolumn{2}{|c|}{{ \w{vid}}} & \multicolumn{2}{c|}{{ \w{label}}} &  & \multicolumn{1}{l|}{} & \multicolumn{1}{c|}{{ \w{eid}}} & \multicolumn{1}{c|}{{ \w{time}}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{{ \w{eid}}} & \multicolumn{1}{l|}{{ \w{time}}} \\ \cline{1-4} \cline{7-8} \cline{10-11} 
% % \multicolumn{2}{|c|}{\val{v{1}}} & \multicolumn{2}{c|}{\val{person}} &  & \multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\val{e\textsubscript{1}}} & \multicolumn{1}{c|}{\val{1}} & \multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\val{e\textsubscript{3}}} & \multicolumn{1}{c|}{\val{1}} \\ \cline{1-4} \cline{7-8} \cline{10-11} 
% % \multicolumn{2}{|c|}{\val{v\textsubscript{2}}} & \multicolumn{2}{c|}{\val{store}} &  & \multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\val{e\textsubscript{1}}} & \multicolumn{1}{c|}{\val{2}} & \multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\val{e\textsubscript{3}}} & \multicolumn{1}{c|}{\val{2}} \\ \cline{1-4} \cline{7-8} \cline{10-11} 
% % \multicolumn{2}{|c|}{\val{v\textsubscript{3}}} & \multicolumn{2}{c|}{\val{person}} &  & \multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\val{e\textsubscript{1}}} & \multicolumn{1}{c|}{\val{4}} & \multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\val{e\textsubscript{3}}} & \multicolumn{1}{c|}{\val{3}} \\ \cline{1-4} \cline{7-8} \cline{10-11} 
% % \multicolumn{4}{l}{} &  & \multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\val{e\textsubscript{2}}} & \multicolumn{1}{c|}{\val{5}} & \multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\val{e\textsubscript{3}}} & \multicolumn{1}{c|}{\val{4}} \\ \cline{7-8} \cline{10-11} 
% % \multicolumn{4}{l}{\textbf{Edge}} &  & \multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\val{e\textsubscript{2}}} & \multicolumn{1}{c|}{\val{6}} & \multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\val{e\textsubscript{3}}} & \multicolumn{1}{c|}{\val{5}} \\ \cline{7-8} \cline{10-11} 
% % \multicolumn{1}{l}{{ \w{eid}}} & \multicolumn{1}{l}{{ \w{vid\textsubscript{1}}}} & \multicolumn{1}{l}{{ \w{vid\textsubscript{2}}}} & \multicolumn{1}{l}{{ \w{label}}} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\val{e\textsubscript{2}}} & \multicolumn{1}{c|}{\val{7}} & \multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\val{e\textsubscript{3}}} & \multicolumn{1}{c|}{\val{6}} \\ \cline{1-4} \cline{7-8} \cline{10-11} 
% % \multicolumn{1}{|c|}{\val{e\textsubscript{1}}} & \multicolumn{1}{c|}{\val{v\textsubscript{1}}} & \multicolumn{1}{c|}{\val{v\textsubscript{2}}} & \multicolumn{1}{c|}{\val{work}} &  &  &  &  & \multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\val{e\textsubscript{3}}} & \multicolumn{1}{c|}{\val{7}} \\ \cline{1-4} \cline{10-11} 
% % \multicolumn{1}{|c|}{\val{e\textsubscript{2}}} & \multicolumn{1}{c|}{\val{v\textsubscript{3}}} & \multicolumn{1}{c|}{\val{v\textsubscript{1}}} & \multicolumn{1}{c|}{\val{married}} &  &  &  &  &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ \cline{1-4}
% % \multicolumn{1}{|c|}{\val{e\textsubscript{3}}} & \multicolumn{1}{c|}{\val{v\textsubscript{3}}} & \multicolumn{1}{c|}{\val{v\textsubscript{2}}} & \multicolumn{1}{c|}{\val{own}} &  &  &  &  &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ \cline{1-4}
% % \end{tabular}
% % \caption{Representation of a temporal graph $H$ as relations $Node$, $Edge$ and $Active$ for the temporal graph in Figure~\ref{fig:def2}. \TODO{Update these tables after confirming the example is good}}
% % \label{fig:h-rep}
% % \end{figure}

% We also define ``snapshots'' and ``history'' follow. 
% \begin{definition}[Snapshot]
% For any $t \in T$, define the snapshot $ \EdgeSnap t = \{(\eid,\vid_1,\vid_2,\lab) \in \Edge \mid (\eid,t) \in \Xitab \} $ consisting of all edges that are active at time $t$.  
% \end{definition}

% \begin{definition}[History]
% The union of all snapshots up to time $t$, formally defined as $ \EdgeH t = \bigcup \{ \EdgeSnap u \mid u \in T \text{ and } u\leq t \}, $ is  referred to as the \emph{history} up to time $t$.  
% \end{definition}

% Note that $\EdgeH {t_n}$ equals the entire $\Edge$ relation. Example~\ref{ex:snap-hist} shows these definition for the graph of Figure~\ref{fig:h-rep} for $t=5$.

% \begin{example}
% \label{ex:snap-hist}
%     $$ \EdgeSnap 5 = \{(e_2,v_3,v_1,married),~ (e_3,v_3,v_2,own)  \} $$
% \end{example}

\subsection{Finding the matching}
\label{sec:find-match}

Using the relations introduced in the previous section, we want to compute a relation $\Match$, over the relation schema $X \cup Y$, that consists of all matchings of $P$ in $G$.  

The result of expression $\Exp$ applied to $\Node$ and $\EdgeH t$ is denoted by $\MatchH t$; this relation consists of all matchings of $P$ in the history up to time $t$.  Note that $\MatchH {t_n}$ is the relation $\Match$ that we want to compute.


For the purpose of initialization, we define $t_0:=0$ and define $\MatchH {0}$ and $\EdgeH {0}$ to be empty. We now compute, incrementally for $i=1,\dots,n$, the relation $\MatchH {t_i}$ from the relations $\Node$, $\MatchH {t_{i-1}}$, $\EdgeH {t_{i-1}}$, and $\EdgeSnap {t_i}$. We denote the set of matchings that are newly discovered in iteration $i$ by $\MatchSnap {t_i}$.


To express the structure of patterns in this work we use Datalog queries, Example~\ref{ex:path3} shows this approach for a path of length 3 and Example~\ref{ex:tri} shows a pattern of a triangle. Note that without loss of generality for  simplicity we disregarded the labels here. 
\begin{example}
\label{ex:path3}
Path of length3 %\julia{don't need a space between the name of the relation and its attributes}
$$      Path3(y_1,y_2,y_3) = E(y_1,a,b), E(y_2,b,c), E(y_3,c,d)
$$
\end{example}
\begin{example}
\label{ex:tri}
Triangle
$$    triangle(y_1,y_2,y_3) = E(y_1,a,b), E(y_2,b,c), E(y_3,c,a)$$
\end{example}

Clearly, $\Match$ can be computed by a relational algebra expression $\Exp$ over $\Node$ and $\Edge$; this expression $\Exp$ involves only the operators equijoin, selection, renaming, and projection~\cite{zou2009distance,DBLP:journals/vldb/NeumannW10,DBLP:journals/tods/AbergerLTNOR17}. To find $\MatchSnap {t_i}$ we can be use algorithm from previous work on incremental evaluation of relational algebra expressions \cite{amsj_subgraph}. The focus of our work is to combine existing matching algorithm with temporal constraints. In the remainder of this section, we will first describe how we can use an NFA constraint combined with non-incremental matching to achieve temporal BGPs with complex temporal constraints and then extend our work to incremental algorithms and streams. 

A match of size $M$ would be consist of $M$ edges. One way to represent a matching is to use a nested relation in which the identifier of the matching, \insql{mid}, is the primary key and a list of \insql{eid}s  lists the corresponding edges. The schema for matching can be viewed in the following. We use an ordered list (list) with the size equal to the matching to keep all \insql{eid}s. 

\begin{Verbatim}[fontsize=\small,baselinestretch=.5]
Matching {mid:long, y: list (eid)}
\end{Verbatim}

Using this schema to represent matching of  %$x_1 \xrightarrow{y_1} x_2 \xrightarrow{y_2} x_3$,
 $$P(y_1,y_2,y_3) = E(y_1,a,b), E(y_2,b,c)$$ over the graph in Figure~\ref{fig:def2} we will have only one matching $mid=1 , y=[e_2,e_1]$.

\subsection{Enforcing constraints using NFAs}
\label{sec:bgp:nfa-enforcment}

In Section~\ref{sec:expres}, we discussed different ways to specify temporal constraints using select-project-join queries in SQL. SQL constraints expressed in that section can be simply implemented as select-condition.  The focus of this section is on enforcing complex temporal constraints expressed by NFAs.

We expressed our NFA constraints enforcement using dataflow operators which would enable us to combine NFA with our matching algorithm.  First we describe an NFA as a relation with the following schema.
\begin{verbatim}
    NFA { current-state (cs):long, words(w):bitset, 
          next-state(ns):long }
\end{verbatim}

 In this schema, the current-state and next-state are numerical values and the word is a bitset with a size equal to the matching. Due to the nature of NFA, the primary-key for this relation is a combination of \insql{(current-state, words, next-state)}.   
 
  Figure~\ref{fig:alt-nfa-rel} gives a relational representation of a NFA for alternation constraints where  $y_1$ and $y_2$ must alternate, starting with $y_1$, and ending with $y_2$., 
  In this relation, each row in the table corresponding to a valid transition.  Each bit of the \texttt{words} bitset is assigned to one of the edges in the matching. In this figure you can see the bit would be set to $1$ when the NFA expects the edges to exist (e.g., $y_1$ is part of the transition condition on the edge $(s_0,s_1)$) and zero when the NFA expects the edge not to exist(e.g., $\neg y_2$ is part of the transition condition on the edge $(s_0,s_1)$). To encode transitions that are always taken (where the transition condition is $\mathit{true}$) or where one of the variables can have multiple values, in our design, we need to have multiple rows with the words corresponding to each of these cases. 


%   \begin{figure}[!ht]
%     \centering 
%     \begin{tikzpicture}[->, on grid, node distance=90pt]
%             \node[state, initial, accepting] (s0) {$s_0$};
%             \node[state, right of=s0] (s1) {$s_1$};
%             \draw (s0)
%           (s0) edge[above, bend left] node{$y_1 \land \neg y_2$} (s1)
%           (s1) edge[below, bend left] node{$y_2 \land \neg y_1$} (s0);
%     \end{tikzpicture}
%     %\qquad
%     \\
%         \begin{tabular}{|l|l|l|} 
%         \multicolumn{3}{l}{\textbf{NFA}} \\
%         \hline
%          \w{\underline{current-state}} & \w{\underline{words}} &  \w{\underline{next-state}}  \\ 
%         \hline
%         \val{S0}           & \val{10}    & \val{S1}         \\ 
%         \hline
%         \val{S1}           & \val{01}    & \val{S0}         \\
%         \hline
%         \end{tabular}
%     \captionlistentry[table]{A table beside a figure}
%     \caption{Relational Representation of the NFA}
%     \label{fig:alt-nfa-rel}
%   \end{figure} 

NFA needs the data to arrive as words. In our design, for each snapshot, we use 1-1 map to convert a matching  to a word. Word is defined as a \insql{mid}, list of \insql{eid}s to keep the edge assignment for the matching, a bitset to show the existence of an edge in a similar way to the NFA's bitset, and a time-point to indicate the corresponding validity time of the word. In this relation the primary-key is $(mid,time)$. The bitset in the word tuple has $N$ bits where $N$ is the matching size. If the corresponding edge is valid at the time, the corresponding bit would be set to $1$; otherwise, the bit would be set to zero. Note that for every valid matching at each time point we will have a unique word tuple. 

\begin{Verbatim}[fontsize=\small,baselinestretch=.5]
Word {mid:long, y: list(eid), time:long, words:bitset}
\end{Verbatim}

Figure~\ref{fig:word-matching} shows the words for matching \{ $ mid=1 , y=[e_2,e_1] $ \} in the graph of Figure~\ref{fig:def2}. For example, at time $1$, edge $e2$ exists and edge $e1$ does not, represented by the word $01$, while at time $3$ neither of the edges exists, represented by the word $00$. 

\begin{figure}[!h]
\caption{Word representation of graph in Figure~\ref{fig:def2} for matching \{mid=1,  y=[$e_2$,$e_1$]\}}
\label{fig:word-matching}
\centering
\begin{tabular}{|l|l|l|l|} 
\hline
\w{\underline{mid}} &\w{y (y1,y2)} & \w{\underline{time}} & \w{word}  \\ 
\hline
\val{$1$ }   &\val{$e_2,e_1$ }   & \val{1 }   & \val{01}    \\ 
\hline
\val{$1$ }   &\val{$e_2,e_1$ }   & \val{2 }   & \val{01}    \\ 
\hline
\val{$1$ }   &\val{$e_2,e_1$ }   & \val{3 }   & \val{00 }   \\ 
\hline
\val{$1$ }   &\val{$e_2,e_1$ }   & \val{4  }  & \val{01 }   \\ 
\hline
\val{$1$ }   &\val{$e_2,e_1$ }   & \val{5 }   & \val{10 }   \\ 
\hline
\val{$1$ }   &\val{$e_2,e_1$ }   & \val{6}    & \val{01 }   \\ 
\hline
\val{$1$ }   &\val{$e_2,e_1$ }   & \val{7 }   & \val{01 }   \\
\hline
\end{tabular}
\end{figure}


Algorithm~\ref{alg:non-incr-alpha} shows the process of computing words from matching and active tuples for one snapshot of the graph as defined in Section~\ref{sec:graph-rep}. In this algorithm, for each \insql{eid} in the matching, we perform a left-outer join between the matching relation and the active edge relation. For the cases that the left-outer join returns a tuple with a corresponding (non-null) component inactive, the algorithm produces a True bit for the corresponding edge in the bitset, and for the cases, it is a miss, the algorithm would produce a False.  
\begin{algorithm}[!b]
\caption{Word Computation for one Snapshot}
\label{alg:non-incr-alpha}
\begin{algorithmic}[1]
    \Require Set of active edges in the snapshot: $A$, Set of Matching: $M$, Matching Size: $Match\_Size$
    \State $\alpha \gets M$
    \For {$i \gets 0$ to $Match\_Size$}
        \State $\alpha \gets \alpha$.\textbf{join} (A,~how$\gets$left-outer, on$\gets$ ($\alpha.y[i] = A.eid$)
    \EndFor
    \State words $\gets$ convertToAlpha ($\alpha$) \\ \Comment {Convert null values to 0 and non-null values to 1 and build the bitset}
    \State \Return words

\end{algorithmic}
\end{algorithm}



  The next natural step is to feed the words to NFA. Algorithm~\ref{alg:incr-nfa} shows the process of running the NFA. In this algorithm, we pass sets of matches, computed using our matching algorithm explained in Section~\ref{sec:bgp:tbgp-math}, sets of words, computed based on Algorithm~\ref{alg:incr-alpha}, an NFA described in the prevision section and an initial state of the algorithm.  The algorithm first creates current\_state by adding the initial state to each matching (note that the matches are unique). For each time-point in the temporal domain, we apply the NFA to the matches using the words and find the next\_state. We implement this using two pairwise inner joins. For cases where there is no appropriate rule in the NFA, the matching would not join with any rows in the NFA and, as a result, will be removed from the matching set. In this algorithm, we update the list of remaining matches at each step and then compute words only for the valid matches at each time-point. Put another way, we delay the production of the words until the time when they are needed. This algorithm needs a set of precomputed matches, a set of active tuples, and the initial state as inputs. In the final step of this algorithm, the matching list gets updated.

\begin{algorithm}[!h]
\caption{NFA Enforcment}
\label{alg:incr-nfa}
\begin{algorithmic}[1]
    \Require  Set of Matching: $M$, NFA: $NFA$, Set of Active  Edges:A, Initial State: $S0$, Match Size:  $Match\_Size$;
    \State $current\_state \gets M$.map ($m \rightarrow (m.mid,m.y, S0)$) \\ \Comment{ Add initial state to all the matches }
    \State $A' \gets \emptyset$ \\ \Comment{ Initiate current active}
    \State $current\_time \gets 0$
    \ForAll{$a \in A$}
        \If {a.time > $current\_time$}
            \State $words \gets compute\_words (  A',M, $Match\_Size$) $ \\ \Comment {Based on  algorithm~\ref{alg:non-incr-alpha}}
             \State$current\_state \gets current\_state$    \\ \Comment{Update state for each match based on NFA}
             \Indent
                \State .\textbf{join} ($words$,how$\gets$inner, on$\gets y$)
                \State .\textbf{join} (NFA, how $\gets$ inner,   on$\gets words$)) 
                \State  .\textbf{map} ( $cs \rightarrow (cs.y, cs.ns)$)
            \EndIndent
       \State $ M \gets $current\_state .\textbf{map} ( $cs \rightarrow (cs.mid, cs.y)$)   \\ \Comment { Update the remaining matchings}
            \State $current\_time \gets a.time$
            \State $A' \gets \emptyset$

        \EndIf
    \State $A' \gets A' + a $
    \EndFor
\end{algorithmic}
\end{algorithm}

Eventually, after the NFA finishes running or even at the end of each step, we can look at the remaining matches in the current\_state and see how many are in one of the accepting states.   Note that this algorithm does not need to know the time-domain of the graph in advance.


\subsection{On-demand NFA}
Algorithm~\ref{alg:non-incr-alpha} needs all the possible matches to be precomputed and will run over all those matchings from time zero; yet, for many scenarios where the graph is arriving in the real time the list of all edges and matching can not be computed at time zero. In addition to that in many real graphs %where the distribution of the number of new edges over time follows the power-law,
most edges and matchings will not exist until the last few time-points of the graph\cite{leskovec2008microscopic}. For cases where we want to see the results as early as possible, this would add an unnecessary delay to the computation of the NFA over the initial section of the graph where we have fewer matchings.

One solution to this problem is to run an on-demand NFA for the new matching arrived at time ${t}$, $Match_{t}$ from time $0$ to $t-1$ and then after assigning a correct state to these newly matching, we add those to the existing matching set and continue running our original NFA as described in Algorithm~\ref{alg:incr-nfa} for all the matching $\MatchH t$ for one iteration. 

Algorithm~\ref{alg:on-dem-nfa} describe the process for single time point $t$. In this algorithm, the ``getNewMatching'' function would use an incremental algorithm to compute the new matchings at time $t$  and then run an NFA from $0$ to $t-1$ over these new matchings. After the on-demand NFA finish running, we will merge these new matchings to the existing matching and continue running the main NFA.   Note that in this algorithm ``RunNFA'' follows the same logic as Algorithm~\ref{alg:incr-nfa}. 


\begin{algorithm}[!h]
\caption{On-Demand NFA}
\label{alg:on-dem-nfa}
\begin{algorithmic}[1]
    \Require  Set of Existing Matching with States at time t: $ms_{\leq t-1}$, NFA: $NFA$, Set of Active Edges:$A$, Set of Edge: $E$, Initial State: $S0$, current time : $t$;

    \State $ Match_t = getNewMatchings(t, A, E)$
    \State $ms_{t} \gets Match_{t}$.map ($m \rightarrow (m.mid,m.y, S0)$) \\ \Comment{ Add initial state to new the matchings } 
    
    
    \For {$t'$ from $1$ to $t-1$}
    \State $A_i= A.filter (a \rightarrow a.t ==t')$
    \State $ ms_{t}  \gets RunNFA(ms_{t},A_i)$
    \EndFor
    \State $ ms_{\leq t} \gets  ms_{\leq t-1} +  ms_{t}   $
    
    \State $A_t \gets A.filter (a \rightarrow  a.t == t)$
    \State $ ms_{\leq t}  \gets RunNFA(  ms_{\leq t} , A_t)$
    
\end{algorithmic}
\end{algorithm}




\subsection{Partial Matching} \amir{Jan this is the updated algorithm}
While the on-demand algorithm can postpone the execution of the NFA until the matching becomes valid, it still runs the NFA for the same number of cycles as the algorithm~\ref{alg:incr-nfa}. One way to optimize the number of cycles is to reduce the duplicate computations by leveraging the partial matchings.

We define the following partial matching schema. In this schema, ``mid'' is unique ID  assigned to each total or partial matching. The ``y'' array contains the  edges assigned to the variables in the BGP. For variables that we have not assigned yet, the corresponding element of the ``y'' array would be null. The ``size'' shows how many edges have been set and can be between zero for empty partial matching and the pattern size for the total matching. The ``state'' shows the current state of the matching regarding the temporal automaton.  The ``clock'' array contains the clocked set for matching. Note that in this schema the primary key is $(mid,state)$, this is due to the nature of the timed automaton where one matching can exist in multiple states. 

 \begin{Verbatim}[fontsize=\small,baselinestretch=.5]
Partial Matching {mid:long , y:array[edge], 
        size:long, state:long, clock:array[long]}
\end{Verbatim}
 
 We consider a partial match to be any match that at least one of its variables in the edge array has not been set (is null). For a matching of size $M$, the smallest partial match would have no edge, meaning the list used to keep \insql{edge}s would have $M$ null values, and the largest partial match would have only one null element in the \insql{eid}s list. (e.g., y=[$null$,$null$], y=[$e_1$,$null$],  y=[$null$,$e_1$]). We define the size of partial matchings as the number of variables that assigned here y=[$null$,$null$] will have a size of zero, while y=[$e_1$,$null$] would have size one.  



Algorithm~\ref{alg:partial-nfa} shows the process of running time automaton for cases where we have partial matching. In this algorithm, first, we create a matching set with only one matching which is an empty partial match.  Then at each iteration, we compute new partial and new total matchings using the function getNewMatchings. This function runs multiple join queries producing all possible partial and total matching based on the partial/total matching that already exists and newly arrived edges. Any algorithm capable of finding static matching can be used here, in the Section~\ref{sec:impl} we discuss how we implemented this. 

Note that unlike the  on-demand algorithm, here we do not need to compute the current state for the newly arrived matchings and they would inherit the current state from the partial matching that they got created from. All new matchings either get created from an existing matching, which can be the initial empty matching that we added at time zero. 

After finding all matchings, we run the timed automaton in a similar way to the baseline algorithm. Note that the NFA can threat a nonassigned edge the same way as a non-existing edge. 

\begin{algorithm}[!h]
\caption{Partial-Match NFA}
\label{alg:partial-nfa}
\begin{algorithmic}[1]
    \Require  Set of edges: $Edge$, NFA: $NFA$, Set of Active Edges:A,  current time : $t$;

    \State $M \gets M + EmptyMatching()$ \Comment{Initiate matching with an empty matching}
    \State $E \gets \emptyset$ \Comment{ Initiate seen edges}
    
    \State $A' \gets \emptyset$  \Comment{ Initiate current active}
    \State $current\_time \gets 0$
    
    \ForAll{$a \in A$}
        \If {a.time > $current\_time$}
            \State $ \Delta M = getNewMatchings(M, \Delta E)$
            \State $M \gets M + \Delta M$
            \State $ M  \gets RunNFA( M , A')$
            \State $ E \gets E + \Delta E$
            \State $\Delta E \gets \emptyset$
            \State $A' \gets \emptyset$
            \State $current\_time \gets a.current\_time$

        \EndIf
    \State $A' \gets A' + a $
    \If {$a.eid \not \in E$}
        \State $\Delta E \gets \Delta E + Edges.get(a.eid) $  \Comment{Add the edge if this is the first time we see it}
    \EndIf
    \EndFor
\end{algorithmic}
\end{algorithm}


\subsection{Extension to Clock}
We introduced the timed automaton in Section~\ref{sec:expr}. The main difference between the regular NFA and timed automaton(TA) is the ability to set clocks, and checking the condition of the clocks before making the pass. 

We can implement a TA as a relation, the same way we implemented the NFA. In our design, TA has the following schema. 

\begin{verbatim}
    TA { current-state (cs):long, words(w):bitset, 
          next-state(ns):long, clock-set: long, 
          clock-cond : func([long]) -> bool }
\end{verbatim}

The TA has all the properties of an NFA with two additional fields, clock-set, and clock-cond. The clock-set is the index of the clock that the transition in the NFA will set. The clock-cond is a user-define function that takes an array of clocks and based on a condition returns a Boolean variable. Figure~\ref{fig:ta-rel} shows an example of a TA. As it can be seen for rows where the TA does not set a clock the clock-set column is empty. 

  \begin{figure}[!ht]
    \centering 
    \begin{center}
        \begin{tikzpicture}[->, on grid, node distance=60pt]
        \node[state, initial] (s0) {$s_0$};
        \node[state, right of=s0] (s1) {$s_1$};
        \node[state, accepting, right of=s1] (s2) {$s_2$};
        \draw (s0) edge[loop above] node{$\mathit{true}$} (s0)
      (s0) edge[above] node{$y_1$} node[below]{$\xx:=0$} (s1)
      (s1) edge[loop above] node{$\mathit{true}$} (s1)
      (s1) edge[above] node{$y_2 \land \xx>7$} (s2);
        \end{tikzpicture}
    \end{center}

    
        \begin{tabular}{|l|l|l|l|l|} 
        \multicolumn{5}{l}{\textbf{NFA}} \\
        \hline
         \w{\underline{current-state}} & \w{\underline{words}} &  \w{\underline{next-state}} &  \w{\underline{clock\_set}}&  \w{\underline{clock\_cond}}  \\ 
        \hline
        \val{S0}           & \val{**}    & \val{S0}  & \val{}  & \val{$f()\rightarrow true$}         \\ 
        \hline
        \val{S0}           & \val{1*}    & \val{S1}  & \val{0}  & \val{$f()\rightarrow true$}         \\ 
        \hline
        \val{S1}           & \val{**}    & \val{S1}  & \val{}  & \val{$f()\rightarrow true$}         \\ 
        \hline
        \val{S1}           & \val{*1}    & \val{S2}   & \val{}  & \val{$f()\rightarrow c[0] > 7$ }       \\
        \hline
        \end{tabular}
    \captionlistentry[table]{A table beside a figure}
    \caption{Relational Representation of the TA}
    \label{fig:ta-rel}
  \end{figure} 


Algorithm~\ref{alg:TA} shows the enforcement process for TA. As you can see the general procedure is the same. The main difference is Line~\ref{alg:ta:clock_set} where we use the clock-set function, a user-defined function to set the clock that TA pointed to and at Line~\ref{alg:ta:clock_cond} where we filter the matchings that did not satisfy the constraints. 

\begin{algorithm}[!h]
\caption{TA Enforcment}
\label{alg:TA}
\begin{algorithmic}[1]
    \Require  Set of Matching: $M$, TA: $TA$, Set of Active  Edges:A, Initial State: $S0$, Match Size:  $Match\_Size$;
    \State $current\_state \gets M$.map ($m \rightarrow (m.mid,m.y, S0)$) \\ \Comment{ Add initial state to all the matches }
    \State $A' \gets \emptyset$ \\ \Comment{ Initiate current active}
    \State $current\_time \gets 0$
    \ForAll{$a \in A$}
        \If {a.time > $current\_time$}
            \State $words \gets compute\_words (  A',M, $Match\_Size$) $ \\ \Comment {Based on  algorithm~\ref{alg:non-incr-alpha}}
             \State$current\_state \gets current\_state$    \\ \Comment{Update state for each match based on NFA}
             \Indent
                \State .\textbf{join} ($words$,how$\gets$inner, on$\gets y$)
                \State .\textbf{join} (TA, how $\gets$ inner,   on$\gets words$)) 
                \State  .\textbf{map} ( $cs \rightarrow (cs.y, cs.ns, cs.clk\_cond, setCLK(cs.clock\_set)$) \label{alg:ta:clock_set}
                 \State  .\textbf{filter} ( $cs \rightarrow apply(cs.clock\_cond(cs.clocks)$) \label{alg:ta:clock_cond}

            \EndIndent
       \State $ M \gets $current\_state .\textbf{map} ( $cs \rightarrow (cs.mid, cs.y)$)   \\ \Comment { Update the remaining matchings}
            \State $current\_time \gets a.time$
            \State $A' \gets \emptyset$

        \EndIf
    \State $A' \gets A' + a $
    \EndFor
\end{algorithmic}
\end{algorithm}



%\subsection{Optimization over Existential Constraints}


==> old-tex/bgp.tex <==
\section{A new approach}

We begin by recalling the basic notions of graph and graph pattern used in graph databases \cite{wood_survey}.\julia{We probably have to say something about property graphs, that our goal is to bring graph databases to the temporal setting, and that we begin with the most basic graph database model, extension to the property graph model being an obvious next step to do in future work.}  Thereto, we assume some finite alphabet $L$ of \emph{labels}, and define:

\begin{definition}[Graph]
\label{def:tg1}
A graph is a tuple $(N,E,\rho,\lambda)$, where:
\begin{itemize}
\item $N$ is a finite set of {\em nodes}, $E$ is a finite set of {\em edges}, and $N \cap E = \emptyset$;
%\item $L$ is a finite set of labels; 
\item $\rho: E \to (N \times N)$ is a total function that indicates for each edge its source and destination nodes;
\item $\lambda: N \cup E \to L$ is a total function giving a label to every node and edge.
\end{itemize}
\end{definition}

For our purposes, \emph{timepoints} can be taken to be strictly positive real numbers.

\begin{definition}[Temporal graph]
A temporal graph is a pair $(G,\xi)$ where $G$ is a graph and
$\xi$ assigns a finite set of timepoints to each edge of $G$.\footnote{Nodes are non-temporal for now.}  When $e$ is an edge and $t \in \xi(e)$, we also say that $e$ is ``active'' at time $t$.
\label{def:tg}

Figure~\ref{fig:def2} shows an example of a temporal graph, where nodes $v_1$ and $v_3$ have label ``person'', so $\lambda(v_1) = \lambda(v_3) =$ ``person'',  and are connected to a node $v_2$ that has label ``store'', so $\lambda(v_2) =$ ``store''. For edge $e_1$ that connects $v_1$ to $v_3$ we have time set of $\xi(e_1)= \{1,2,6,7\}$. It means that $v_1$ worked (was active) in the store for $\{1,2\}$, stop working for times 3, 4 and 5, and started again at timepoint $\{6,7\}$. 
\begin{figure}
  \centering
  \includegraphics[width=\linewidth]{figs/def2.pdf}
  \caption{An example of a temporal graph. \julia{Amir, please make this into a tikzpicture.}}
  \label{fig:def2}
\end{figure}
\end{definition}

\jan{I don't like $\xi$ it looks very cryptic. If you insist on Greek let's use $\tau$, the Greek for $t$, for ``time''.}\julia{$\tau$ usually stands for ``temporal slice'' in the temporal relational literature, I'd rather not overload.}

We realized that even for \emph{basic} graph patterns (without the ability to match edge variables in the pattern to entire paths in the data) things are complicated enough. We revise earlier definitions as follows.

\begin{definition}[Basic graph pattern (BGP)]
A BGP is a tuple $(X,Y,\rho,\lambda$),
where:
\begin{itemize}
\item $X$ and $Y$ are disjoint sets of variables, called \emph{node variables} and \emph{edge variables} respectively;
%\item $L$ is a finite set of labels; 
\item $\rho: Y \to (X \times X)$ is a total function that indicates for each  edge variable  its source and destination node variables;
\item $\lambda:X \cup Y \to L$ assigns a label from $L$ to each variable.
\end{itemize}
\label{def:bgp}
\end{definition}

Note that Definition~\ref{def:bgp} do not support node and edge constants, but may add them at a later point.

So, we have dropped the regular expressions. The definition of matching is accordingly simplified as follows:

\begin{definition}[Matching] \label{defmatch}
A \emph{partial matching} from BGP $(X,Y,\rho_P,\lambda_P)$ in a graph $G=(N,E,\rho,\lambda)$ is a function $\mu:Z \to N \cup E$ such that
\jan{I include here a notion of partial matching, but I am not sure yet if we will use it in the end, depends on how we are going to initialize the state set of newly found matchings, see algorithm.}
\begin{itemize}
\item
$Z$, the domain of $\mu$, is a subset of $X \cup Y$;
\item
$\mu(Z \cap X) \subseteq N$ and $\mu(Z \cap Y) \subseteq E$;
\item
For any edge variable $y \in Z$, if $\rho_P(y)=(x_1,x_2)$, then also $x_1,x_2 \in Z$, and
$\rho(\mu(y))=(\mu(x_1),\mu(x_2))$;
\item
For every $z\in Z$, we have
$\lambda(\mu(z)) = \lambda_P(z)$.
\end{itemize}
If $Z$ equals $X\cup Y$ then $\mu$ is called a (total) \emph{matching}.
\end{definition}

To extend the notion of matching to temporal graphs, we will enrich BGPs with temporal constraints, introduced as follows.

\begin{definition}[Temporal variables, assignments, and constraints]\label{defassign}
Let $V$ be a set of temporal variables. A \emph{temporal assignment} $\alpha$  on $V$ is a function that assigns a finite set of timepoints to every variable in $V$. A \emph{temporal constraint} over $V$ is a set of temporal assignments on $V$.  When a temporal assignment $\alpha$ belongs to a temporal constraint $\Gamma$, we also say that $\alpha$ \emph{satisfies} $\Gamma$.
\end{definition}

This is, for the moment, a purely semantic definition of temporal constraints; later we will go into how such constraints may be specified, using various logics or automata.

%Suppose that the set of temporal variables is $V=\{y_1,y_2,y_3\}$. The corresponding $\alpha$ to Temporal Graph in  Figure~\ref{fig:def5} can be $\alpha(y1) = \{1,2,4\}$, $\alpha(y2) = \{5,6,7\}$ and $\alpha(y3) = \{1,2,3,4,5,6,7\}$. 


% \begin{figure}
%   \centering
%   \includegraphics[width=\linewidth]{figs/def5.pdf}
%   \caption{An example of a temporal graph. \julia{Amir, please make this into a tikzpicture.}}
%   \label{fig:def5}
% \end{figure}


\begin{figure}
  \centering
    \begin{tikzpicture}[on grid, node distance=90pt]
      \node[state,minimum size= 10pt]   (v1)                {$v_1$:p};
      \node[state,minimum size= 10pt]           (v2) [right=of v1] {$v_2$:s};
      \node[state,minimum size= 10pt] (v3) [right=of v2] {$v_3$:p};
      \path[->] (v1) edge                node [above] {$e_1$} node[below]{\tiny{$T:=\{1,2,4\}$}} (v2)
                (v3) edge [bend left=35] node [above] {$e_2$} node[below]{\tiny{$T:=\{5,6,7\}$}} (v1)
                (v3) edge                node [above] {$e_3$} node[below]{\tiny{$T:=\{1,2,3,4,5,6,7\}$}}(v2);
    \end{tikzpicture}
  \caption{An example of a temporal graph.}
  \label{fig:def5}
\end{figure}




The following are examples of temporal constraints over three temporal variables $V=\{y_1,y_2,y_3\}$:
\begin{enumerate}
\item
The set of all assignments $\alpha$ on $T$ where $\alpha(y_1)$ and $\alpha(y_2)$ are disjoint.
\item
The set of all $\alpha$ where $\max\alpha(y_3) - \min\alpha(y_3)>5$.
\item
The set of all $\alpha$ where there exist $t_i \in \alpha(y_i)$, for $i=1,2,3$, such that $t_1<t_2<t_3$.
\item
And so on!
\end{enumerate}

If we have a matching $\mu$ from a BGP in a graph $G$, and we consider a temporal version $(G,\xi)$ of $G$, then we automatically obtain a temporal assignment on the edge variables of the BGP.  Indeed, each edge variable is matched to an edge in $G$, and we take the set of timepoints of that edge.  So, the edge variables serve as temporal variables.  We thus arrive at the following definition:

%\marginpar{\jan{Proposal to use $\Gamma$ (capital gamma) instead of $\gamma$, I find that $\gamma$ is not visible enough.}}

\begin{definition}[Temporal BGP, matching]
A temporal BGP is a pair $(P,\Gamma)$ where $P$ is a BGP and $\Gamma$ is a temporal constraint over $Y$ (the edge variables of $P$).
Let $(G,\xi)$ be a temporal graph.

Given a matching $\mu$ of $P$ in $G$, we can consider the temporal assignment $\xi \circ \mu|_Y$ on $Y$; we denote this assignment by $\alpha_\mu$ (and read it ``$\xi$ after $ \mu$ restricted to $Y$'').
% "\xi composed after \mu, restricted to the edge variables $Y$"

A matching of $(P,\Gamma)$ in $(G,\xi)$ is a matching $\mu$ of $P$ in $G$ such that $\alpha_\mu$ satisfies $\Gamma$.
\end{definition}
%%TODO: Add example

Now the whole game is to consider various ways of specifying temporal constraints.  We consider various possibilities.
\begin{description}
\item[SQL]
(FOL with order and gap constraints.) Indeed, we can consider each temporal variable as a unary relation name.  A temporal assignment is an instance over these relation names; each unary relation is a set of timepoints.  Then we could specify a temporal constraint by writing a boolean SQL expression.  This is obviously very powerful. \julia{This is one of the methods we consider in this work.}
\item[Temporal logic]
We can also take a temporal logic perspective and specify the temporal constraint as a temporal logic formula where the temporal variables serve as the propositions.

To allow for gap constraints we can use a timed temporal logic that allows this.
\item[Timed automata]
Temporal logic (or timed temporal logic) can be efficiently compiled into timed automata.  This may be interesting for processing temporal BGP queries. \julia{This is one of the methods we consider in this work.}
\item[Existential constraints]
These are much simpler, but possibly already quite useful.  If the temporal variables are $\{y_1,\dots,y_k\}$, use timepoint variables $t_1,\dots,t_k$, and write a quantifier-free formula over these timepoint variables, where you can use order and gap comparisons.  Then $\Gamma$ is the constraint $$ \exists t_1 \in y_1 \dots \exists t_k\in y_k : \psi. $$
\end{description}

==> old-tex/incremental.tex <==
\section{Incremental evaluation of temporal BGPs with NFA temporal constraints}

\emph{(The idea here is to do the exercise first for an NFA and not yet for a fully fledged timed automaton. An NFA is a timed automaton without any clocks. Once we understand this, we can then beef up the exercise by dealing with the clocks.)}

We are given a temporal graph $H=(G,\xi)$ where $G=(N,E,\rho_G,\lambda_G)$. We are also given a temporal BGP $Q=(P,\Gamma)$ where $P=(X,Y,\rho_P,\lambda_P)$.
Our goal is to compute all matchings $\mu$ of $Q$ in $H$; recall that this means that $\mu$ must be a matching of $P$ in $G$, and, moreover,
the temporal assignment $\alpha_\mu$ must satisfy $\Gamma$ (Definition~\ref{defassign}).
Here, we assume $\Gamma$ is specified as an NFA (nondeterministic finite automaton) over the alphabet $\Sigma=2^Y$.

\subsection{NFA temporal constraint} \label{secnfa}

Using an NFA makes sense because the temporal assignment $\alpha_\mu$ can be naturally viewed as a word (string) over $\Sigma$. Formally, define $T = \bigcup \{\xi(e) \mid e \in E\}$ as the set of all distinct timepoints used in $H$; we also refer to $T$ as the \emph{temporal domain} of $H$. Let $T=\{t_1,\dots,t_n\}$, ordered as $t_1<\cdots<t_n$. We can then view $\alpha_\mu$ as a word $a_1 \dots a_n$, where $a_i = \{y \in Y \mid t_i \in \xi(\mu(y))\}$.  
%\marginpar{Julia: add example (see notes)}

Since a temporal constraint specifies a set of temporal assignments, and we view temporal assignments as words, a temporal constraints specifies a set of words, i.e., a formal language over $\Sigma$.  This motivates the use of NFAs, which are indeed a standard mechanism to specify formal languages.

\julia{Amir, please merge everything below into a single example.  The BGP and the graph should be part of the example environment.}

Consider the following example. We are matching a BGP \\

$P: x_1 \xrightarrow{y_1} x_2 \xrightarrow{y_2} x_3$  over a temporal graph $H=(G, \xi)$, where\\ $G=v_1 \xrightarrow{e_1} v_2 \xrightarrow{e_2} v_3 \xrightarrow{e_3} v_4$ and $\xi(e_1) = \{1, 2 \}$,  $\xi(e_2) = \{2, 3 \}$, and  $\xi(e_3) = \{1, 3 \}$.


\begin{example}\label{ex1}
Consider the following matching: $\mu(x_1) =v_1$, $\mu(x_2) =v_2$, $\mu(x_3) =v_3$, $\mu(y_1) =e_1$ and $\mu(y_2) =e_2$. Then $\alpha_\mu(y_1) = \{1,2\}$ and $\alpha_\mu(y_2)=\{2,3\}$.

We can represent this assignment $\alpha_\mu$ as the word consisting of the following letters: $a_1 = \{y_1\}$,  $a_2 = \{y_1,y_2\}$, $a_3 = \{y_2\}$.  Further, $\alpha_\mu$ can be viewed as:

\begin{tabular}{llll}
&$t_1=1$ & $t_2=2$ & $t_3=3$ \\
$\alpha_\mu =$&$\{y_1\}$ & $\{y_1,y_2\}$ & $\{y_2\}$
\end{tabular}

This is a both a word and a temporal assignment. 
\end{example}

\begin{example}\label{ex2}
Consider the following matching: $\mu(x_1) =v_2$, $\mu(x_2) =v_3$, $\mu(x_3) =v_4$, $\mu(y_1) =e_2$ and $\mu(y_2) =e_3$.  Then $\alpha_\mu(y_1) = \{2,3\}$ and $\alpha_\mu(y_2)=\{1,3\}$

We can represent this matching $\alpha_\mu$ as a word a: $a_1 = \{y_2\}$,  $a_2 = \{y_1\}$, $a_3 = \{y_1, y_2\}$ and $\alpha_\mu$ can be viewed as:

\begin{tabular}{llll}
&$t_1=1$ & $t_2=2$ & $t_3=3$ \\
$\alpha_\mu =$&$\{y_2\}$ & $\{y_1\}$ & $\{y_1,y_2\}$
\end{tabular}

This is a both a word and a temporal assignment. 
\end{example}

Note that in Examples~\ref{ex1} and~\ref{ex2}, the temporal domain $T = \{1, 2, 3\}$.  It doesn't have to be sequential natural numbers, and can be, for example, $T = \{1.4, 3.8, 7\}$.

%We specify the NFA $\gamma$ by a tuple $(Q,I,F,\Delta)$, where $Q$ is the finite set of states; $q_0 \in Q$ is the initial state; $F \subseteq Q$ is the set of accepting states; and $\Delta \subseteq Q \times \Sigma \times Q$ is the set of transitions.

\subsection{Finding the matchings}

We represent a temporal graph $H$ by three relations $\Node(\vid,\lab)$, \\ $\Edge(\eid,\vid_1,\vid_2,\lab)$ and $\Xitab(\eid,\tim)$. An example of this representation can be viewed in Figure~\ref{fig:h-rep}. We want to compute a relation $\Match$, over the relation schema $X \cup Y$, that consists of all matchings of $P$ in $G$.  Clearly, $\Match$ can be computed by a relational algebra expression $\Exp$ over $\Node$ and $\Edge$; this expression $\Exp$ involves only the operators equijoin, selection, renaming, and projection. Our approach is to evaluate $\Exp$ incrementally over time.


\begin{figure}[!htb]
\centering
\small
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{tabular}{ccccclcclcc}
\multicolumn{4}{l}{\textbf{Node}} & \multicolumn{2}{p{3em}}{} & \multicolumn{5}{l}{\textbf{Active}} \\ \cline{1-4} \cline{7-8} \cline{10-11} 
\multicolumn{2}{|c|}{{ \w{vid}}} & \multicolumn{2}{c|}{{ \w{label}}} &  & \multicolumn{1}{l|}{} & \multicolumn{1}{c|}{{ \w{eid}}} & \multicolumn{1}{c|}{{ \w{time}}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{{ \w{eid}}} & \multicolumn{1}{l|}{{ \w{time}}} \\ \cline{1-4} \cline{7-8} \cline{10-11} 
\multicolumn{2}{|c|}{\val{v{1}}} & \multicolumn{2}{c|}{\val{person}} &  & \multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\val{e\textsubscript{1}}} & \multicolumn{1}{c|}{\val{1}} & \multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\val{e\textsubscript{3}}} & \multicolumn{1}{c|}{\val{1}} \\ \cline{1-4} \cline{7-8} \cline{10-11} 
\multicolumn{2}{|c|}{\val{v\textsubscript{2}}} & \multicolumn{2}{c|}{\val{store}} &  & \multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\val{e\textsubscript{1}}} & \multicolumn{1}{c|}{\val{2}} & \multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\val{e\textsubscript{3}}} & \multicolumn{1}{c|}{\val{2}} \\ \cline{1-4} \cline{7-8} \cline{10-11} 
\multicolumn{2}{|c|}{\val{v\textsubscript{3}}} & \multicolumn{2}{c|}{\val{person}} &  & \multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\val{e\textsubscript{1}}} & \multicolumn{1}{c|}{\val{4}} & \multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\val{e\textsubscript{3}}} & \multicolumn{1}{c|}{\val{3}} \\ \cline{1-4} \cline{7-8} \cline{10-11} 
\multicolumn{4}{l}{} &  & \multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\val{e\textsubscript{2}}} & \multicolumn{1}{c|}{\val{5}} & \multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\val{e\textsubscript{3}}} & \multicolumn{1}{c|}{\val{4}} \\ \cline{7-8} \cline{10-11} 
\multicolumn{4}{l}{\textbf{Edge}} &  & \multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\val{e\textsubscript{2}}} & \multicolumn{1}{c|}{\val{6}} & \multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\val{e\textsubscript{3}}} & \multicolumn{1}{c|}{\val{5}} \\ \cline{7-8} \cline{10-11} 
\multicolumn{1}{l}{{ \w{eid}}} & \multicolumn{1}{l}{{ \w{vid1}}} & \multicolumn{1}{l}{{ \w{vid\textsubscript{2}}}} & \multicolumn{1}{l}{{ \w{label}}} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\val{e\textsubscript{2}}} & \multicolumn{1}{c|}{\val{7}} & \multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\val{e\textsubscript{3}}} & \multicolumn{1}{c|}{\val{6}} \\ \cline{1-4} \cline{7-8} \cline{10-11} 
\multicolumn{1}{|c|}{\val{e\textsubscript{1}}} & \multicolumn{1}{c|}{\val{v\textsubscript{1}}} & \multicolumn{1}{c|}{\val{v\textsubscript{2}}} & \multicolumn{1}{c|}{\val{work}} &  &  &  &  & \multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\val{e\textsubscript{3}}} & \multicolumn{1}{c|}{\val{7}} \\ \cline{1-4} \cline{10-11} 
\multicolumn{1}{|c|}{\val{e\textsubscript{2}}} & \multicolumn{1}{c|}{\val{v\textsubscript{3}}} & \multicolumn{1}{c|}{\val{v\textsubscript{1}}} & \multicolumn{1}{c|}{\val{married}} &  &  &  &  &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ \cline{1-4}
\multicolumn{1}{|c|}{\val{e\textsubscript{3}}} & \multicolumn{1}{c|}{\val{v\textsubscript{3}}} & \multicolumn{1}{c|}{\val{v\textsubscript{2}}} & \multicolumn{1}{c|}{\val{own}} &  &  &  &  &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ \cline{1-4}
\end{tabular}
\caption{Representation of a temporal graph $H$ as relations $Node$, $Edge$ and $Active$ for the temporal graph in Figure~\ref{fig:def5}.}
\label{fig:h-rep}
\end{figure}


% \begin{figure}[!htb]
% \centering
% \caption{Representation of H as Node, Edge and Active for graph in section~\ref{secnfa}}
% \label{fig:h-rep2}
% \begin{tabular}{ccccccl}
% Node: &  &  &  &  & Active: &  \\ \cline{1-4} \cline{6-7} 
% \multicolumn{2}{|c}{vid} & \multicolumn{2}{c|}{label} & \multicolumn{1}{c|}{} & eid & \multicolumn{1}{c|}{time} \\ \cline{1-4} \cline{6-7} 
% \multicolumn{2}{|c|}{\val{$v_1$}} & \multicolumn{2}{c|}{label1} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\val{$e_1$}} & \multicolumn{1}{c|}{1} \\ \cline{1-4} \cline{6-7} 
% \multicolumn{2}{|c|}{\val{$v_2$}} & \multicolumn{2}{c|}{labl\val{$e_2$}} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\val{$e_1$}} & \multicolumn{1}{c|}{2} \\ \cline{1-4} \cline{6-7} 
% \multicolumn{2}{|c|}{\val{$v_3$}} & \multicolumn{2}{c|}{label3} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\val{$e_2$}} & \multicolumn{1}{c|}{2} \\ \cline{1-4} \cline{6-7} 
% \multicolumn{2}{|c|}{\val{$v_4$}} & \multicolumn{2}{c|}{label4} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\val{$e_2$}} & \multicolumn{1}{c|}{3} \\ \cline{1-4} \cline{6-7} 
% Edge: &  &  &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\val{$e_3$}} & \multicolumn{1}{c|}{1} \\ \cline{1-4} \cline{6-7} 
% \multicolumn{1}{|c}{eid} & vid1 & vid2 & \multicolumn{1}{c|}{label} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\val{$e_3$}} & \multicolumn{1}{c|}{1} \\ \cline{1-4} \cline{6-7} 
% \multicolumn{1}{|c|}{\val{$e_1$}} & \multicolumn{1}{c|}{\val{$v_1$}} & \multicolumn{1}{c|}{\val{$v_2$}} & \multicolumn{1}{c|}{label1} &  &  &  \\ \cline{1-4}
% \multicolumn{1}{|c|}{\val{$e_2$}} & \multicolumn{1}{c|}{\val{$v_2$}} & \multicolumn{1}{c|}{\val{$v_3$}} & \multicolumn{1}{c|}{label2} &  &  &  \\ \cline{1-4}
% \multicolumn{1}{|c|}{\val{$e_3$}} & \multicolumn{1}{c|}{\val{$v_3$}} & \multicolumn{1}{c|}{\val{$v_4$}} & \multicolumn{1}{c|}{label3} &  &  &  \\ \cline{1-4}
% \end{tabular}
% \end{figure}{}


Specifically, for any $t \in T$, define the snapshot $$ \EdgeSnap t = \{(\eid,\vid_1,\vid_2,\lab) \in \Edge \mid (\eid,t) \in \Xitab \} $$ consisting of all edges that are active at time $t$.  The union of all snapshots up to time $t$, formally defined as $$ \EdgeH t = \bigcup \{ \EdgeSnap u \mid u \in T \text{ and } u\leq t \}, $$ is also referred to as the \emph{history} up to time $t$.  Note that $\EdgeH {t_n}$ equals the entire $\Edge$ relation. The result of expression $\Exp$ applied to $\Node$ and $\EdgeH t$ is denoted by $\MatchH t$; this relation consists of all matchings of $P$ in the history up to time $t$.  Note that $\MatchH {t_n}$ is the relation $\Match$ that we want to compute.


For the purpose of initialisation, we define $t_0:=0$ and define $\MatchH {0}$ and $\EdgeH {0}$ to be empty. We now compute, incrementally for $i=1,\dots,n$, the relation $\MatchH {t_i}$ from the relations $\Node$, $\MatchH {t_{i-1}}$, $\EdgeH {t_{i-1}}$, and $\EdgeSnap {t_i}$.  The algorithm can be taken from previous work on incremental evaluation of relational algebra expressions \cite{amsj_subgraph,related papers}.  We denote the set of matchings that are newly discovered in iteration $i$ by $\MatchSnap {t_i}$.

\begin{example}
    For the temporal graph in Figure~\ref{fig:h-rep} for $t=5$ we have:
    $$ \EdgeSnap 5 = \{(e_2,v_3,v_1,married),~ (e_3,v_3,v_2,own)  \} $$
    
\end{example}{}

\subsection{Checking the temporal constraint} \label{secstates}

For each $\mu \in \Match$, we need to check that the word $\alpha_\mu$ is accepted by the NFA $\Gamma$.  We integrate this check into our incremental approach, where snapshots are processed in chronological order.  Specifically, for $i=1,\dots,n$, we work as follows.
\begin{enumerate}
    \item
    For each newly discovered matching, i.e., $\mu \in \MatchSnap {t_i}$, we determine the set $S$ of states the NFA can be in after reading the prefix of $\alpha_\mu$ of length $i$.  We store $(\mu,S)$ in an auxiliary table $\States$.
    
    %Alternatively, it may be desirable to generate an identifier $\emid$ for every matching. Then table $\Match$ gets $X \cup Y \cup \{\emid\}$ as relation schema, and table $\States$ has relation schema $\{\emid,\state\}$.
    \item
    For the matchings $\mu$ that we already had, i.e., $\mu \in \MatchH {t_{i-1}}$, we do not have to rerun the NFA from the beginning, but we can update the set of possible states. Let $a_i$ be the $i$th letter of the word $\alpha_\mu$ as defined in Section~\ref{secnfa}. Let $S$ be the set of current possible states for $\mu$ as stored in table $\States$. Let $S'$ be the set of states $s'$ for which there exists a state $s \in S$ such that $(s,a_i,s')$ is an allowed transition in the NFA\@.  Then modify table $\States$ by updating $(\mu,S)$ to $(\mu,S')$. 
\end{enumerate}

Now after the $n$th iteration, the desired matchings are returned as $$ \{ \mu \in \Match \mid \exists S : (\mu,S) \in \States \text{ and $S$ contains an accepting state}\}. $$

Let us give more detail on how the incremental state update algorithm (Step~2 above) can be processed using queries.  \jan{The following is only a suggestion; more efficient approaches may be possible, or doing it without queries may also be more efficient.}

\begin{comment}
\paragraph{Nesting relation $\Xitab$.} Above we have conceptually presented the relation $\Xitab$ as consisting of the pairs $(e,t)$ where $e$ is an edge and $t \in \xi(e)$.  It may be more efficient, however, to store the pairs $(e,\xi(e))$ directly.  The set $\xi(e)$ may be represented in an array, or as a bitmap $b_1\dots b_n$ where $b_i = 1$ if $t_i \in \xi(e)$ and $0$ otherwise.
\end{comment}

\paragraph{Flattening the relation $\States$.} It will be convenient to assume an artificial key $\emid$ in the $\Match$ relation that holds a unique identifier for every matching.  Relation $\States$ is then represented as a flat relation $\States(\emid,\state)$.  So, $\States$ contains those pairs $(m,s)$ such that $m$ is the identifier of a matching $\mu$ and $s$ is a possible current state of the automaton running on word $\alpha_\mu$. 

\paragraph{NFA transitions.}  When working, as we do, over an alphabet $\Sigma$ that is of the form $2^Y$, it is convenient to work with a form of NFA where the transition table is set of triples of the form $(s_1,\theta,s_2)$ where $s_1$ and $s_2$ are states and $\theta$ is a boolean formulas over $Y$.  The meaning is that if some set $a$ of variables satisfies $\theta$, then the transition from $s_1$ to $s_2$ on input letter $a$ is allowed.

\paragraph{Current letter.} For each $\mu \in \Match$ we need to determine the current letter $a_i$, defined to be the set of edge variables $y$ for which $t_i \in \xi(\mu(y))$. Thereto, consider the following query $$ \varactive_y := \pi_{\emid,\text{`$y$'}} \, \sigma_{y=\eid \text{ and } \tim=t_i} (\Match \times \Xitab). $$
Note that the variable $y$ is returned verbatim, as a constant.  We can now form the union $\bigcup_{y \in Y} \varactive_y$ and array-aggregate the second column, grouped on the $\emid$ column. In this manner, each matching identifier is associated to an array of edge variables representing the current letter for that matching.\jan{This does not work if the current letter is empty; then the matching identifier will not appear at all. This can be fixed in various ways.} We denote the resulting relation by $\Letters(\emid,\letter)$.

\paragraph{Updating the current states.}  For any transition $(s_1,\theta,s_2)$ of the automaton, consider the query $$ \transition_{s_1,s_2} := \pi_{\emid,\text{`$s_2$'}} \, \sigma_{\state=s_1 \text{ and $\letter \models \theta$}}(\States \times \Letters). $$
Now form the union of all $\transition_{s_1,s_2}$ for all transitions of the automaton. The result is the updated value for the $\States$ relation.

\subsection{Extension to clocks}

In order to be able to express temporal constraints that involve not only temporal ordering but also actual delays or time gaps, we move from NFAs to timed automata \cite{alurdill_ta}. Timed automata extend NFA's with clocks. The condition on a state transition can now involve comparison of clock values with delay constants. Moreover, transitions can reset clocks. For example, consider the following NFA which expresses the existential constraint $ \exists t_1 \in y_1 \exists t_2 \in y_2 : t_1 < t_2$:
    \begin{center}
        \begin{tikzpicture}
        \node[state, initial] (s0) {$s_0$};
        \node[state, right of=s0] (s1) {$s_1$};
        \node[state, accepting, right of=s1] (s2) {$s_2$};
        \draw (s0) edge[loop above] node{$\mathit{true}$} (s0)
        (s0) edge[above] node{$y_1$} (s1)
        (s1) edge[loop above] node{$\mathit{true}$} (s1)
        (s1) edge[above] node{$y_2$} (s2);
        \end{tikzpicture}
    \end{center}
    

    
    
\newcommand{\xx}{\mathtt{x}}
\newcommand{\RR}{\mathtt{R}}




Suppose we want to express the constraint $\exists t_1 \in y_1 \exists t_2 \in y_2 : t_1 < t_2 \: \land \: t_2-t_1>7$ (in other words, the delay between $y_1$ and $y_2$ should be at least seven time units).  We can do this by adapting the above automaton as follows. We introduce a clock $\xx$. The clock starts running at time $0$.  When we see $y_1$, we reset the clock.  Then when we see $y_2$, we check that the clock has progressed beyond the desired $7$ time units.
\begin{center}
        \begin{tikzpicture}
        \node[state, initial] (s0) {$s_0$};
        \node[state, right of=s0] (s1) {$s_1$};
        \node[state, accepting, right of=s1] (s2) {$s_2$};
        \draw (s0) edge[loop above] node{$\mathit{true}$} (s0)
        (s0) edge[above] node{$y_1$} node[below]{$\xx:=0$} (s1)
        (s1) edge[loop above] node{$\mathit{true}$} (s1)
        (s1) edge[above] node{$y_2 \land \xx>7$} (s2);
        \end{tikzpicture}
    \end{center}

We next discuss how the incremental state update algorithm (Section~\ref{secstates}) is adapted to support clocks.  Formally, the transition table of the timed automaton is a set of triples of the form $(s_1,\theta,\delta,\RR,s_2)$. Here, as in the NFA case, $s_1$ and $s_2$ are states and $\theta$ is a boolean formula over $Y$. In a timed automaton transition we have two additional ingredients $\delta$ and $\RR$, where $\delta$ is the clock condition and $\RR$ is the set of clocks to be reset.  Here, $\delta$ is a boolean combination of conditions of the form $\xx \geq c$ where $\xx$ is a clock and $c$ is a strictly positive real number.

Accordingly, table $\States$ is expanded to keep not only the set of possible states for each matching, but also the corresponding clock values.  Assume there are $k$ clocks $\xx_1,\dots,\xx_k$. Then $\States(\emid,\state,\xx_1,\dots,\xx_k)$ contains those pairs $(m,s,c_1,\dots,c_k)$ such that $m$ is the identifier of a matching $\mu$ and $s$ is a possible current state of the timed automaton running on word $\alpha_\mu$, with current clock values $c_1,\dots,c_k$.

We next describe how this table is updated from time $t_{i-1}$ to $t_i$. Let $\States_{t_{i-1}}$ denote the contents of $\States$ immediately after processing timepoint $t_{i-1}$.  At time $t_i$ we populate $\States_{t_i}$ as follows.  Let $(m,s,c_1,\dots,c_k)$ be a tuple in $\States_{t_{i-1}}$ where $m$ identifies some matching $\mu$. As before, let $a_i$ be the $i$th letter of the word $\alpha_\mu$.  Let $(s,\theta,\delta,\RR,s')$ be a transition such that $a_i$ satisfies $\theta$ and $(c_1,\dots,c_k)$ satisfies $\delta$.  Then we insert $(m,s',c'_1,\dots,c'_k)$ in $\States_{t_i}$, where $c'_j$, for $j=1,\dots,k$, is defined as follows:
\begin{itemize}
    \item If $\xx_j \in \RR$ then $c'_j = 0$ (clock reset).
    \item Otherwise, $c'_j = c_j + t_i - t_{i-1}$ (clock advance).
\end{itemize}

\subsection{Discussion}

\begin{enumerate}
    \item The approach outlined in Section~\ref{secstates} is hybrid in the following sense.  On the one hand, on newly discovered matchings, the NFA is run from the beginning until the current time.  Note that this takes more and more time the further we progress in time, as the words get longer and longer. On the other hand, for already existing matchings, we maintain the current NFA states incrementally.  We could go completely incremental, if we compute not only total matchings but also partial matchings (Definition~\ref{defmatch}).  For any partial matching $\nu$, we can still consider the word $a_\nu$, just like we did for total matchings. Each letter will be a subset of the edge variables on which $\nu$ is defined.  Now an important observation is that, \emph{When a partial matching $\nu$ can be extended at time $t_i$ to a partial matching $\mu$, the words $\alpha_\nu$ and $\alpha_\mu$ have the same prefix of length $i-1$}.  Hence, we can update the set $S'$ of states for $\mu$ at time $t_i$ from the set $S$ of states for $\nu$ at time $t_{i-1}$ in the same way as described in step~2 of the algorithm.  The downside of this fully incremental approach is that the number of partial matchings generated may be huge. Indeed, the prohibitive number of partial matchings is mentioned by Ammar et al.\ \cite{amsj_subgraph} as the main problem with many BGP matching algorithms.  Are we going to work this out in the paper, and compare the hybrid with the purely incremental approach?
    \item Yet another approach would be a two-stage approach: (A) Find all matchings of $P$ in $G$, using whatever approach available from the literature; (B) Run the NFA on all these matchings to determine those that satisfy the temporal constraint.  It is not obvious that this is worse than the hybrid approach (or the purely incremental approach).  Also this could be empirically investigated.
    \item For the special case of existential temporal constraints, these can be incorporated directly in the relational algebra expression $\Exp$, without any need to use an NFA.  For a simple example, consider a BGP $$ x_1 \overset{y_1}{\longrightarrow} x_2 \overset{y_2}{\longrightarrow} x_3 $$ with temporal constraint $$ \exists t_1 \in y_1 \exists t_2 \in y_2 : t_1 < t_2. $$  The resulting temporal BGP can be expressed in SQL as 
    \begin{verbatim}
select $e_1$.eid as y1, $e_2$.eid as y2
from Edge $e_1$, Edge $e_2$, Active A1, Active A2
where $e_1$.vid2 = $e_2$.vid1 and $e_1$.eid=A1.eid and $e_2$.eid=A2.eid
  and A1.time < A2.time
    \end{verbatim}
    
\julia{Amir, if you wanted to use datalog syntax, here is an example that I like.  Note the distinction between variables like $c_1$ and constants like \val{F}.  And no dollar-signs, which is good.}


\[
Q_1() \leftarrow P(\_,\_;c_1;c_2), C(c_1,\_,\val{F},\_,\_,\_), C(c_2,\_,\val{M},\_,\_,\_)
\]

\julia{Here is another example, with conditions.}
\begin{equation*}
\begin{split}
Q() \leftarrow & P(\_,date;c_1;c_2), P(\_,date;c_1;c_3), P(\_,date;c_1;c_4), \\
& C(c_1,p,\_,\_,\_,\val{NE}), C(c_2,p,\_,\_,\_,\val{MW}), date=\val{"5/5"}, \\
& C(c_3,\_,\_,age,\_,\val{NE}), C(c_4,\_,\val{M},\_,\val{BA},\_), age = \val{50};
\end{split}
\end{equation*}

\begin{verbatim}
BGP($e1,$e2)   :- Edge($e1,$x1,$x2), Edge($e2,$x2,$x3)
T_BGP($e1,$e2) :- BGB($e1,$e2), Active($e1,$t1), Active($e2,$t2), $t1<$t2 
\end{verbatim}  

\begin{verbatim}
TEdge($e1,$t1,$x1,$x2) :- Edge($e1,$x1,$x2), Active($e1,$t1)
T_BGP($e1,$e2)         :- TEdge($e1,$t1,$x1,$x2), TEdge($e2,$t2,$x2,$x3), $t1<$t2

Or: 
T_BGP(e_1,e_2) :- TEdge(e_1,T1,x1,x2), TEdge(delta(e_2,T1+delta(t),x2,x3)

\end{verbatim}  
\julia{What's delta???}


Triangle: 
\begin{verbatim}
BGP(e_1,e_2)   :- Edge(e_1,x1,x2) AND Edge(e_2,x2,x3) AND Edge(e_3,x3,x1)
T_BGP(e_1,e_2) :- BGB(e_1,e_2) AND Active(e_1,T1)
                         AND Active(e_2,T2), AND Active(e_3,T3), T1<T2<T3 
\end{verbatim}  



    This SQL query can be processed using any approach, it is not suggested that this must be done on a conventional (whatever that may mean) RDBMS.
    
    On the other hand, the same temporal constraint can also be expressed by an NFA: 
    \begin{center}
        \begin{tikzpicture}
        \node[state, initial] (s0) {$s_0$};
        \node[state, right of=s0] (s1) {$s_1$};
        \node[state, accepting, right of=s1] (s2) {$s_2$};
        \draw (s0) edge[loop above] node{$\mathit{true}$} (s0)
        (s0) edge[above] node{$y_1$} (s1)
        (s1) edge[loop above] node{$\mathit{true}$} (s1)
        (s1) edge[above] node{$y_2$} (s2);
        \end{tikzpicture}
    \end{center}
    Again, are we going to compare the ``SQL approach'' with the other approaches?
    
    This can be also done for more complex temporal constraints that are still expressible in SQL\@.  For example consider the constraint that $y_1$ and $y_2$ must alternate, starting with $y_1$, and ending with $y_2$.  This is still expressible in SQL but requires complex non-exists subqueries.  With an NFA it is elegantly expressed by adapting the NFA shown above as follows: replace the two $\mathit{true}$ loops by $\emptyset$ loops; and add an $\epsilon$-transition from $s_2$ to $s_0$.  Here the NFA approach might win more clearly from the SQL approach?
    \begin{center}
        \begin{tikzpicture}
        \node[state, initial, accepting] (s0) {$s_0$};
        \node[state, right of=s0] (s1) {$s_1$};
        \draw (s0)
        (s0) edge[above, bend left] node{$y_1$} (s1)
        (s1) edge[below, bend left] node{$y_2$} (s0);
        \end{tikzpicture}
    \end{center}
    
    
\end{enumerate}

==> old-tex/intro.tex <==
\section{Introduction}
\label{sec:intro}
\amir{hi}
\julia{This section is stale.}

Suppose that we are interested in reachability and ask: What are the pairs of nodes that are connected by a path?  We can state this question using a navigational graph pattern (NGP) in Figure~\ref{fig:ngp}, an edge-labelled graph where nodes can be constants or variables, and edge labels can be constants, variables or regular path queries (RPQs)~\cite{DBLP:journals/corr/AnglesABHRV16}.  Note the symbol $*^T$, the temporal version of the Kleene closure operator. Evaluating the pattern in Figure~\ref{fig:ngp} under conventional (non-temporal) Kleene closure semantics on the graph in Figure~\ref{fig:timeasdata} will incorrectly return \insql{Alice} and \insql{Bill} as a connected pair, although there is no point in time during which there is a path between them!  

Intuitively, to compute the correct result we need to evaluate the query with respect to the state of the graph at each time instant.  Conceptually, we iterate through times  $t_1$ through $t_5$ and compute pairs Alice and John at times $t_2$ and $t_3$, and John and Bill at time $t_4$. This semantics is formalized in the temporal relational literature as the principle of {\em snapshot reducibility}, which states that the result of applying a temporal operator to a database is equivalent to applying the non-temporal variant of the operator to each state of the database~\cite{Bohlen2009}.

\begin{figure}
  \centering
  \includegraphics[width=
  \linewidth]{figs/TimeAsData.png}
  \caption{A time-annotated property graph.}
  \label{fig:timeasdata}
\end{figure}

\begin{figure}
	\centering
	\includegraphics[width=2in]{figs/TNGP.png}
    \caption{Temporal NGP $P_1$.}
    \label{fig:ngp}
\end{figure}

A user of an existing graph processing system may attempt to re-state the query to compute a temporally sensible result: Match paths in which all elements have an overlapping period of validity. % (as per Allen's overlap relation~\cite{Allen1983}).  
This condition can be checked incrementally by intersecting time periods as the path is traversed. However, stating such a query in a model in which time is treated as data is challenging, due to limited support for graph queries that combine data and topology. Conceptually, a query of this kind has the flavor of Regular Data Path Queries (RDPQs)~\cite{DBLP:journals/jacm/LibkinMV16}, which allow referencing data values of nodes that are connected by an edge, but  do not support predicates like overlap. Practically, Cypher~\cite{Neo4j_dm} and Gremlin~\cite{DBLP:conf/dbpl/Rodriguez15}, two state-of-the-art query languages for property graphs, cannot express this condition~\cite{DBLP:journals/corr/AnglesABHRV16}, and we are not aware of any graph query language that can.

For this and other queries, preserving snapshot reducibility ``by hand'' may in principle be possible, but it significantly increases conceptual complexity on the user, is error-prone, and will lead to queries that are more difficult to optimize and evaluate efficiently.

\paragraph{Contributions} In this work we introduce a new model$\dots$

==> old-tex/model.tex <==
\section{Model}
\label{sec:model}

We begin by recalling the basic notions of graph and graph pattern used in graph databases \cite{wood_survey}.\marginpar{We probably have to say something about property graphs, that our goal is to bring graph databases to the temporal setting, and that we begin with the most basic graph database model, extension to the property graph model being an obvious next step to do in future work.} Thereto, we assume some finite alphabet $L$ of \emph{labels}, and define:

\begin{definition}[Graph]
\label{def:tg1}
A graph is a tuple $(N,E,\rho,\lambda)$, where:
\begin{itemize}
\item $N$ is a finite set of {\em nodes}, $E$ is a finite set of {\em edges}, and $N \cap E = \emptyset$;
%\item $L$ is a finite set of labels; 
\item $\rho: E \to (N \times N)$ is a total function that indicates for each edge its source and destination nodes;
\item $\lambda: N \cup E \to L$ is a total function giving a label to every node and edge.
\end{itemize}
\end{definition}

Graph patterns, defined next, have the same structure as graphs, except that a pattern consists of node and edge \emph{variables} instead of actual nodes and edges. Moreover, edge variables can be labeled by regular expressions instead of just single labels.\marginpar{Can also have constants rather than variables.  Add later perhaps.}

\begin{definition}[Graph pattern]\textbf{}
\label{def:pattern}
A graph pattern is a tuple $(X,Y,\rho,\lambda_1,\lambda_2)$, where:
\begin{itemize}
\item $X$ and $Y$ are disjoint sets of variables, called \emph{node variables} and \emph{edge variables} respectively;
%\item $L$ is a finite set of labels; 
\item $\rho: Y \to (X \times X)$ is a total function that indicates for each an edge variable to its source and destination node variables;
\item $\lambda_1$ assigns a label from $L$ to each node variable;
\item $\lambda_2$ assigns a regular expression over $L$ to each edge variable.
\end{itemize}
\end{definition}

Edge variables in patterns actually represent paths in a graph.\footnote{Perhaps they should be called path variables instead of edge variables!} Formally, we define:

\begin{definition}[Path]
A path in a graph is a sequence of consecutive edges of the graph. For any graph $G$, denote the set of paths in $G$ by $\mathit{Paths}(G)$.
\end{definition}
\begin{definition}[Matching]
A \emph{matching} from graph pattern $(X,Y,\rho_P,\lambda_1,\lambda_2)$ in a graph $G=(N,E,\rho,\lambda)$ is a function $\mu:X\cup Y \to N \cup \mathit{Paths}(G)$ such that
\begin{itemize}
\item
$\mu(X) \subseteq N$ and $\mu(Y) \subseteq \mathit{Paths}(G)$;
\item
For any edge variable $e$, if $\rho_P(e)=(v,w)$, then $\mu(e)$ must be a path from $\mu(v)$ to $\mu(w)$.
\item
For every node variable $v$, we have
$\lambda(\mu(v)) = \lambda_1(v)$;
\item
For every edge variable $e$, the string of labels $\lambda(\mu(e))$ matches the regular expression $\lambda_2(e)$.
\end{itemize}
\end{definition}

\subsection{Temporal graphs}

For our purposes, \emph{timepoints} can be simply taken to be natural numbers, that is, timepoints are drawn from an \emph{ordered} domain.

\begin{definition}[Temporal graph]
A temporal graph is a pair $(G,\xi)$ where $G$ is a graph and
$\xi$ assigns a finite set of timepoints to each edge of $G$.\footnote{Nodes are non-temporal for now.}  When $e$ is an edge and $t \in \xi(e)$, we also say that $e$ is ``active'' at time $t$.
\label{def:tg}
\end{definition}

Our goal is to extend the notion of graph pattern so it can be used on temporal graphs.  One important aspect is the matching of edge variables to paths.  In a non-temporal pattern, we do this by specifying a regular expression over labels; the string of edge labels formed by the path should then match the regular expression.  In a temporal graph, a path forms not only a string of labels but also a string of sets of timepoints (one set per edge on the path).

Formally, consider a temporal graph $H=(G,\xi)$ and a path
$p = e_1\dots e_m$ in $G$.  The \emph{alternating set sequence of $p$ in $H$} is the sequence $$ \lambda(e_1) \xi(e_1) \dots \lambda(e_m) \xi(e_m). $$ Recall that $\lambda(e_i)$ is the label of edge $e_i$ and $\xi(e_i)$ is the set of timepoints associated to $e_i$.

The alternating set sequence of a path is an alternating sequence of labels and sets of timepoints.  In contrast to the labels, the timepoints do not come from a fixed finite alphabet. The same issue occurs in \emph{graphs with data} \cite{lmv_graph_data}, where nodes and edges not only have a label from a finite alphabet, but additionally carry a single data value from some infinite domain.  To implement regular expression matching over such sequences, we can follow the approach proposed by Libkin, Martens and Vrgo\v{c}, and move from standard finite automata (or regular expressions) to \emph{register automata}.  This automaton model is one of the established formalisms for dealing with strings over an infinite alphabet \cite{segoufin_survey}.

A challenge, however, is that we are dealing here with \emph{sets} of timepoints.  Our approach towards this challenge is to come up with ways to reduce (alternating) sequences of sets of timepoints to sequences of individual timepoints.  Specifically, we propose two natural such reductions: the \emph{sequential semantics} and the \emph{existential semantics}.

\subsubsection{Sequential semantics}

The sequential semantics takes advantage of the natural linear order on timepoints.  Indeed, in the alternating set sequence of some path, we can simply list all elements of every set of timepoints in order (of natural numbers).  The result is what we call the \emph{time sequence} of the path.

Formally, for any finite set $S$ of timepoints, we denote by $\seq(S)$ the sequence of the elements of $S$, listed in order.  Now given a path $p=e_1\dots e_m$ as before, we define the \emph{time sequence} of $p$ as the sequence $$ \lambda(e_1) \cdot \seq(\xi(e_1)) \cdot \cdots \cdot \lambda(e_1) \cdot \seq(\xi(e_m)) $$ where the dot denotes concatenation.


\subsubsection{Existential semantics}

The existential semantics extracts a sequence of timepoints from a sequence of sets of timepoints by picking one element from each set.  

Formally, a \emph{choice sequence} of a path $p=e_1\dots e_m$ is a sequence of the form $$ \lambda(e_1) x_1 \dots \lambda(e_m) x_m $$ where $x_i \in \xi(e_i)$ for $i=1,\dots,m$. As soon as one of the $\xi(e_i)$ contains more than one timepoint, the path $p$ obviously has multiple possible choice sequences for $p$.  In this sense, the existential semantics is nondeterministic.  On the other hand, if one of the $\xi(e_i)$ is empty, there does not exist a choice sequence for $p$.\marginpar{Jan: Do we want to allow edges with the empty set of timepoints? Julia: I think we should; an empty set of timepoints can occur in the result of a query that returns paths or edges.}


\subsection{Register automata}

We give a self-contained definition of register automata.  NOTE: PERHAPS WE CAN BETTER USE THE REGISTER REGULAR EXPRESSIONS INTRODUCED BY LIBKIN-MARTENS-VRGOC?

\subsection{Temporal graph patterns}

JAN: still need to do a pass on this.

Temporal constraints are defined over temporal variables, ranging over timepoints.

\begin{definition}[Temporal assignment]
Let $T$ be a set of temporal variables.  An \emph{assignment} on $T$ is a function that assigns a timepoint to every variable in $T$.
\end{definition}

\begin{definition}[Temporal constraint]
A \emph{temporal constraint} on a set $T$ of temporal variables is a set of assignments on $T$.
\end{definition}

\begin{comment}
Examples:
\begin{itemize}
\item
Suppose $T$ consists of a single second-order variable $x$.  Then the set of all assignments $\alpha$ satisfying $20180701 \in \alpha(x)$ is an example of a temporal constraint on $x$.
\item
Suppose $T$ consists of a single third-order variable $Y$.  Then the set of all assignments $\alpha$ such that $\alpha(Y) = S_1,\dots,S_n$, where there exist $t_1<\cdots<t_n$ with $t_i\in S_i$ for $i=1,\dots,n$, formalizes the journey constraint on paths.
\end{itemize}
\end{comment}

%\jan{What we are going to need are concrete simple languages for expressing such temporal constraints.}
%\julia{Allen relations~\cite{Allen1983} are a starting point, but they work over pairs of intervals, which is not what we are interested in here.}
%\julia{Temporal constraints article in the Temporal\_DBEncyclopedia.pdf, page 157 of the document.  Not terribly insightful, after a brief glance.}

\begin{definition}[Temporal graph pattern]
A temporal graph pattern is a tuple $(V_1,V_2,\rho_2,\lambda_1,\lambda_2,C)$ where
\begin{itemize}
\item
$(V_1,V_2,\rho_2,\lambda_1)$ is as in the definition of graph pattern;
\item
$\lambda_2$ assigns to every edge variable a register automaton over $L$ and the natural numbers;
\item
$C$ is a temporal constraint on the following variables: for each edge variable $y$, we have the three variables $\min(y)$, $\max(y)$, and $\exists(y)$.
\end{itemize}
\label{def:tgp}
\end{definition}

Register automata work on finite sequences of the form $(L\mathbf{N}^*)^*$, so sequences that alternate labels from $L$ with one or more timepoints.  These sequences will be generated from paths in the temporal graph. Th

\begin{definition}[Temporal matching]
Let $\mu$ be a matching from graph pattern $P$ in graph $G$.  Let $Q=(P,\gamma)$ be a temporal graph pattern and let $H=(G,\xi)$ be a temporal graph. We say that $\mu$ is a matching from $Q$ in $H$ if the following temporal assignment $\alpha$ belongs to $\gamma$.
\begin{itemize}
\item
For each node variable $v$, we define $\alpha(v) = \xi(\mu(v))$.
\item
For each edge variable $e$, let $\mu(e)=e_1,\dots,e_n$.  Then $\alpha(e)=\xi(e_1),\dots,\xi(e_n)$.
\end{itemize}
\end{definition}

Example. Consider a pattern with two node variables $x_1$ and $x_2$ and one edge variable $v$ from $x_1$ to $x_2$.  We could consider the temporal constraint that requires that $x_1$ contains the timepoint $20180701$ and that requires the journey constraint on $v$.  

\subsection{Examples}

%\julia{Examples: semantics, query, result (all matchings, at least one matching, does there exist a matching?)  ``Is there a journey from NYC to AMS?''  Expressible simply with existential semantics, but not with sequential. ``Are all flights from NYC to AMS before all flights from AMS to SVO?''  Expressible with sequential semantics, but not with existential semantics.  These examples show that the two semantics are incomparable, and that both are useful.  Do we want to allow the use of different semantics for different edge variables?}

To start, let us consider the following temporal graph pattern (TGP): 

$$P_1: v_1 - e \rightarrow v_2$$

In line with Definition~\ref{def:tgp}, vertices $v_1$ and $v_2$ and edge $e$ of $P_1$ are associated with labels $\lambda(v_1)$, $\lambda(v_2)$, and $\lambda(e)$, respectively.  Additionally, edge $e$ is associated with a set of time points $\xi(e)$.  

In what follows, it is sometimes convenient to treat $\xi(e)$ as an ordered sequence rather than as a set, which we denote $seq(\xi(e))$.  Recall that time points are drawn from a discrete domain with limited precision.  Time points $t_1$ and $t_2$ are {\em consecutive} if $t_2 - t_1 = 1$.

In what follows, $t$ is a constant that represents a time point, $T$ is a constant that represents a set of time points, $x$ is an integer.

We are interested in answering the following queries (most of these are Boolean, but we may be interested in non-Boolean variants as well):

\begin{enumerate}
\item Is $e$ valid at time $t$? In other words, we wish to check whether $t \in \xi(e)$.
\item Is there a time during which $e$ exists that is not included in $T$? That is, we are checking whether $\xi(e) - T \neq \emptyset$.
\item Is there a time during which $e$ exists that is included in $T$? In other words, we are checking whether $\xi(e) \cap T = \emptyset$.
\item Is $e$ valid for exactly / at least / at most $x$ intervals?  This query compares $|\xi(e)|$ with integer $x$.
\item Is $e$ valid for at period of length exactly / at least / at most $x$?  This query asks whether $seq(\xi(e))$ contains a sequence of exactly / at least / at most $x$ consecutive timepoints as a sub-sequence.
\item Is $e$ valid during exactly / at least / at most $x$ consecutive periods?  This query asks whether there are exactly / at least / at most $x-1$ gaps in $seq(\xi(e))$.
\item Get the earliest / latest point from $\xi(e)$, which we'll denote $min(\xi(e))$ and $max(\xi(e))$, respectively.
\item Compute $max(\xi(e)) - min(\xi(e))$.
\item Is $max(\xi(e)) - min(\xi(e))$ exactly / at least / at most $x$?
\item Size of gap, size of consecutive interval.... \julia{Continue here.  Look at temporal alignment.}
\end{enumerate}

Next, let us consider the following temporal graph pattern:

$$P_2: v_1 - e_1 \rightarrow v_2 - e_2 \rightarrow v_3$$

We may be interested in evaluating the following additional queries over $P_2$, which in some sense relate $\xi(e_1)$ and $\xi(e_2)$:

\begin{enumerate}
\item Is every point in $\xi(e_1)$ earlier / later than every point in $\xi(e_2)$?  In other words, is $max(\xi(e_1)) < min(\xi(e_2))$ for ``earlier'', and similarly for ``later''.  
\item Does $e_1$ start before $e_2$?  In other words, is $min(\xi(e_1)) < min(\xi(e_2))$?  Similarly for ``later''.
\item Is there a time during which both $e_1$ and $e_2$ exist?  In other words, is $\xi(e_1) \cap \xi(e_2) = \emptyset$?
\item Is there a time during which $e_1$ exists but $e_2$ does not?  In other words, is $\xi(e_1) - \xi(e_2) = \emptyset$?
\item Journey
\end{enumerate}






==> old-tex/old-intro.tex <==
\section{Introduction}
\label{sec:intro}

\begin{itemize}
    \item The Chronograph~\cite{DBLP:journals/tkde/ByunWK20}. Graph Traverse System. Temporal Graph model consists of $G_s$, the static graph, $G_t$: Events active in time points, $G_i$: events active in intervals. Gremlin~\cite{} based traverse language.  
    
    \item The T-GQL language\cite{debrouvier2021model},  introduce 3 temporal graph model Duration-labeled temporal graphs (DLTG), Interval-labeled temporal graphs (ILTG), Snapshot-based temporal graphs (SBTG)
    \item Nepal~\cite{DBLP:conf/sigmod/JohnsonKLS16} introduce a path query language, that supports time-travel queries which is a normal path query expressed over one specific time point. 
\end{itemize}

Graph pattern matching, the problem of finding instances of one graph in a larger graph, has been extensively studied since 1974 and a variety of algorithms have been proposed~\cite{conte2004thirty, cheng2008fast, ullmann1976algorithm, reza2020approximate, fan2010graph}. One of the early works in this area is Ullman et. al.~\cite{ullmann1976algorithm}, which is a back-tracing algorithm with a look-ahead function to reduce the search space. Many extensions of this algorithm have been proposed~\cite{ulman2011,vcibej2015improvements}, to improve the performance. Foggia and Vento~\cite{cordella1999performance,cordella2004sub,DBLP:journals/pami/CarlettiFSV18} work is another famous method for subgraph matching, which is a brute-force algorithm with simple but efficient prune strategies for the search space. 

One other way to view the graph matching problem is to treat the matching as relational table~\cite{lai2019distributed} built by series of  natural joins over an edge relation. By doing this, we can transfer this problem to the problem of finding an optimal join. For many years, the best way to solve this was edge-growing pairwise join plans.~\cite{selinger1989access, DBLP:journals/pvldb/SunWWSL12,DBLP:journals/pvldb/LaiQLC15}, but in recent years, a new family of vertex-growing plans, known as worst-case optimal join have emerged ~\cite{DBLP:journals/sigmod/NgoRR13,DBLP:journals/corr/abs-1210-0481} which have a better performance for cyclic patterns such as triangles. 

Most of the works mentioned above are focused on static graphs, where the temporal information has not been recorded. Finding patterns in static graphs can be helpful for some tasks, such as finding mutual interests among users in a social network without temporal information. However, using nontemporal graphs for other tasks such as contact tracing will likely produce inaccurate results. Our study aims to express and extract all instances of a pattern with complex temporal constraints from a large size temporal graph, where edges as events can reoccur many times. We will now introduce an example to demonstrate the necessity of temporal information in a graph. Later on, we use the same toy graph to represent different temporal graph matchings.

Figure~\ref{fig:def2},represent a communication graph, where each node is a person, either a customer or an employee, and each connection shows messages between a source node and a target node. Note that each edge is associated with a set of time-points during which that edge is valid.  This type of graphs with static nodes but dynamic edges that are active at multiple time-points are common for graphs that model interactions between entities \cite{DBLP:conf/wsdm/ParanjapeBL17}. 


\julia{Need to typeset labels differently here and in the text, hard to read.}

\begin{figure}
  \centering
    \begin{tikzpicture}[on grid, node distance=80pt,auto]
      \node[state,minimum size= 10pt, node distance=80pt]   (v1)                     {$v_1$:e};
      \node[state,minimum size= 10pt, node distance=80pt]   (v2) [above right=of v1] {$v_2$:e};
      \node[state,minimum size= 10pt, node distance=80pt]   (v3) [below right=of v1] {$v_3$:e};
      \node[state,minimum size= 10pt, node distance=80pt]   (v4) [below right=of v2] {$v_4$:e};
      
      \node[state,minimum size= 10pt, node distance=100pt]   (v5) [above left=of v1]   {$v_5$:c};
      \node[state,minimum size= 10pt, node distance=120pt]  (v6) [      left=of v1]        {$v_6$:c};
      \node[state,minimum size= 10pt, node distance=100pt]   (v7) [below left=of v1]  {$v_7$:c};
      
    \path[->] 
     (v1) edge  node [sloped,above] {$e_1$:m} node[sloped,below]{\small{$T=\{1,3\}$}} (v2)
     (v1) edge  node [sloped,above] {$e_2$:m} node[sloped,below]{\small{$T=\{1.1,1.9\}$}} (v3)
     (v2) edge  node [sloped,above] {$e_3$:m} node[sloped,below]{\small{$T=\{9\}$}} (v4)
     (v3) edge  node [sloped,above] {$e_4$:m} node[sloped,below]{\small{$T=\{1\}$}} (v4)
    
     (v5) edge [bend  left=25] node [sloped,above] {$e_5$:m} node[sloped,below]{\small{$T=\{1,3,5\}$}} (v1)
     (v1) edge [bend  left=25] node [sloped,above] {$e_6$:m} node[sloped,below]{\small{$T=\{2,4,6\}$}} (v5)
     
     (v2) edge node [sloped,above] {$e_{10}$:m} node[sloped,below]{\small{$T=\{2,4,6\}$}} (v3)
     
     (v6) edge  node [sloped,above] {$e_7$:m} node[sloped,below]{\small{$T=\{2\}$}} (v1)

     (v7) edge [bend  left=25] node [sloped,above] {$e_8$:m} node[sloped,below]{\small{$T=\{2,3,4\}$}} (v1)
     (v1) edge [bend  left=25] node [sloped,above] {$e_9$:m} node[sloped,below]{\small{$T=\{9\}$}} (v7)
    ;
    %             (v2) edge                node [above] {$e_3$:m} node[below]{\small{$T=\{1.7,2,3.5,6,8\}$}}(v3);
    \end{tikzpicture}
  \caption{An example of a temporal graph: a labeled graph with nodes $v_1$, $v_2$, $v_3$ and $v_4$ of type employee (denoted 'e'), node  $v_5$, $v_6$ and $v_7$ of type customer (denoted 'c'), and edges $e_1$, $\dots$, $e_9$ of type message (denoted 'm').  Each edge is associated with a set of time-points during which that edge is valid.}
  \label{fig:def2}
\end{figure}
 
 Assume in this graph, node $v_1$ shared a secret with $v_2$ and $v_3$ and one of them shared this secret with node $v_4$. Without the temporal data, both $v_2$ and $v_3$ can be a source of this information leak, but by looking at time-points on each edge, we can observe that there is no temporally valid path between $v_1$, $v_3$ and $v_4$. More formally, we can express a problem such as this, as a path of length two, with a temporal order over edges. Example~\ref{ex:exist-const} shows a case where we are looking for a path of length two, where the first edge in the path exists before or at the same time as the second edge in a temporal window of size two. 

\begin{example}
\label{ex:exist-const}
Path of length two, where the first edge exists at $t_1$ and second edge exists at $t_2$, $t_1 \leq t_2$ and $t_2 - t_1 \leq 2$ 
%$$a \xrightarrow{e_i} b \xrightarrow{e_j}: e_i.t \leq e_j.t$$. 

\begin{figure}[h!]
    \centering
    \begin{center}
    \begin{tikzpicture}[->, on grid, node distance=60pt]
    \node[state ] (a) {$a$};
    \node[state, right of=a] (b) {$b$};
     \node[state, right of=b] (c) {$c$};
    \draw
    (a) edge[left] node[above]{$y_1$} (b)
    (b) edge[left] node[above]{$y_2$} (c);
    \end{tikzpicture}
    \end{center}    
\caption{Path of Length 2}
    \label{fig:bgp-path}
\end{figure}


$$a \xrightarrow{y_1} b \xrightarrow{y_2} c: \exists t_1 \in y_1.T \exists t_2 \in y_2.T:  t_1 \leq t_2$$.
\end{example}

Various works have tackled different aspects of pattern matching in temporal graphs during recent years, but most of these works only  support temporal constraints such as the one in the Example~\ref{ex:exist-const}.  An example of such work in the literature is series of papers specifically focused on temporal motifs mining\cite{DBLP:journals/corr/abs-1107-5646,DBLP:conf/sigmod/GurukarRR15,DBLP:conf/wsdm/ParanjapeBL17}, with the goal of mining statistically significant frequent temporal subgraphs. In these temporal motifs, the edges follow a specific temporal order, such as the one demonstrated in Example~\ref{ex:exist-const}. Furthermore, these works defined $\delta$ temporal motifs~\cite{DBLP:conf/wsdm/ParanjapeBL17} where all the edges in a given motif occur inside the period of $\delta$ time units. For Example~\ref{ex:exist-const}, $\delta = 2$. The temporal graph model used in this family of works is similar to what is described in Figure~\ref{fig:def2} where nodes are persistent over time and edges can have one or multiple time-points. The goal of these studies has been to find the most frequent subgraphs, which can be achieved by algorithms that do not require the system to enumerate all matchings. These algorithms generally find all nontemporal motifs and efficiently count those that satisfy the temporal constraints.  %The main goal of all these works is to find frequent static patterns and then, among those counts, the ones that satisfy the temporal constraints.  
A complimentary work to frequent motif mining is finding the most durable patterns. A durable pattern is a pattern that persists over time, either continuously or collectively~\cite{semertzidis2016durable}. This has been done by counting the number of snapshots where each matching existed. %To the best of our knowledge, the only temporal constraint in this work is that all edges of one matching should exist during the snapshot.

While mining frequent or durable subgraphs will give insights about the evolution of graphs and are advantageous in many fields such as protein interaction~\cite{cho2009predicting}, social network~\cite{DBLP:journals/computer/FlakeLGC02,DBLP:journals/pvldb/WuCHKLX14,miritello2013temporal}, and fraud detection~\cite{choo2008money}, for many use-cases, users are rather interested in extracting all instances of one fixed temporal pattern. While the temporal graph model and our methods for representing the temporal constraints that we will describe in this work can be applied to motif mining, our focus here is on pattern extraction. 

One of the few works focused on temporal graph pattern matching is by Xu et al.~\cite{xu2017time}. They define a ``temporal graph'' as a set of static nodes and dynamic edges. Each edge has sets of intervals corresponding to the validity period of the edge. They introduced time constraint query patterns using Allen's interval algebra~\cite{Allen1983}. One other recent work using Allen's intervals to extract a subgraph from a temporal graph is Gradoop~\cite{rost2021distributed}. They defined their temporal model as a set of temporal nodes and temporal edges where each node / edge is valid for an interval. Gradoop  introduces a temporalGDL similar to Allen's intervals algebra,  which can be combined with Cypher~\cite{cypher} language to describe temporal BGPs.   While using Allen's algebra will enable us to express more complex constraints, it is limited to comparing two intervals and is not suitable for comparing two sets of intervals or two sets of time-points. \amir{ we can add ``Portal'' here, while Portal does not support temporal constraints it has subgraph operator the filter nodes / edges by a predicate and produce a temporally correct graph }

One other interesting work in the area of temporal pattern matching is Franzke et al.~\cite{DBLP:conf/edbt/ZufleREF18}, where they defined a ``temporal graph'' as a set of static nodes and dynamic edges, where each edge has a set of temporal points. Using a set of temporal points for each edge is more appropriate for cases where events do not have a duration.  Franzke et al. consider a particular class of temporal constraints where the time-points within a query range are specified \emph{exactly} up to the translation of the query range in a temporal range occurring in the temporal graph. One interesting aspect of this work is that they convert the history of each subgraph to a string and enforce the temporal constraint using a substring search algorithm. While this method of expressing constraints can work over a set of time-points, it is limited to continuous temporal constraints. That is to say, their model can not support reoccurring edges or temporal gaps. Reoccurring edges with a temporal pattern is a common phenomena in temporal graphs. In fraud detection, a single transaction might be acceptable, but multiple transactions between two suspicious users can be a red flag. In communication networks, users do send many messages to each other; for instance social networks users tend to send their friend a messages every year during that friend birthday week~\cite{DBLP:conf/sigmod/GurukarRR15}.  Examples~\ref{ex:complex-const1} shows one case of such constraints four our toy graph in Figure~\ref{fig:def2}. 

\begin{example}
\label{ex:complex-const1}
Assume in the graph in Figure~\ref{fig:def2}; we are looking for all pairs of customers and employees who exchanged emails in alternation in a temporal window of size two.  In other words, this means that the customer will send an email first, and during the subsequent two time units, the employee will reply, and the cycle will continue. 

The graph pattern for this question would be a loop of length two, which is described in Figure~\ref{fig:bgp-cycle2}. Figure~\ref{fig:def2} contains two loops of size two, $(e_5,e_6)$ and $(e_8,e_9)$ but only the latter satisfy the temporal constraint. 

\begin{figure}[h!]
    \centering
    \begin{center}
    \begin{tikzpicture}[->, on grid, node distance=60pt]
    \node[state ] (x) {$x$};
    \node[state, right of=x] (y) {$y$};
    \draw
    (x) edge[bend left] node[above]{$y_1$} (y)
    (y) edge[bend left] node[below]{$y_2$} (x);
    \end{tikzpicture}
    \end{center}    
\caption{Cycle of length 2}
    \label{fig:bgp-cycle2}
\end{figure}

\end{example}


To the best of our knowledge, expressing constraints such as the one in Example~\ref{ex:complex-const1}, is not possible using any of the models introduced in the literature and is difficult using existing query languages such as SQL and Cyper~\cite{cypher}.


In Section~\ref{sec:model}, we will introduce a formal definition for a new temporal graph model built with the problem of temporal pattern matching in mind. We then will introduce a novel method of expressing temporal constraints using timed-automaton~\cite{timed-automata} that can express all previously used constraints (e.g. Example~\ref{ex:exist-const}) and the reoccurring constraints (e.g. Example~\ref{ex:complex-const1}).We will show that timed-automaton can express all constraints studied in previous works and more. \amir{Can we use it over intervals?}. We then introduce efficient algorithms to enforce these constraints over the matching found in the graph. 

Another trend  of works related to temporal patterns is incremental graph pattern matching,~\cite{fan2013incremental,DBLP:conf/sigmod/HanLL13,DBLP:journals/tkde/ChenW10,DBLP:conf/sigmod/KimSHLHCSJ18,amsj_subgraph,DBLP:conf/eurosys/BindschaedlerML21}, where the goal is to find and maintain patterns in an updating stream of a graph.
In Section~\ref{sec:dataflow} we will show how our algorithm can be efficiently combined with state-of-the-art incremental and non-incremental matching algorithms. 



\paragraph{Contributions} 

Our contributions of this work are  summarized as follows \julia{present tense, not past tense}
\begin{itemize}
    \item We formally introduce a new temporal graph model motivated by the problem of graph pattern matching with complex temporal constraints.

    \item We introduce a novel method using ``timed automata'' to express temporal constraints. 
    
    \item We introduce algorithms to enforce the constraints expressed by ``timed automaton'' and combine those with state-of-the-art matching algorithms using dataflow operators.
    

    \item We show the effectiveness of our methods over graphs where the history is available and when the graph arrives as a stream.  

    \item We show that our method performance is independent of the size of temporal constraints and can be used to answer multiple constraints at once without change of performance. 

\end{itemize}


The rest of this paper is organized as follows. Section~\ref{?model} we will formally define a temporal graph model designed for graphs where nodes are static, but edges can exist over multiple time-points. Over this model, we define temporal graph patterns and temporal constraints. Using these formal definitions, then we introduce a novel method of expressing temporal constraints over graph patterns based on timed automaton~\cite{alur1994theory}. We will describe the timed automaton in detail in Section~\ref{?timed-automata}. Section~\ref{dataflow?} is focus on describing our algorithms to enforce the temporal constraints described by timed-automaton and how we can combine our algorithms with known matching algorithms that use incremental-joins over the stream of data. Using incremental algorithms would enable us to find temporal matching both when all information is available at once or when the graph is arriving over a period of time. In Section~\ref{?implementation} we will discuss our implementation details of these algorithms using Rust. Finally, we show our system performance for multiple real datasets, various patterns, and timed automaton in Section~\ref{expr}. 











==> old-tex/related.tex <==
\section{Related Work}
\label{sec:related}
Graph pattern matching has applications in knowledge discovery, information retrieval,  computer vision, biology, and sociology. One of the first pattern matching problems studied is the subgraph isomorphism problem. The subgraph isomorphism problem consists of deciding if there exists a copy of a graph-pattern in a target graph~\cite{zampelli2010solving}. 

Pattern matching algorithms can be categorized in many ways. One example of this categorization is exact-matching algorithms and inexact-matching algorithms. Exact matching methods require a strict correspondence among the two objects being matched. In contrast, in inexact matching methods~\cite{fan2010graph,reza2020approximate}, a matching can occur even if the two graphs being compared are structurally different from some extent~\cite{conte2004thirty}. It can be said that an exact match algorithm would return results that match a specific pattern, but an inexact match algorithm will return a ranked list of the most similar matches~\cite{gallagher2006matching}. The primary use of Inexact algorithms is where noise or errors are present in the graph.  One of the most famous  works for exact-matching problems is Ullmann's algorithm~\cite{ullmann1976algorithm} that was introduced in 1976 and uses depth-first-tree-search. One interesting aspects of Ullmann's work is the pruning step, where the algorithm uses criteria such as degree to eliminate the search path as early as possible.  Systems such as GraphQL~\cite{taelman2018graphql} and GADDI~\cite{zhang2009gaddi} , VF2~\cite{cordella2004sub} improved Ullmanns algorithm by introducing smarter search order, better index structure and refined heuristics.  

A popular approach for the exact pattern matching and finding subgraph is to implement the matching search algorithms using select-project-join queries~\cite{zou2009distance,DBLP:journals/vldb/NeumannW10,DBLP:journals/tods/AbergerLTNOR17}. It has been proven that the problem of Boolean conjunctive query evaluation is equivalent to the homomorphism problem, and hence the former is NP-complete in the general case~\cite{chandra1977optimal}. For decades, significant efforts have been put in to identify tractable cases of conjunctive query evaluation. In 1981, Yannakakis showed that the query evaluation problem is tractable for acyclic conjunctive queries ~\cite{yannakakis1981algorithms} and it runs in input/output polynomial time. A query is acyclic if the query hypergraph contains no cycles.  Yannankakis decomposition algorithm is the building block of modern DBMS join query plans ~\cite{Abiteboul1995}. Traditionally, DBMS has been used to utilize an Edge-at-time query plan for subgraph queries. However, in recent years, a more efficient family of join-plans called Worst-Case Optimal Join (WOJ) has been introduced, utilizing a node-at-time query plan. Algorithms such as Generic Join~\cite{DBLP:journals/sigmod/NgoRR13}, NPRR~\cite{DBLP:journals/jacm/NgoPRR18} and Leapfrog TrieJoin~\cite{DBLP:journals/corr/abs-1210-0481} belong to this trend. 




\julia{This section is stale.}
Temporal constraints are surveyed in a 1998 paper by Schwalb and Vila~\cite{DBLP:journals/constraints/SchwalbV98}.  The paper focuses on the Temporal Constraint Satisfaction Problem (TCSP) and, in particular, presents results on deciding satisfiability of TCSPs and on answering queries on TCSPs.  The paper surveys three classes of TCSPs: qualitative point, qualitative interval, metric point, and some combinations.

We have so far been working with qualitative point constraints (QPC).  Three algebras have been studied over such constraints: basic point algebra, with relations $<$, $=$, $>$, $?$, convex point algebra that also adds $\emptyset$, $\leq$ and $\geq$, and point algebra, that further includes the $\neq$ relation. 

Gutierrez et al.~\cite{DBLP:journals/tkde/GutierrezHV07} start an investigation of incorporating time into RDF, to support temporal reasoning (e.g., temporal entailment).  Temporal information is associated with triples using what the authors call \emph{labeling} --- associating time with triples directly.  This is in contrast to what they call \emph{versioning}, where a new version of the graph (a snapshot) is stored whenever some change occurs. 

Tappolet and Bernstein~\cite
{DBLP:conf/esws/TappoletB09} propose a temporal RDF extension, and a corresponding shorthand temporal format called $\tau$-SPARQL, with a translation of statements into standard SPARQL.

Ontology-Mediated Query Answering over Temporal Data: A Survey (Invited Talk), Artale et al.~\cite{DBLP:conf/time/ArtaleKKRWZ17}.

Other papers:
\begin{itemize}
\item papers about RDF and time:
	\begin{itemize}
    	\item brief survey with pointers to existing approaches~\cite{Wang2017}
		\item Gutierrez et al., journal version: \cite{DBLP:journals/tkde/GutierrezHV07}, conference paper: \cite{DBLP:conf/esws/GutierrezHV05}
		\item Tappolet and Bernstein~\cite{DBLP:conf/esws/TappoletB09}
		\item Koubarakis and Kyzirakos~\cite{DBLP:conf/esws/KoubarakisK10}, and a few later papers by these authors
		\item Perry et al.~\cite{DBLP:conf/swb/PerryJS11}
		\item ``A Framework for Generating Evolving RDF Graphs'' by Alami et al.~\cite{Alami2017}
	\end{itemize}
\end{itemize}

==> old-tex/todo.tex <==
\section{Todo}

\paragraph{Old list}
\begin{enumerate}
    \item
    If temporal constraint is given in SQL, compile the entire TBGP in SQL.  Give examples of TBGPs and the corresponding SQL queries. A general method for constructing SQL queries. (start with phase 1 of 6) - Julia
    \item
    Can a journey query on $k$ edge variables $e_1$, \dots, $e_k$ be expressed simply in terms of the mins and maxes? - Jan
    
    For example, for $k=2$ this seems to be possible, simply that the min of $e_1$ is less than max of $e_2$.
    \item
    Containment problem for TBGPs. - Jan
    \item
    Literature research: use of automata in temporal query processing? Ask Tova, Michael Boehlen. - Julia and Jan
    \item
    Literature research: processing techniques for timed automata? - Julia  (verification - tutorials for timed automata)
    \item
    Two-phase approach as an alternative to compiling into SQL. First phase, compute all matchings of the BGP. This can still be done in SQL of course.
    
    Second phase is to run the automaton on the temporal models for the different matchings. This could be done in parallel: keep a current state for each matching and run through the snapshots.
    
    \item {\bf New} see George Fletcher's response + see about processing BGPs over distributed architectures
    \item {\bf New} partitioning to efficiently process temporal BGPs (refer to two-phase approach)
    
\end{enumerate}

\paragraph{Plan of the paper}
\begin{enumerate}
    \item Motivate model of temporal graphs where each edge gets a SET of timepoints, not just a single one.
    \item Introduce our notion of temporal BGP which amounts to adding temporal constraints to BGPs.
    \item Discuss ways of formulating temporal constraints: possibly SQL, possibly some kind of temporal logic, possibly some kind of first-order logic, some kind of timed automata, last but not least: existential constraints.
    \item Two-phase processing approach, which assumes the set of matchings of the underlying BGP is given, and focuses on filtering out those temporal assignments that satisfy the temporal constraint. When the temporal constraint is given as a timed automaton, we need an algorithm for the following problem: given a set of temporal assignments, select those that are accepted by the automaton.
    \item Integrated approach, where we try to push the temporal constraint in the BGP matching process.  This should be attempted first for the simplest kind of temporal constraints, namely, the existential case.  The thing is that there are widely different approaches to BGP matching, we should focus on some of them?
    \item If we could say something about containment checking of temporal BGPs that would be good. It probably follows from known results on constraint query languages (Jan).
\end{enumerate}

==> otherqueries.tex <==
QTA1: WITH matching(y1, y2) AS (...), Succ AS
(SELECT y1, y2, A1.eid AS e1, A2.eid AS e2
 FROM matching, active A1, active A2
 WHERE (A1.eid = y1 OR A1.eid = y2) AND (A2.eid = y1 OR A2.eid = y2)
   AND A1.time<A2.time AND NOT EXISTS
         (SELECT * FROM active A3
          WHERE (A3.eid = y1 or A3.eid = y2)
            AND A1.time<A3.time AND A3.time<A2.time))
SELECT *  FROM matching M
WHERE NOT ( EXISTS (SELECT * FROM active WHERE eid = y2)
            AND NOT EXISTS (SELECT * FROM active WHERE eid = y1) )
  AND ( NOT EXISTS (SELECT * FROM active A1, active A2
                    WHERE A1.eid = y1 AND A2.eid = y2)
        OR (SELECT MIN(time) FROM active WHERE eid = y1) <
           (SELECT MIN(time) FROM active WHERE eid = y2) )
  AND NOT EXISTS (SELECT * FROM Succ
                  WHERE M.y1 = y1 AND M.y2 = y2 AND e1 = e2)
                  
QTA7: WITH matching(y1, y2) as (...)
 SELECT DISTINCT y1, y2 FROM matching, active A1, active A2, active B1, active B2 WHERE A1.eid = y1 AND A2.eid = y2 AND A1.time = A2.time AND B1.eid = y1 AND B2.eid = y2 AND B1.time = B2.time AND B1.time - A1.time > 3 AND NOT EXISTS
     (SELECT * FROM active C WHERE A1.time < C.time AND C.time < B1.time
        AND NOT EXISTS (SELECT * FROM active C1, active C2
           WHERE C1.time = C.time AND C2.time = C.time AND C1.eid = y1 AND C2.eid = y2))

==> scratch.tex <==
\multirow{9}{*}{\STAB{\rotatebox[origin=c]{90}{\textbf{EPL Cycle2}}}}
&$\ta_e$ & \multicolumn{1}{r|}{933} & 0.04 & 0.597 & \textbf{0.01} \\
&$\ta_1$ & \multicolumn{1}{r|}{35} & \textbf{0.01} & 2.67 & 0.41 \\
&$\ta_2$ & \multicolumn{1}{r|}{22} & \textbf{0.01} & 3.33 & 0.26 \\
&$\ta_3$ & \multicolumn{1}{r|}{418} & \textbf{0.01} & 0.1 & \textbf{0.01} \\
&$\ta_4$ & \multicolumn{1}{r|}{740} & \textbf{0.01} & 0.1 & \textbf{0.01} \\
&$\ta_5$ & \multicolumn{1}{r|}{90} & \textbf{0.02} & 0.53 & 1.19 \\
&$\ta_6$ & \multicolumn{1}{r|}{312} & 0.07 & 0.07 & \textbf{0.01} \\
&$\ta_7$ & \multicolumn{1}{r|}{0} & \textbf{0.05} & 1.18 & 5.15 \\
&$\ta_8$ & \multicolumn{1}{r|}{188} & 0.02 & \textbf{0.01} & 0.09 \\ \hline
\end{tabular}

\begin{tabular}{c|lrrrr}
\multirow{9}{*}{\STAB{\rotatebox[origin=c]{90}{\textbf{Contact O-Star2}}}}
& $\ta_e$ & \multicolumn{1}{r|}{169410} & \textbf{8.87} & 22.43 & 19.29 \\
& $\ta_1$ & \multicolumn{1}{r|}{0} & \textbf{0.67} & \omem & 316.5 \\
& $\ta_2$ & \multicolumn{1}{r|}{0} & \textbf{0.72} & \omem & 205.95 \\
& $\ta_3$ & \multicolumn{1}{r|}{101268} & \textbf{0.58} & 0.95 & 0.69 \\
& $\ta_4$ & \multicolumn{1}{r|}{107650} & \textbf{0.67} & 0.91 & 0.68 \\
& $\ta_5$ & \multicolumn{1}{r|}{4154} & \textbf{0.72} & \omem & 2.035 \\
& $\ta_6$ & \multicolumn{1}{r|}{10832} & 4.68 & 0.99 & \textbf{0.54} \\
& $\ta_7$ & \multicolumn{1}{r|}{76} & \textbf{15.12} & \omem & 102.89 \\
& $\ta_8$ & \multicolumn{1}{r|}{4646} & 1.3 & \textbf{1.1} & 1.16 \\ \hline
\multirow{9}{*}{\STAB{\rotatebox[origin=c]{90}{\textbf{Email Path2}}}}
& $\ta_e$ & \multicolumn{1}{r|}{719609} & 501.07 & 649.69 & \textbf{239.82} \\
& $\ta_1$ & \multicolumn{1}{r|}{35594} & \textbf{22.35} & \omem & \omem \\
& $\ta_2$ & \multicolumn{1}{r|}{801} & \textbf{3.73} & \omem & 1748.85 \\
& $\ta_3$ & \multicolumn{1}{r|}{443431} & \textbf{2.71} & 17.84 & 8.59 \\
& $\ta_4$ & \multicolumn{1}{r|}{455977} & \textbf{3.05} & 17.78 & 8.26 \\
& $\ta_5$ & \multicolumn{1}{r|}{2474} & \textbf{1.27} & \omem & 48.87 \\
& $\ta_6$ & \multicolumn{1}{r|}{693956} & 320.04 & 8.98 & \textbf{5.61} \\
& $\ta_7$ & \multicolumn{1}{r|}{390} & \textbf{327.33} & \omem & \omem \\
& $\ta_8$ & \multicolumn{1}{r|}{12919} & 19.32 & \textbf{8.02} & 21.58 \\ \hline
\multirow{9}{*}{\STAB{\rotatebox[origin=c]{90}{\textbf{Email Cycle2}}}}
$\ta_e$ & \multicolumn{1}{r|}{14188} & \textbf{4.71} & 254.7 & 15.3 \\
& $\ta_1$ & \multicolumn{1}{r|}{843} & \textbf{0.83} & \omem & 1788.87 \\
& $\ta_2$ & \multicolumn{1}{r|}{240} & \textbf{0.64} & \omem & 1733.05 \\
& $\ta_3$ & \multicolumn{1}{r|}{6333} & 0.44 & \textbf{0.38} & 0.68 \\
& $\ta_4$ & \multicolumn{1}{r|}{11396} & 0.43 & \textbf{0.38} & 0.68 \\
& $\ta_5$ & \multicolumn{1}{r|}{1800} & \textbf{0.97} & 206.26 & 1.19 \\
& $\ta_6$ & \multicolumn{1}{r|}{4230} & 24.09 & 8.63 & \textbf{5.48} \\
& $\ta_7$ & \multicolumn{1}{r|}{134} & \textbf{7.1} & \omem & \omem \\
& $\ta_8$ & \multicolumn{1}{r|}{3441} & 1.79 & \textbf{0.219} & 49.79

==> ta4.tex <==
\begin{figure}
    \centering
    
    \begin{tikzpicture}[->, on grid, node distance = 60pt]
    \node[state, initial] (s0) {$s_0$};
    \node[state, right of = s0] (s1) {$s_1$};
    \node[state, right of = s1, accepting] (s2) {$s_2$};
    \draw (s0)
  (s0) edge[loop above] node{$\emptyset$} (s0)
  (s1) edge[loop above] node{$\neg y_2$} (s1)
  (s2) edge[loop above] node{$\mathit{true}$} (s2)

  (s0) edge[above] node{$y_1 \land  \neg y_2$} (s1)
  (s0) edge[below, bend right = 18] node{$y_1 \land y_2 $} (s2)
  (s1) edge[above] node{$y_2$} (s2);
    \end{tikzpicture}
    \caption{$\ta_4$ - incremental order with equality for all patterns of size 2 for QT4.}
      \label{fig:apx:ta4-2}
\end{figure}

==> temp-const.tex <==
\section{Expressing Temporal Constraints}
\label{old_sec:automata}
\amir{ After agreeing on intro. section I need to go over this section and update all the exampled based on what we have there. }  

\amir{I think we can remove extra stuff  starting from Section 4.4 (Checking the temporal constrain)  }  


Our conception of a temporal BGP, as a standard BGP $P$ equipped with a temporal constraint $\Gamma$ on the edge variables of $P$, leaves open how $\Gamma$ is specified.  We next discuss three natural possibilities.

\subsection{Existential constraints}\label{sec:expres:existential}  This is arguably the simplest natural class of temporal constraints.  Consider the set of temporal variables $\{y_1,\dots,y_k\}$, with the corresponding timepoint variables $t_1$, \dots, $t_k$, where $t_i$ ranges over the timepoints assigned to $y_i$. An \emph{existential constraint} is a formula of the form
$$ \exists t_1 \in y_1 \dots \exists t_k\in y_k : \psi, $$ where $\psi$ is a Boolean combination of \emph{gap comparisons}.  Here, by a gap comparison, we mean a condition of the form $t_i \leq t_j + c$, where $c$ is a real number constant, possibly negative.  Note that by taking $c=0$ we obtain simple order comparisons as a special case.  Also, using negation, we obtain strict inequalities, and using conjunction, we can express equalities as well.

For example, consider a temporal graph where nodes are bus stops and edges are direct connections; an edge from node $v_1$ to $v_2$ is active at all timepoints where a bus departs at $v_1$ heading to $v_2$.  Assume for simplicity that time is measured in minutes since midnight. Now consider the BGP $x_1 \xrightarrow{y_1} x_2 \xrightarrow{y_2} x_3$ that looks for two consecutive edges $y_1$ and $y_2$.  Then the existential constraint $$ \exists t_1 \in y_1, \, \exists t_2 \in y_2 : t_2 \geq t_1 + 15 $$ would be satisfied by bus connections with at least fifteen minutes to do the change.

\subsection{SQL expressions} A much more powerful alternative,
which encompasses the existential constraints as a special case,
is to use SQL\@.  Ignoring labels for the moment, a temporal
graph can naturally be represented by two relations $\rm
Edge(\underline{eid}, from, to)$ and $\rm Active(eid,time)$,
where here eid stands for edge id.
Under this representation, BGPs are, of course, expressible in
SQL as cartesian products and equijoins over the Edge relation.
Arbitrary temporal constraints can then be added in the form of
extra conditions involving the Active table.

For example, the previous example temporal BGP, looking for bus connections with at least fifteen minutes in between, is expressed as
\begin{Verbatim}[fontsize=\small]
SELECT y1.eid, y2.eid 
FROM Edge y1, Edge y2, Active t1, Active t2 
WHERE y1.to=y2.from AND y1.eid=t1.eid AND y2.eid=t2.eid
  AND t2.time >= t1.time + 15
\end{Verbatim}

The SQL approach is not limited to existential constraints, however, as, in principle, any query expressible in SQL could be used.  For example, we could express the temporal constraint that all timepoints where $y_1$ is active come before all timepoints where $y_2$ is active.

\subsection{Timed automata} \label{sec:nfa}
 
Processing arbitrary SQL queries is of course overly general in that all the specifics about temporal BGPs and temporal graphs are lost.  We would lose the opportunity to design and exploit algorithms that are specifically focused on processing temporal BGPs.  We next propose an interesting alternative for expressing temporal constraints that lies in between the very simple existential constraints and the very general SQL constraints. The idea is to use \emph{timed automata}, an established formalism for expressing temporal constraints in the area of verification \cite{timed-automata,timed-automata-survey}.  While timed automata are often interpreted over infinite words, here we will use them on finite words.

A timed automata over a finite set $Y$ of variables is an extension of the standard notion of non-deterministic finite automata (NFA), over the alphabet $\Sigma = 2^Y$ (the set of subsets of $Y$).  Recall that an NFA specifies a finite set of states, an initial state, a set of final states,
and a set of transitions of the form $(s_1,\theta,s_2)$, where $s_1$ and $s_2$ are states and $\theta$ is a boolean formula over $Y$.  The automata reads a word over $\Sigma$, starting in the initial state.  Whenever the automata is in a current state $s_1$, the next letter to be read is $a$, and there exists a transition $(s_1,\theta,s_2)$ such that $a$ satisfies $\theta$, the automata can change state to $s_2$ and move to the next letter.  If, after reading the last letter, the automata is in a final state, the run accepts. If the last state is not final, or there is no suitable transition at some point, the run fails.  A word is accepted if there exists an accepting run.  

The extra feature added by timed automata to the standard NFA apparatus is a finite set $C$ of \emph{clocks}, which can be used to measure time gaps between successive letters in a \emph{timed} word (to be defined momentarily).  Transitions are of the extended form $$ (s_1,\theta,\delta,R,s_2), \eqno (*) $$ where $s_1$, $\theta$ and $s_2$ are as in NFAs; $\delta$ is a boolean combination of \emph{clock conditions}; and $R$ is a subset of $C$.  Here, by a clock condition, we mean a condition of the form $x \leq c$ or $x \geq c$, where $x$ is a clock and $c$ is a real number constant.

As just mentioned, timed automata work over timed words.  A timed word over an alphabet $\Sigma$ is a sequence of the form $$ (t_1,a_1)\dots (t_n,a_n), $$ where each $a_i \in \Sigma$, and $t_1 < \cdots < t_n$ are timepoints. When the automata is started on the timed word, all clocks are initially set to $t_0 := 0$. Now for $i=1,\dots,n$ the automata runs as follows.  Upon reading position $(t_i,a_i)$, every clock has increased by $t_i-t_{i+1}$. Now the automata can take a transition $(*)$ as above on condition that the current state is $s_1$ and $a_i$ satisfies $\theta$, as before; and, moreover, the current valuation of the clocks satisfies $\delta$.  If this is so, the automata can change state to $s_2$, move to the next position in the timed word, and must reset to zero all clocks in $R$.  As with NFAs, a run is accepting if it ends in a final state, and a timed word is accepted if there exists an accepting run.

A timed automata defines the set of timed words that it accepts. But how does it define, as announced, a temporal constraint over $Y$, which is not a set of timed words, but a set of temporal assignments?  This is simple once we realize that a temporal assignment over $Y$, in the context of a temporal graph $H = (G,\xi)$, is nothing but a timed word over $\Sigma = 2^Y$. We can see this as follows. Let $T = \bigcup \{\xi (e) \mid e \in E\}$ be the set of all distinct timepoints used in $H$; we also refer to $T$ as the \emph{temporal domain} of $H$. Let $T=\{t_1,\dots,t_n\}$, ordered as $t_1<\cdots<t_n$. We can then view any temporal assignment $\alpha : Y \to T$ as the timed word $(t_1,a_1)\dots (t_n,a_n)$, where $a_i = \{y \in Y \mid t_i \in \alpha (y)\}$.
%\marginpar{Julia: add example (see notes)}

NFAs are a special case of timed automata without any clocks, and this special case is already useful for expressing temporal constraints.
For example, consider the following NFA which expresses the existential constraint $ \exists t_1 \in y_1 \exists t_2 \in y_2 : t_1 < t_2$:
    \begin{center}
    \begin{tikzpicture}[->, on grid, node distance=60pt]
        \node[state, initial] (s0) {$s_0$};
        \node[state, right of=s0] (s1) {$s_1$};
        \node[state, accepting, right of=s1] (s2) {$s_2$};
        \draw (s0) edge[loop above] node{$\mathit{true}$} (s0)
      (s0) edge[above] node{$y_1$} (s1)
      (s1) edge[loop above] node{$\mathit{true}$} (s1)
      (s1) edge[above] node{$y_2$} (s2);
        \end{tikzpicture}
    \end{center}

As a simple example of the use of clocks, suppose we instead want to express the existential constraint $$ \exists t_1 \in y_1 \exists t_2 \in y_2 : t_1 < t_2-7. $$  We can do this by introducing a clock $\xx$. When we see $y_1$, we reset the clock.  Then when we see $y_2$, we check that the clock has progressed beyond the desired $7$ time units.
\begin{figure}[!h]
    \centering
    \begin{center}
        \begin{tikzpicture}[->, on grid, node distance=60pt]
        \node[state, initial] (s0) {$s_0$};
        \node[state, right of=s0] (s1) {$s_1$};
        \node[state, accepting, right of=s1] (s2) {$s_2$};
        \draw (s0) edge[loop above] node{$\mathit{true}$} (s0)
      (s0) edge[above] node{$y_1$} node[below]{$\xx:=0$} (s1)
      (s1) edge[loop above] node{$\mathit{true}$} (s1)
      (s1) edge[above] node{$y_2 \land \xx>7$} (s2);
        \end{tikzpicture}
    \end{center}
    \caption{Timed automata for $\exists t_1 \in y_1, \exists t_2 \in y_2 : t_1 < t_2-7$ }
    \label{fig:clock-automata}
\end{figure}

Of course, automata are more powerful than mere existential constraints.  For example, the following automata expresses the temporal constraint that $y_1$ and $y_2$ strictly alternate:
\begin{figure}[!h]
\caption{Alternation automata}
\label{fig:alt-nfa2}
    \centering
    \begin{center}
\begin{tikzpicture}[->, on grid, node distance=60pt]
\node[state, initial, accepting] (s0) {$s_0$};
\node[state, accepting, right of=s0] (s1) {$s_1$};
\draw
(s0) edge[bend left] node[above]{$y_1 \land \neg y_2$} (s1)
(s1) edge[bend left] node[below]{$y_2 \land \neg y_1$} (s0);
\end{tikzpicture}
\end{center}
\end{figure}
Note that the above temporal constraint is also expressible in SQL. Since the expression is complex, we give a more compact formulation in relational calculus.  The following formula $\psi(y_1,y_2)$ expresses that edges $y_1$ and $y_2$ strictly alternate in time, beginning with $y_1$:
\begin{align*}
& \exists t_1 (A(y_1,t_1) \land \neg \exists e \exists t (A(e,t) \land t<t_1)) \\
{} \land \bigwedge_{i=1,2} &
 \forall t(A(y_i,t) \to \exists t' (A(y_{3-i},t') 
\land \neg A(y_i,t') \land S(t,t'))),
\end{align*}
where $A$ abbreviates `Active' and
$S(t,t')$ abbreviates the formula stating that $t'$ is the successor of $t$ in the temporal domain: $t < t' \land \neg \exists e \exists t'' (\mathrm{Active}(e,t'') \land t < t'' < t')$.

The above formula $\psi$ (or an equivalent SQL expression) obscures the simple structure of the above automata.  Instead, in the next section, we will show how specific temporal matching methods can be designed by leveraging the automata directly.

% \jan{I actually think that everything below (until the next subsection) can be removed now.}

% \julia{Amir, please merge everything below into a single example.  The BGP and the graph should be part of the example environment.}

% Consider the following example. We are matching a BGP \\

% $P: x_1 \xrightarrow{y_1} x_2 \xrightarrow{y_2} x_3$  over a temporal graph $H=(G, \xi)$, where\\ $G=v_1 \xrightarrow{e_1} v_2 \xrightarrow{e_2} v_3 \xrightarrow{e_3} v_4$ and $\xi(e_1) = \{1, 2 \}$,  $\xi(e_2) = \{2, 3 \}$, and  $\xi(e_3) = \{1, 3 \}$.


% Consider the following example, where we are matching a BGP  $P: x_1 \xrightarrow{y_1} x_2 \xrightarrow{y_2} x_3$  over a temporal graph $H= (G, \xi)$, where:
% \begin{center}
% $G=v_1 \xrightarrow{e_1} v_2 \xrightarrow{e_2} v_3 \xrightarrow{e_3} v_4$ and $\xi (e_1) = \{1, 2 \}$,  $\xi (e_2) = \{2, 3 \}$, and  $\xi (e_3) = \{1, 3 \}$
% \end{center}


% \begin{example}\label{ex1}
% Consider the following matching: $\mu (x_1) =v_1$, $\mu (x_2) =v_2$, $\mu (x_3) =v_3$, $\mu (y_1) =e_1$ and $\mu (y_2) =e_2$. Then $\alpha_\mu (y_1) = \{1,2\}$ and $\alpha_\mu (y_2)=\{2,3\}$.

% We can represent this assignment $\alpha_\mu$ as the word consisting of the following letters: $a_1 = \{y_1\}$,  $a_2 = \{y_1,y_2\}$, $a_3 = \{y_2\}$.  Further, $\alpha_\mu$ can be viewed as:

% \begin{tabular}{llll}
% &$t_1=1$ & $t_2=2$ & $t_3=3$ \\
% $\alpha_\mu =$&$\{y_1\}$ & $\{y_1,y_2\}$ & $\{y_2\}$
% \end{tabular}

% This is both a word and a temporal assignment. 
% \end{example}


% Note that in Example~\ref{ex1}, the temporal domain $T$ does not have to be sequential over natural numbers, and can be, for example, $T = \{1.4, 3.8, 7\}$.  Using NFAs we can define complex and simple temporal constrains. Example~\ref{ex:precede-query} shows such an example for case where one edge edge ``prece'' another edge. 


% \begin{example}
% \label{ex:precede-query}
% Suppose we have a query `select all pair of edges ($y_1$,$y_2$)  where $y_1$  precedes $y_2$''. One can interpret this query in many ways, here we show three possible interpretations: (1) edge $y_1$ existed for at least one time-point before existence of edge $y_2$, (2) there exists at least one pair of time-points $(t_1, t_2)$, where edge $y_1$ existed at $t_1$ and edge $y_2$ existed at $t_2$, and where $t_1<t_2$, (3) edge $y_1$ did not exist at any time-points after existence of $y_2$. 
% The  NFAs in Figure~\ref{fig:nfa-simp} show each of these three interpretations. Note that the NFA in Figure~\ref{fig:nfa-simp-c} is equivalent to the first SQL query in Example~\ref{ex:sql-const} . Expressing the other two NFAs using a SQL query is extremely difficult.


% \begin{figure}[!h]%
% \caption{NFA for Example~\ref{ex:precede-query}}
% \label{fig:nfa-simp}
% \centering
% \subfloat[Interpretation 1]{
%     \begin{tikzpicture}[->, on grid, node distance=55pt]
%         \node[state, initial] (s0) {$s_0$};
%         \node[state,accepting, right of=s0] (s1) {$s_1$};
%         \draw 
%       (s0) edge[loop above] node{$\neg y_1 \land \neg y_2$} (s0)
%       (s0) edge[above] node{$y_1 \land \neg y_2$} (s1)
%       (s1) edge[loop above] node{$\mathit{true}$} (s1);
%         \end{tikzpicture}
% }%
% \subfloat[Interpretation 2]
%     {
%     \label{fig:nfa-simp-c}
%     \begin{tikzpicture}[->, on grid, node distance=40pt]
%         \node[state, initial] (s0) {$s_0$};
%         \node[state, right of=s0] (s1) {$s_1$};
%         \node[state, accepting, right of=s1] (s2) {$s_2$};
%         \draw (s0) edge[loop above] node{$\mathit{true}$} (s0)
%       (s0) edge[above] node{$y_1$} (s1)
%       (s1) edge[loop above] node{$\mathit{true}$} (s1)
%       (s1) edge[above] node{$y_2$} (s2);
%         \end{tikzpicture}
% }\\%
% \subfloat[Interpretation 3]{
%     \begin{tikzpicture}[->, on grid, node distance=55pt]
%         \node[state, initial] (s0) {$s_0$};
%         \node[state, right of=s0] (s1) {$s_1$};
%         \node[state, accepting, right of=s1] (s2) {$s_2$};
%         \draw (s0) 
%       (s0) edge[loop above] node{$\neg y_1 \land \neg y_2$} (s0)
%       (s0) edge[above] node{$y_1 \land \neg y_2$} (s1)
%       (s1) edge[loop above] node{$y_1 \land \neg y_2 $} (s1)
%       (s1) edge[above] node{$\neg y_1 \land y_2$} (s2)
%       (s2) edge[loop above] node{$\neg y_1 $} (s2);
        
%         \end{tikzpicture}
% }%
% \\
% \end{figure}

% \end{example}

% Note that while it is possible to express these constraints using SQL, it can be done only using complicated sub-queries. 

\subsection{Discussion}
\todo{incorporate this in the body of the paper and then remove this section}
Existential temporal constraints can be incorporated directly in the relational algebra expression $\Exp$, without any need to use an NFA.  For a simple example, consider a BGP $$ x_1 \overset{y_1}{\longrightarrow} x_2 \overset{y_2}{\longrightarrow} x_3 $$ with temporal constraint $$ \exists t_1 \in y_1 \exists t_2 \in y_2 : t_1 < t_2. $$  The resulting temporal BGP can be expressed in SQL as 
    \begin{verbatim}
SELECT $e_1$.eid AS y1, $e_2$.eid AS y2
FROM Edge $e_1$, Edge $e_2$, Active A1, Active A2
WHERE $e_1$.vid2 = $e_2$.vid1 
  AND $e_1$.eid=A1.eid AND $e_2$.eid=A2.eid
  AND A1.time < A2.time
    \end{verbatim}


==> vldb-block.tex <==
%%% do not modify the following VLDB block %%
%%% VLDB block start %%%
\pagestyle{\vldbpagestyle}
\begingroup\small\noindent\raggedright\textbf{PVLDB Reference Format:}\\
\vldbauthors. \vldbtitle. PVLDB, \vldbvolume(\vldbissue): \vldbpages, \vldbyear.\\
\href{https://doi.org/\vldbdoi}{doi:\vldbdoi}
\endgroup
\begingroup
\renewcommand\thefootnote{}\footnote{\noindent
This work is licensed under the Creative Commons BY-NC-ND 4.0 International License. Visit \url{https://creativecommons.org/licenses/by-nc-nd/4.0/} to view a copy of this license. For any use beyond those covered by this license, obtain permission by emailing \href{mailto:info@vldb.org}{info@vldb.org}. Copyright is held by the owner/author(s). Publication rights licensed to the VLDB Endowment. \\
\raggedright Proceedings of the VLDB Endowment, Vol. \vldbvolume, No. \vldbissue\ %
ISSN 2150-8097. \\
\href{https://doi.org/\vldbdoi}{doi:\vldbdoi} \\
}\addtocounter{footnote}{-1}\endgroup
%%% VLDB block end %%%

%%% do not modify the following VLDB block %%
%%% VLDB block start %%%
\ifdefempty{\vldbavailabilityurl}{}{
\vspace{.3cm}
\begingroup\small\noindent\raggedright\textbf{PVLDB Artifact Availability:}\\
The source code, data, and/or other artifacts have been made available at \url{\vldbavailabilityurl}.
\endgroup
}
%%% VLDB block end %%%
